Optimal Diagonal Preconditioning

Preconditioning has long been a staple technique in optimization, often applied to reduce the condition number of a matrix and speed up the convergence of algorithms. Although there are many popular preconditioning techniques in practice, most lack guarantees on reductions in condition number. Moreover, the degree to which we can improve over existing heuristic preconditioners remains an important practical question. In this paper, we study the problem of optimal diagonal preconditioning that achieves maximal reduction in the condition number of any full-rank matrix by scaling its rows and/or columns. We first reformulate the problem as a quasi-convex problem and provide a simple algorithm based on bisection. Then we develop an interior point algorithm with $O(\log(1/\epsilon))$ iteration complexity, where each iteration consists of a Newton update based on the Nesterov-Todd direction. Next, we specialize to one-sided optimal diagonal preconditioning problems, and demonstrate that they can be formulated as standard dual SDP problems. We then develop efficient customized solvers and study the empirical performance of our optimal diagonal preconditioning procedures through extensive experiments on large matrices. Our findings suggest that optimal diagonal preconditioners can significantly improve upon existing heuristics-based diagonal preconditioners at reducing condition numbers and speeding up iterative methods. Moreover, our implementation of customized solvers, combined with a random row/column sampling step, can find near-optimal diagonal preconditioners for matrices up to size 200,000 in reasonable time, demonstrating their practical appeal.

==> concentration.tex <==
\section{Diagonal Preconditioning and Reduction in Condition Number}
\label{sec:concentration}


In this section, we study the problem of when applying the diagonal
preconditioning method with normalization by column norm is effective
at reducing the condition number. When applying such methods, the
matrix being transformed is often a data or design matrix with i.i.d.
rows drawn from some common distribution. In this case the condition
number can also be viewed as a random variable. We first use matrix
concentration to show that with high probability, the reduction of
condition number using column normalization is close to that achieved
by transforming the population covariance matrix to the population
correlation matrix. Then we give sufficient conditions on when the
corresponding procedure on the population covariance matrix reduces
condition number significantly.

\subsection{Concentration of Condition Numbers}

We consider the setting where each row of the $n\times p$ design
matrix $X$ is an i.i.d. observation of a $p$-dimensional sub-Gaussian
vector. We are interested in how the procedure of normalizing by column
norm/standard deviation affects the condition number of the design
matrix. Because the condition number is a random variable in this
setting, we would like to simplify the analysis by first proving that
it concentrates around the condition number of population parameters
with high probability, from which we can conclude how much the condition
number can be reduced with this procedure. 

For ease of presentation, we assume for now that the sub-Gaussian
vector has mean zero and covariance matrix $\Sigma$. One of the most
common diagonal preconditioning procedures is to normalize each column
of $X$ by its mean or standard deviation. Thus we first analyze the
concentration behavior of the condition number under this particular
diagonal preconditioning, which takes the form 
\begin{align*}
X_{0} & =XD^{-\frac{1}{2}}
\end{align*}
where $D$ is the diagonal matrix with 
\begin{align*}
D_{jj} & =\frac{1}{n-1}\sum_{i=1}^{n}(X_{ij}-\mu_{j})^{2}\\
\mu_{j} & =\frac{1}{n}\sum_{i=1}^{n}X_{ij}\text{ or }\mu_{j}\equiv0
\end{align*}
corresponding to column variance or norm squared. 

We recall the definition of sub-Gaussian random vectors and some results
from matrix concentration and analysis that are useful in the proof
of our main result. 
\begin{definition}
	Define the sub-Gaussian norm of a random variable $x$ to be 
	\begin{align*}
	\|x\|_{\psi_{2}} & =\sup_{p\geq1}p^{-1/2}(\mathbb{E}|x|^{p})^{1/p}
	\end{align*}
	and the sub-Gaussian norm of a random vector $X\in\mathbb{R}^{n}$
	to be 
	\begin{align*}
	\|X\|_{\psi_{2}} & =\sup_{x\in S^{n-1}}\|\langle X,x\rangle\|_{\psi_{2}}
	\end{align*}
	
	Equivalently, the sub-Gaussian norm of $X$ is given by the smallest
	$K$ such that
	\begin{align*}
	\mathbb{E}\left[\exp(s\cdot u^{T}X)\right] & \leq\exp(K^{2}s^{2}/2),\forall s\in\mathbb{R},\|u\|=1
	\end{align*}
\end{definition}
\begin{lemma}
	(sub-Gaussian matrix concentration \cite{rudelson2010non} \label{lem:sub-Gaussian-concentration})
	Let $X$ be an $n\times p$ random matrix with $n>p$ and i.i.d sub-Gaussian
	rows $X_{i}$ with sub-Gaussian norm $K=\|X_{i}\|_{\psi_{2}}$ and
	$\Sigma=\mathbb{E}X_{i}^{T}X_{i}=\frac{1}{n}\mathbb{E}X^{T}X$ its
	second moment matrix. Then with probability at least $1-2\exp(-\frac{ct^{2}}{K^{4}})$,
	\begin{align*}
	\|\frac{1}{n}X^{T}X-\Sigma\|_{op} & \leq\max(\delta,\delta^{2})\\
	\delta & =CK^{2}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}
	\end{align*}
	where $c$ and $C$ are universal constants. Moreover, the above
	also implies
	\begin{align*}
	\sqrt{n}-(CK^{2})\sqrt{p}-t\leq\sigma_{\min}(X)\leq\sigma_{\max}(X) & \leq\sqrt{n}+(CK^{2})\sqrt{p}+t
	\end{align*}
\end{lemma}
%
\begin{lemma}
	(Weyl inequality \label{lem:weyl}) Let $\lambda_{i}(X)$ be the $i$-th
	eigenavlue of a self-adjoint matrix $X$. Then 
	\begin{align*}
	|\lambda_{i}(X)-\lambda_{i}(Y)| & \leq\|X-Y\|_{op}
	\end{align*}
	for all $i$. In other words, the eigenvalue map is 1-Lipschitz on
	the space of self-adjoint matrices with respect to the metric induced
	by the operator norm.
\end{lemma}
Our main result is that the condition number of $X_{0}^{T}X_{0}$
where $X=X_{0}D^{-\frac{1}{2}}$ concentrates around that of $D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}$,
where $D$ is the diagonal of $\Sigma$, i.e. $D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}$
is the population correlation matrix. Since $\kappa(X_{0}^{T}X_{0})=\kappa(X_{0})^{2}$,
this implies that $\frac{\kappa(X)}{\kappa(X_{0})}$ is on the order
of $\frac{\sqrt{\kappa(\Sigma)}}{\sqrt{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}}$
with high probability. 
\begin{theorem}
	\label{thm:concentration_1}Let $X$ be an $n\times p$ random matrix
	with $n>p$ and i.i.d. sub-Gaussian rows $X_{i}$ with $K=\|X_{i}\|_{\psi_{2}}$
	the sub-Gaussian norm of its rows, $\mathbb{E}X_{i}=0$, and let $\Sigma=\mathbb{E}X_{i}^{T}X_{i}=\frac{1}{n}\mathbb{E}X^{T}X$
	be the population covariance matrix. Let $\hat{D}$ be the diagonal
	matrix with $\hat{D}_{ii}=(X^{T}X)_{ii}$, i.e. $\hat{D}_{ii}$ is
	the norm squared of the $i$-th column of $X$, and let $X_{0}:=X\hat{D}^{-\frac{1}{2}}$
	be the matrix normalized with diagonal entries of $\hat{D}$. Then
	with probability at least $1-2\exp(-\frac{ct^{2}(\min_{i}(\Sigma)_{ii})^{2}}{K^{4}})-2\exp(-\frac{ct^{2}}{K^{4}})-2p\exp(-\frac{c}{K^{4}}\left[K^{2}+\frac{\min_{i}(\Sigma)_{ii}}{\sqrt{p}}\cdot t\right]^{2})$,
	we have
	\begin{align*}
	|\frac{\kappa(X^{T}X)}{\kappa(\Sigma)}- & \frac{\kappa(X_{0}^{T}X_{0})}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}|\leq\frac{2}{(1-(CK^{2})\sqrt{\frac{p}{n}}-\frac{t}{\sqrt{n}})^{2}}\cdot\left[CK^{2}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}\right]\\
	& +\frac{2}{(1-(C\frac{K^{2}}{\min_{i}(\Sigma)_{ii}})\sqrt{\frac{p}{n}}-3\frac{t}{\sqrt{n}})^{2}}\cdot\left[C\frac{K^{2}}{\min_{i}(\Sigma)_{ii}}\sqrt{\frac{p}{n}}+3\frac{t}{\sqrt{n}}\right]
	\end{align*}
\end{theorem}
\proof{Proof}
	See the appendix.\textbf{}%
	\begin{comment}
	\textbf{Note: dependence on $p$ may be refined. Refine it!}
	\end{comment}
	\hfill \Halmos
\endproof
\begin{comment}
\begin{proof}
Since the rows of $X$ are independent, its columns are sub-Gaussian
vectors with independent entries with sub-Gaussian norm bounded above
by $K$. Standard concentration result of the norm implies that with
probability at least $1-2\exp(-\frac{cT^{2}}{K^{4}})$, 
\begin{align*}
|\hat{D}_{ii}^{\frac{1}{2}}-D_{ii}^{\frac{1}{2}}| & \leq T
\end{align*}
for all large $T$. Union bound then gives that with probability
at least $1-2p\exp(-\frac{cT^{2}}{K^{4}})$, 
\begin{align*}
|\hat{D}_{ii}^{\frac{1}{2}}-D_{ii}^{\frac{1}{2}}| & \leq T,\forall i
\end{align*}
so that 
\begin{align*}
|\frac{\hat{D}_{ii}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}}-1| & \leq T\frac{1}{\sqrt{\min_{i}(\Sigma)_{ii}}}
\end{align*}
For any $i,j$, we have 
\begin{align*}
|\hat{D}_{ii}^{-\frac{1}{2}}X_{i}^{T}X_{j}\hat{D}_{jj}^{-\frac{1}{2}}-D_{ii}^{-\frac{1}{2}}X_{i}^{T}X_{j}D_{jj}^{-\frac{1}{2}}| & \leq\|X_{i}^{T}\|_{2}\|X_{j}^{T}\|_{2}|\hat{D}_{ii}^{-\frac{1}{2}}\hat{D}_{jj}^{-\frac{1}{2}}-D_{ii}^{-\frac{1}{2}}D_{jj}^{-\frac{1}{2}}|\\
& =|\hat{D}_{ii}^{\frac{1}{2}}\hat{D}_{jj}^{\frac{1}{2}}|\cdot|\hat{D}_{ii}^{-\frac{1}{2}}\hat{D}_{jj}^{-\frac{1}{2}}-D_{ii}^{-\frac{1}{2}}D_{jj}^{-\frac{1}{2}}|\\
& =|1-\frac{\hat{D}_{ii}^{\frac{1}{2}}\hat{D}_{jj}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}D_{jj}^{\frac{1}{2}}}|\\
& =|1-\frac{\hat{D}_{ii}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}}+\frac{\hat{D}_{ii}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}}-\frac{\hat{D}_{ii}^{\frac{1}{2}}\hat{D}_{jj}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}D_{jj}^{\frac{1}{2}}}|\\
& \leq|1-\frac{\hat{D}_{ii}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}}|+|\frac{\hat{D}_{ii}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}}-\frac{\hat{D}_{ii}^{\frac{1}{2}}\hat{D}_{jj}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}D_{jj}^{\frac{1}{2}}}|\\
& \leq T\frac{1}{\sqrt{\min_{i}(\Sigma)_{ii}}}(1+\frac{\hat{D}_{ii}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}})\\
& \le2\frac{T^{2}}{\min_{i}(\Sigma)_{ii}}
\end{align*}
for all large $T$. 

The relation between operator norm and maximum entry of a matrix $A$,
$\|A\|_{op}\leq\sqrt{np}\cdot\max_{i,j}|A_{ij}|$ then implies that 

\begin{align*}
\|\frac{1}{n}D^{-\frac{1}{2}}X^{T}XD^{-\frac{1}{2}}-\frac{1}{n}\hat{D}^{-\frac{1}{2}}X^{T}X\hat{D}^{-\frac{1}{2}}\|_{op} & \leq\sqrt{np}\cdot\frac{1}{n}\max_{i,j}|\hat{D}_{ii}^{-\frac{1}{2}}X_{i}^{T}X_{j}\hat{D}_{jj}^{-\frac{1}{2}}-D_{ii}^{-\frac{1}{2}}X_{i}^{T}X_{j}D_{jj}^{-\frac{1}{2}}|\\
& \leq2\frac{T^{2}}{\min_{i}(\Sigma)_{ii}}\cdot\sqrt{\frac{p}{n}}
\end{align*}

Now recall the result from Theorem 5, that with probability at least
$1-2\exp(-\frac{ct^{2}(\min_{i}(\Sigma)_{ii})^{2}}{K^{4}})-2\exp(-\frac{ct^{2}}{K^{4}})$,
the following two inequalities hold simultaneously
\begin{align*}
\|\frac{1}{n}D^{-\frac{1}{2}}X^{T}XD^{-\frac{1}{2}}-D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}\|_{op} & \leq C\frac{K^{2}}{\min_{i}(\Sigma)_{ii}}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}\\
\|\frac{1}{n}X^{T}X-\Sigma\|_{op} & \leq CK^{2}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}
\end{align*}
Now choose $T$ such that $T^{2}=K^{2}+\frac{\min_{i}(\Sigma)_{ii}}{\sqrt{p}}\cdot t$,
we see that 
\begin{align*}
\|\frac{1}{n}D^{-\frac{1}{2}}X^{T}XD^{-\frac{1}{2}}-\frac{1}{n}\hat{D}^{-\frac{1}{2}}X^{T}X\hat{D}^{-\frac{1}{2}}\|_{op} & \leq2\frac{K^{2}}{\min_{i}(\Sigma)_{ii}}\cdot\sqrt{\frac{p}{n}}+2\frac{t}{\sqrt{n}}
\end{align*}
so that 
\begin{align*}
\|\frac{1}{n}\hat{D}^{-\frac{1}{2}}X^{T}X\hat{D}^{-\frac{1}{2}}-D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}\|_{op} & \leq C\frac{K^{2}}{\min_{i}(\Sigma)_{ii}}\sqrt{\frac{p}{n}}+3\frac{t}{\sqrt{n}}\\
\|\frac{1}{n}X^{T}X-\Sigma\|_{op} & \leq CK^{2}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}
\end{align*}
and eigenvalue stability result allows us to conclude that 
\begin{align*}
|\frac{\kappa(X^{T}X)}{\kappa(\Sigma)}-\frac{\kappa(X_{0}^{T}X_{0})}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}| & \leq\frac{2}{(1-(CK^{2})\sqrt{\frac{p}{n}}-\frac{t}{\sqrt{n}})^{2}}\cdot\left[CK^{2}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}\right]\\
& +\frac{2}{(1-(C\frac{K^{2}}{\min_{i}(\Sigma)_{ii}})\sqrt{\frac{p}{n}}-3\frac{t}{\sqrt{n}})^{2}}\cdot\left[C\frac{K^{2}}{\min_{i}(\Sigma)_{ii}}\sqrt{\frac{p}{n}}+3\frac{t}{\sqrt{n}}\right]
\end{align*}
with probability at least 
\begin{align*}
1-2\exp(-\frac{ct^{2}(\min_{i}(\Sigma)_{ii})^{2}}{K^{4}})-2\exp(-\frac{ct^{2}}{K^{4}})-2p\exp(-\frac{c}{K^{4}}\left[K^{2}+\frac{\min_{i}(\Sigma)_{ii}}{\sqrt{p}}\cdot t\right]^{2})
\end{align*}
\end{proof}
\end{comment}
%
If we assume that the diagonal of $\Sigma$ is lower bounded, we can
further simplify the bound. 
\begin{corollary}
	Same assumptions as the previous theorem, and additionally $\min_{i}(\Sigma)_{ii}\geq1$.
	Then 
	\begin{align*}
	|\frac{\kappa(X^{T}X)}{\kappa(\Sigma)}- & \frac{\kappa(X_{0}^{T}X_{0})}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}|\leq\frac{6}{(1-(CK^{2})\sqrt{\frac{p}{n}}-3\frac{t}{\sqrt{n}})^{2}}\cdot\left[CK^{2}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}\right]
	\end{align*}
	with probability at least 
	\begin{align*}
	1-4\exp(-\frac{ct^{2}}{K^{4}})-2p\exp(-\frac{c}{K^{4}}\left[K^{2}+\frac{t}{\sqrt{p}}\right]^{2})
	\end{align*}
\end{corollary}
It is straightforward to extend these results to the case of sub-Gaussian
matrices with independent rows and non-zero mean. The above results
imply that with high probability, the ``reduction'' in condition
number of a sub-Gaussian design matrix with column normalization is
on the order of $\sqrt{\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}}$.
Therefore we can shift the focus of our analysis to the problem of
comparing the condition numbers of population covariance and correlation
matrices. 

\textbf{Proof Strategy} Because the scaling matrix $D=\hat{D}$ is
a function of sample statistics, namely the column-wise sample standard
deviations or column norm, the analysis with $\hat{D}$ directly is
cumbersome. Our strategy for showing the main result is to start with
the simplest possible case for $D$ and gradually increase the complexity
of the scaling matrix. More precisely, we show a sequence of concentration
results, each one built on top of the other, with the following scaling
matrices:
\begin{itemize}
	\item $D$ is equal to the population covariance matrix $\Sigma$, with
	general non-diagonal $\Sigma$.
	\item $D$ is the sample column-wise standard deviation, under the assumption
	that $\Sigma$ is diagonal. 
	\item $D$ is the diagonal of the population covariance matrix, with general
	non-diagonal $\Sigma$.
	\item $D$ is the sample standard deviation, with general non-diagonal $\Sigma$. 
\end{itemize}
For details of the proof, see the appendix. 

\begin{remark}
	The diagonal preconditioning considered in the above results is widely
	used in practice. It is common knowledge that when variables have
	different scales, the condition number of the design matrix (whose
	columns correspond to variables) tends to be large. This can be alleviated
	by rescaling the columns of the design matrix by its norm, so that
	each column has norm 1. This procedure does not guarantee, however,
	that there is always a significant reduction in condition number.
	In the next subsection, we study conditions under which such a procedure
	does result in a significant reduction in condition number, or equivalently
	that $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}\gg1$. 
	
	\begin{comment}
	\begin{rem}
	We have shown that diagonal pre-conditioning with batch standard deviations
	yields matrices with condition numbers close to the population correlation
	matrix. The next question is then: When does a covariance matrix have
	a much larger condition number than its corresponding correlation
	matrix. 
	
	The condition number of a correlation matrix and a covariance matrix
	are related in the following way. Let $\Sigma_{0}$ be a correlation
	matrix, and let $\Sigma_{0}=LL^{T}$ be the Cholesky decomposition
	of $\Sigma$ with $L$ a lower triangular matrix. Then 
	\begin{align*}
	\kappa(\Sigma_{0}) & =\kappa^{2}(L)=\kappa^{2}(L^{T})
	\end{align*}
	and 
	\begin{align*}
	\kappa(D^{\frac{1}{2}}\Sigma_{0}D^{\frac{1}{2}}) & =\kappa^{2}(L^{T}D^{\frac{1}{2}})=\kappa^{2}(D^{\frac{1}{2}}L)
	\end{align*}
	Because $\Sigma_{0}$ is a correlation matrix, the diagonal entries
	of $L$ have norm bounded above by 1. If the spectrum of $D$ satisfy
	$\sigma_{\max}(D^{\frac{1}{2}})\cdot\sigma_{\min}(L)\gg1$, then
	\begin{align*}
	\kappa(D^{\frac{1}{2}}L) & \approx\kappa(D^{\frac{1}{2}})\cdot\kappa(L)
	\end{align*}
	
	\textbf{(Need to write formal analysis of the statement)}
	
	The Cholesky factorization also tells us when a correlation matrix
	is ill-conditioned. Consider $LL^{T}$, with the condition that the
	norm of every column is 1. Then the off diagonal of $LL^{T}$ is large
	if and only if the corresponding diagonal of $L$ is small (so that
	the mass of that row is concentrated on the off-diagonal), i.e. $L$
	is ill-conditioned. 
	
	So the condition number of a covariance matrix is largely dependent
	on the scale difference between the largest standard deviation and
	smallest standard deviation. If the diagonal matrix with standard
	deviations is ill-conditioned, so will be the covariance matrix.
	
	Assume $U$ is square invertible with $|u_{ii}|\ge\alpha\sum_{j\neq i}|u_{ij}|\geq0$,
	then 
	\begin{align*}
	\kappa(U) & \leq\frac{\alpha+1}{\alpha-1}\cdot\frac{\max_{i}|u_{ii}|}{\min_{i}|u_{ii}|}
	\end{align*}
	so what we are looking for is a lower bound, that says if the matrix
	is not diagonally dominant, then it is ill-conditioned. This can then
	be applied to conclude that covariance matrix with columns of different
	scales generally is much more ill-conditioned than correlation matrix.
	\begin{align*}
	\frac{\kappa(\Sigma)}{\kappa(D)}\leq\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}) & \leq\kappa(D^{-1})\cdot\kappa(\Sigma)
	\end{align*}
	and we would like to show 
	\begin{align*}
	\frac{\kappa(\Sigma)}{\kappa(D)} & \approx\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})
	\end{align*}
	for a suitable class of matrices $\Sigma$. 
	
	Is $\frac{\alpha+1}{\alpha-1}$ a proxy of the condition number of
	$\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})$? Yes-- the larger
	$\alpha$ is, the closer $D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}$
	is to the identity matrix, and the closer its condition number is
	to 1. Hence the what we are looking for is a result that connects
	$\alpha$ to the condition number of the scaled matrix.
	\end{rem}
	\end{comment}
\end{remark}

\subsection{Diagonal Dominance and Condition Number}

In the previous subsection, we showed that diagonal pre-conditioning
with sample column norms yields matrices with condition numbers close
to the population correlation matrix, so that $\frac{\kappa(X^{T}X)}{\kappa(\Sigma)}$
and $\frac{\kappa(X_{0}^{T}X_{0})}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}$
are both close to 1 with high probability. In other words, the reduction
in condition number by diagonal preconditioning is on the order of
$\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}$.
This ratio, however, is not always large. In fact, it is not even
bounded below by 1. To study when the diagonal preconditioning procedure
is effective in reducing condition number, we pose the next question
in our analysis of diagonal preconditioning and condition numbers: 
\begin{question}
	For what covariance matrices $\Sigma$ is the ratio $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}$
	large, where $D=\text{diag}(\Sigma)$?
\end{question}
\begin{comment}
\textbf{connection with Jacobi method}
\end{comment}
It is well-known that a matrix whose columns have different scales
tends to have a large condition number. This is the reason behind
normalization procedures used to process data in a variety of contexts
such as PCA and first order optimization methods. However, the answer
to our question about whether the correlation matrix has a much smaller
condition number will depend on the structure of the correlation matrix
as well. 

As a first step to explore this dependence, we randomly generate some
covariance matrices and look for those with small ratio $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}$.
In Table \ref{tab:bad covariance} we present some examples of covariance
matrices with $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}<1$,
i.e. the correlation matrix is more ill-conditioned than the covariance
matrix.

\textbf{}
\begin{table}
	\begin{centering}
		\textbf{}%
		\begin{tabular}{|c|c|}
			\hline 
			$\Sigma$ & $D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}$\tabularnewline
			\hline 
			\hline 
			$\begin{bmatrix}0.17 & -0.49 & -0.19 & -0.36\\
			& 2.34 & 0.71 & 1.79\\
			&  & 0.32 & 0.53\\
			&  &  & 1.44
			\end{bmatrix}$ & $\begin{bmatrix}1 & -0.77 & -0.80 & -0.73\\
			& 1 & 0.81 & 0.97\\
			&  & 1 & 0.78\\
			&  &  & 1
			\end{bmatrix}$\tabularnewline
			\hline 
			$\begin{bmatrix}1.76 & -0.41 & -0.61 & -1.86\\
			& 0.21 & -0.11 & -0.45\\
			&  & 0.28 & 0.64\\
			&  &  & 1.99
			\end{bmatrix}$ & $\begin{bmatrix}1 & -0.66 & -0.86 & 0.99\\
			& 1 & -0.47 & -0.68\\
			&  & 1 & 0.85\\
			&  &  & 1
			\end{bmatrix}$\tabularnewline
			\hline 
		\end{tabular}
		\par\end{centering}
	\textbf{\caption{\label{tab:bad covariance}Examples of covariance matrices whose corresponding
			correlation matrices have larger condition number.}
	}
\end{table}
We see that the correlation matrices with large condition numbers
all have off-diagonal entries that are close to 1, which is confirmed
by other examples. %
\begin{comment}
We conjecture that if a covariance matrix $\Sigma$ satisfies $\Sigma_{ij}\approx\sqrt{\Sigma_{ii}\Sigma_{jj}}$,
the associated correlation matrix has a large condition number.\textbf{
In particular, we show first that if the correlation matrix has large
off-diagonal terms, its condition number tends to be large. In this
case, diagonal preconditioning does not help much.}
\end{comment}

In this section, we show that if a covariance matrix $\Sigma$ has
columns (and rows) that are of different scales, but its corresponding
correlation matrix is diagonally dominant, then diagonal preconditioning
can achieve a reduction in condition number on the order of $\kappa(D)$
with high probability, where $D$ is the matrix consisting of the
diagonal entries of $\Sigma$. To put the result in perspective, note
that $\kappa(\Sigma)\leq\kappa(D)\cdot\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})$
is always true. We are interested in sufficient conditions that guarantee
a matching lower bound, so that $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}\approx\kappa(D)$,
i.e. the reduction is on the order of $\kappa(D)$ with high probability
for a class of matrices. 
\begin{remark}
	\begin{comment}
	\textbf{Need to clean up.}
	\end{comment}
	One useful tool that helps us to understand the condition numbers
	of correlation and covariance matrices is the Cholesky decomposition:
	any positive definite matrix $M$ can be written as $M=LL^{T}$ where
	$L$ is a lower triangular matrix with non-negative diagonal entries. 
	
	Let $\Sigma_{0}$ be a correlation matrix, that is $\Sigma_{0}$ is
	positive definite with diagonal entries equal to 1 and off-diagonal
	entries in $[-1,1]$ and let $D$ be a diagonal matrix with strictly
	positive entries. Then $D^{\frac{1}{2}}\Sigma_{0}D^{\frac{1}{2}}$
	defines a covariance matrix whose diagonal is equal to $D$. 
	
	Let $\Sigma_{0}=LL^{T}$ be the Cholesky decomposition of $\Sigma_{0}$.
	This decomposition gives us some intuition about when a correlation
	matrix is ill-conditioned. Since $\Sigma_{0}$ has diagonal entries
	equal to 1, the norm of every row of $L$ is 1. Suppose $(\Sigma_{0})_{ij}$
	has large magnitude for some $i<j$. Since $(\Sigma_{0})_{ij}=\ell_{i}^{T}\ell_{j}$
	where $\ell_{i}$ denotes the $i$th row of $\Sigma_{0}$, and $L_{ij}=0$
	for $j>i$ because $L$ is lower triangular, $|\ell_{i}^{T}\ell_{j}|$
	is large only if the first $i$ entries of $\ell_{j}$ has large norm,
	which forces $L_{jj}$ to be small. The condition number of $L$,
	$\kappa(L)$, is not equal to $\frac{\max_{i}|L_{ii}|}{\min_{i}|L_{ii}|}$,
	which is only true for diagonal matrices. However, as we have seen,
	$\kappa(L)\geq\frac{\max_{i}|L_{ii}|}{\min_{i}|L_{ii}|}$, which implies
	that $\kappa(L)$ is likely to be large, i.e. $\Sigma_{0}$ is ill-conditioned.
	This heuristic argument will be made rigorous, but it provides the
	main intuition that a correlation matrix is ill-conditioned if and
	only if it has off-diagonal term with magnitude close to 1. 
	
	By the basic properties of condition number, $\kappa(\Sigma_{0})=\kappa^{2}(L)=\kappa^{2}(L^{T})$
	and 
	\begin{align*}
	\kappa(\Sigma) & =\kappa(D^{\frac{1}{2}}\Sigma_{0}D^{\frac{1}{2}})
	=\kappa^{2}(L^{T}D^{\frac{1}{2}})=\kappa^{2}(D^{\frac{1}{2}}L)
	\end{align*}
	Again, since $\kappa(D^{\frac{1}{2}}L)\geq\frac{\max_{i}|L_{ii}D_{ii}^{\frac{1}{2}}|}{\min_{i}|L_{ii}D_{ii}^{\frac{1}{2}}|}$
	and $L_{ii}$ are bounded above by 1, the right hand side will be
	dominated by $\frac{\max_{i}(D_{ii}^{\frac{1}{2}})}{\min_{i}(D_{ii}^{\frac{1}{2}})}=\kappa(D^{\frac{1}{2}})$
	if $\max_{i}(D_{ii}^{\frac{1}{2}})\gg1$ and $\frac{\max_{i}L_{ii}}{\min_{i}L_{ii}}$
	is not too large. On the other hand, if $\frac{\max_{i}L_{ii}}{\min_{i}L_{ii}}$
	is large, in which case $\Sigma_{0}$ is ill conditioned, then the
	right hand side may well be dominated by this quantity instead of
	$\kappa(D^{\frac{1}{2}})$.
	
	So the intuition here is that the condition number of a covariance
	matrix also depends on the scale difference between the largest standard
	deviation and smallest standard deviation. If the diagonal matrix
	$D$ of variances is ill-conditioned but the correlation matrix is
	well conditioned, the condition number of the covariance matrix is
	close to that of its diagonal. 
\end{remark}
The Cholesky decomposition has thus provided us with the following
two intuitions. First, a correlation matrix is ill conditioned if
it has off diagonal entries with magnitude close to 1. Second, if
the diagonal of a covariance matrix has a large condition number,
then likely so does the covariance matrix itself. We now make these
intuitions rigorous. 

We start with a result on the condition number of diagonally dominant
matrices. 
\begin{lemma}
\label{lem:diagonal dominance}Assume $M\in\mathbb{R}^{p\times p}$
is square invertible with $|M_{ii}|\ge\alpha\sum_{j\neq i}|M_{ij}|$
for all $i$ and some $\alpha>1$, then 
\begin{align*}
\kappa_{\infty}(M) & \leq\frac{\alpha+1}{\alpha-1}\cdot\frac{\max_{i}|M_{ii}|}{\min_{i}|M_{ii}|}
\end{align*}
for $\kappa_{\infty}$ defined based on the sup norm $\|M\|_{\infty}=\sup_{i,j}|M_{ij}|$,
and 
\begin{align*}
\kappa_{q}(M) & \leq p{}^{2/q}\frac{\alpha+1}{\alpha-1}\cdot\frac{\max_{i}|M_{ii}|}{\min_{i}|M_{ii}|}
\end{align*}
for $\kappa_{q}$ defined based on the $q$-norm $\|M\|_{q}=\sup_{\|v\|_{q}=1}\|Mv\|_{q}$
for $1\leq q<\infty$.
\end{lemma}
\proof{Proof}
For a fixed vector $x\in\mathbb{R}^{p}$, let $\|x\|_{\infty}=|x_{i}|$.
We have 
\begin{align*}
|(Mx)_{i}| & \geq|M_{ii}||x_{i}|-\sum_{j\neq i}|M_{ij}||x_{j}| \geq|M_{ii}||x_{i}|-\sum_{j\neq i}|M_{ij}||x_{i}|\\
& \geq(1-\frac{1}{\alpha})|M_{ii}||x_{i}|=(1-\frac{1}{\alpha})|M_{ii}|\|x\|_{\infty}
 \geq(1-\frac{1}{\alpha})\min_{i}|M_{ii}|\|x\|_{\infty}
\end{align*}
which implies $\frac{\|Mx\|_{\infty}}{\|x\|_{\infty}}\geq(1-\frac{1}{\alpha})\min_{i}|M_{ii}|$,
so that 
\begin{align*}
\|M^{-1}\|_{\infty} & =\max_{x\neq0}\frac{\|M^{-1}x\|_{\infty}}{\|x\|_{\infty}}=\max_{x\neq0}\frac{\|M^{-1}Mx\|_{\infty}}{\|Mx\|_{\infty}}\\
& =\max_{x\neq0}\frac{\|x\|_{\infty}}{\|Mx\|_{\infty}}\leq\frac{\alpha}{\alpha-1}\cdot\frac{1}{\min_{i}|M_{ii}|}
\end{align*}
On the other hand, 
\begin{align*}
\|M_{i}\|_{\infty} & \leq\sum_{j}|M_{ij}|\leq(1+\frac{1}{\alpha})|M_{ii}| \leq(1+\frac{1}{\alpha})\max_{i}|M_{ii}|
\end{align*}
from which we can conclude that $\kappa_{\infty}(M)\leq\frac{\alpha+1}{\alpha-1}\frac{\max_{i}|M_{ii}|}{\min_{i}|M_{ii}|}$.

Based on the upper bound for $\kappa_{\infty}$ and equivalence of
matrix norms, we can obtain upper bounds for condition numbers based
on $q$-norms. By Holder's inequality, $\|M\|_{q}\leq n^{1/q-1/q'}\|M\|_{q'}$
for $q\leq q'\leq\infty$. This suggests that $\|M\|_{q}\leq n^{1/q}\|M\|_{\infty}$
and so 
\begin{align*}
\kappa_{q}(M) & \leq p^{2/q}\kappa_{\infty}(M)\leq p^{2/q}\cdot\frac{\alpha+1}{\alpha-1}\frac{\max_{i}|M_{ii}|}{\min_{i}|M_{ii}|}
\end{align*}
	\hfill \Halmos
\endproof
To understand the above lemma in the context of covariance and correlation
matrices, compare $\kappa(\Sigma) \leq\kappa(\Sigma_{0})\cdot\kappa(D)$ with the bound 
\begin{align*}
\kappa(\Sigma) & \leq p\frac{\alpha+1}{\alpha-1}\frac{\max_{i}|\Sigma_{ii}|}{\min_{i}|\Sigma_{ii}|}=p\frac{\alpha+1}{\alpha-1}\cdot\kappa(D)
\end{align*}
from the lemma. We can see $\frac{\alpha+1}{\alpha-1}$ as a proxy
of the condition number $\kappa(\Sigma_{0})$ of the correlation matrix.
The larger $\alpha$ is, the closer $\Sigma_{0}$ is to the identity
matrix, and the closer its condition number is to 1. In the limit,
we should have $\lim_{\alpha\rightarrow\infty}\kappa(\Sigma_{0})=1=\lim_{\alpha\rightarrow\infty}\frac{\alpha+1}{\alpha-1}$.%
\begin{comment}
\textbf{Hence the what we are looking for is a result that connects
$\alpha$ to the condition number of the scaled matrix. }

There are analogous bounds if we assume similar diagonal dominance
properties in $p$-norm.\textbf{ The upper bounds for $\kappa_{p}$
are not very satifactory because of the dependence on dimension. If
instead of $|M_{ii}|\ge\alpha\sum_{j\neq i}|M_{ij}|$, we have an
analogous diagonal dominance condition in $p$-norm, we can obtain
dimension independent bounds.}
\begin{lem}
Assume $M\in\mathbb{R}^{n\times n}$ is square invertible with $|M_{ii}|\ge\alpha\cdot n^{\frac{1}{p}}\cdot(\sum_{j\neq i}|M_{ij}|^{q})^{1/q}$
for $\alpha>1$ and all $i$, then 
\begin{align*}
\kappa_{p}(M) & \leq\frac{(1+\frac{1}{\alpha^{q}n^{\frac{q}{p}}})^{\frac{1}{q}}\cdot n^{\frac{1}{p}}}{(1-\frac{1}{\alpha})}\cdot\frac{\max_{i}|M_{ii}|}{\min_{i}|M_{ii}|}
\end{align*}
for $1\leq q<\infty$ and $\frac{1}{p}+\frac{1}{q}=1$. 
\end{lem}
\begin{proof}
We have
\begin{align*}
|(Mx)_{i}| & =|\sum_{j}M_{ij}x_{j}|\\
& \leq|\sum_{j}|M_{ij}|^{q}|^{\frac{1}{q}}\cdot\|x\|_{p}\\
& =||M_{ii}|^{q}+\sum_{j\neq i}|M_{ij}|^{q}|^{\frac{1}{q}}\cdot\|x\|_{p}\\
& \leq((1+\frac{1}{\alpha^{q}n^{\frac{q}{p}}})|M_{ii}|^{q})^{\frac{1}{q}}\cdot\|x\|_{p}
\end{align*}
which implies 
\begin{align*}
\|M\|_{p} & \leq(1+\frac{1}{\alpha^{q}n^{\frac{q}{p}}})^{\frac{1}{q}}\cdot n^{\frac{1}{p}}\cdot\max_{i}|M_{ii}|
\end{align*}
On the other hand, for each fixed $x$, let $i$ be the coordinate
such that $|x_{i}|\geq n^{-\frac{1}{p}}\|x\|_{p}$. We know that such
$i$ exists, because otherwise $\sum_{i}|x_{i}|^{p}<\|x\|_{p}^{p}$,
a contradiction. With this $i$, we have
\begin{align*}
|(Mx)_{i}| & \geq|M_{ii}|\cdot|x_{i}|-(\sum_{j\neq i}|M_{ij}|^{q})^{\frac{1}{q}}\cdot(\sum_{j\neq i}|x_{j}|^{p})^{\frac{1}{p}}\\
& \geq|M_{ii}|\cdot|x_{i}|-\frac{1}{\alpha}\cdot n^{-\frac{1}{p}}\cdot|M_{ii}|\cdot(\sum_{j\neq i}|x_{j}|^{p})^{\frac{1}{p}}\\
& \geq|M_{ii}|\cdot n^{-\frac{1}{p}}\|x\|_{p}-n^{-\frac{1}{p}}\frac{1}{\alpha}|M_{ii}|\cdot\|x\|_{p}\\
& \geq n^{-\frac{1}{p}}\cdot(1-\frac{1}{\alpha})|M_{ii}|\cdot\|x\|_{p}
\end{align*}
so that 
\begin{align*}
\frac{\|Mx\|_{p}}{\|x\|_{p}} & \geq(1-\frac{1}{\alpha})\cdot\min_{i}|M_{ii}|
\end{align*}
and so 
\begin{align*}
\|M^{-1}\|_{p} & =\max_{x\neq0}\frac{\|x\|_{p}}{\|Mx\|_{p}}\\
& \leq\frac{1}{(1-\frac{1}{\alpha})}\cdot\frac{1}{\min_{i}|M_{ii}|}
\end{align*}
from which we have 
\begin{align*}
\kappa_{p}(M) & \leq\frac{(1+\frac{1}{\alpha^{q}n^{\frac{q}{p}}})^{\frac{1}{q}}\cdot n^{\frac{1}{p}}}{(1-\frac{1}{\alpha})}\cdot\frac{\max_{i}|M_{ii}|}{\min_{i}|M_{ii}|}
\end{align*}
\end{proof}
%
\end{comment}

\begin{comment}
The above lemmas show that diagonally dominant matrices tend to be
well conditioned. Conversely, our heuristic argument suggested that
if a matrix has a large off-diagonal element, it tends to be ill conditioned.
We specialize these ideas in the following result for correlation
matrices. 
\end{comment}
\begin{comment}
\begin{prop}
\textbf{Let $M$ be a correlation matrix. Suppose $|M_{ij}|\geq\beta$
for some $\beta\in(0,1)$. Then 
\begin{align*}
\kappa(\Sigma_{0}) & \geq
\end{align*}
Conversely, if $|M_{ij}|\leq\gamma$ for some $\gamma\in(0,1)$ and
all $i,j$, then }
\end{prop}
\begin{proof}
\textbf{Let $M=LL^{T}$ be the Cholesky decomposition of $M$, and
let $\ell_{i}$ be the $i$th row of $L$. We have 
\begin{align*}
\geq|\ell_{i}^{T}\ell_{j}|=|\Sigma_{ij}| & \geq\beta\cdot\sqrt{\Sigma_{ii}\Sigma_{jj}}
\end{align*}
}

\textbf{We have 
\begin{align*}
\kappa(D^{\frac{1}{2}}L) & \geq\frac{\max_{i}D_{ii}^{\frac{1}{2}}L_{ii}}{\min_{i}D_{ii}^{\frac{1}{2}}L_{ii}}\\
\end{align*}
and 
\begin{align*}
\kappa(L) & \geq\frac{\max_{i}L_{ii}}{\min_{i}L_{ii}}\\
\end{align*}
}
\end{proof}
\textbf{}
%
\textbf{Is it true that $\kappa(\Sigma)\geq\min(\kappa(\Sigma_{0}),\kappa(D))$???}
\end{comment}

\textbf{}%
\begin{comment}
\textbf{so what we are looking for is a lower bound, that says if
the matrix is not diagonally dominant, then it is ill-conditioned.
This can then be applied to conclude that covariance matrix with columns
of different scales generally is much more ill-conditioned than correlation
matrix. 
\begin{align*}
\frac{\kappa(\Sigma)}{\kappa(D)}\leq\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}) & \leq\kappa(D^{-1})\cdot\kappa(\Sigma)
\end{align*}
and we would like to show 
\begin{align*}
\frac{\kappa(\Sigma)}{\kappa(D)} & \approx\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})
\end{align*}
for a suitable class of matrices $\Sigma$. }
\end{comment}

We shall use the above result to give a sufficient condition on when
the ratio $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}$
is large, i.e. when diagonal preconditioning with column standard
deviation/norm achieves a significant reduction in condition number
with high probability. 

More specifically, we show that if the correlation matrix is diagonally
dominant, then the ratio $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}$
is bounded below by $\frac{1}{p}(\frac{\alpha-1}{\alpha+1})^{2}\kappa(D)$.
\begin{theorem}
	For a covariance matrix $\Sigma$, if $\sqrt{\Sigma_{ii}}\ge\alpha\sum_{j\neq i}|\frac{\Sigma{}_{ij}}{\sqrt{\Sigma_{jj}}}|$,
	then we have 
	\begin{align*}
	\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})} & \geq\frac{1}{p}(\frac{\alpha-1}{\alpha+1})^{2}\kappa(D)
	\end{align*}
	
	\begin{comment}
	\textbf{Conversely, ...}
	\end{comment}
\end{theorem}
\proof{Proof}
	Let $\Sigma_{0}=D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}$. The conditions
	$\sqrt{\Sigma_{ii}}\ge\alpha\sum_{j\neq i}|\frac{\Sigma{}_{ij}}{\sqrt{\Sigma_{jj}}}|$
	imply that $\Sigma_{0}$ is diagonally dominant, so that by the previous
	lemma $\kappa(\Sigma_{0})  \leq p\frac{\alpha+1}{\alpha-1}$ since $\Sigma_{0}$ has diagonal equal to 1. 
	
	The main ingredient of the proof is to use the Cholesky decomposition
	of the correlation matrix and the fact that for a triangular matrix
	$L$, the following condition holds:
	\begin{align*}
	\kappa(L) & \geq\frac{\max_{i}L_{ii}}{\min_{i}L_{ii}}
	\end{align*}
	
	Now let $\Sigma_{0}=L_{0}L_{0}^{T}$ be the Cholesky factorization
	of $\Sigma_{0}$where $L_{0}$ is a lower triangular matrix. It then
	follows that $\Sigma=LL^{T}$ where $L=D^{\frac{1}{2}}L_{0}$ is also
	a lower triangular matrix. We have 
	\begin{align*}
	(\frac{\alpha+1}{\alpha-1})^{2}\cdot\kappa(\Sigma) & =(\frac{\alpha+1}{\alpha-1})^{2}\cdot(\kappa(D^{\frac{1}{2}}L_{0}))^{2} \geq(\frac{\alpha+1}{\alpha-1})^{2}\cdot(\frac{\max_{i}(D^{\frac{1}{2}}L_{0})_{ii}}{\min_{i}(D^{\frac{1}{2}}L_{0})_{ii}})^{2}\\
	& \geq(\frac{\alpha+1}{\alpha-1})^{2}\cdot(\frac{\max_{i}(D^{\frac{1}{2}})_{ii}}{\min_{i}(D^{\frac{1}{2}})_{ii}})^{2}\cdot(\frac{\min_{i}(L_{0})_{ii}}{\max_{i}(L_{0})_{ii}})^{2}\\
	& =(\frac{\alpha+1}{\alpha-1})^{2}\cdot\kappa^{-2}(L_{0})\cdot\kappa^{2}(D^{\frac{1}{2}}) =(\frac{\alpha+1}{\alpha-1})^{2}\cdot\kappa^{-1}(\Sigma_{0})\cdot\kappa(D)\\
	& \geq(\frac{\alpha+1}{\alpha-1})\cdot\kappa(D)\geq\frac{1}{p}\kappa(\Sigma_{0})\cdot\kappa(D)
	\end{align*}
	where we have used the inequality $\|f\cdot g\|_{\infty}\geq\|f\|_{\infty}/\|g^{-1}\|_{\infty}$
	for vectors $f,g\in\mathbb{R}_{++}^{p}$ and $f\cdot g$ is element-wise
	multiplication. 
	
	Rewriting the inequality gives the desired inequality
	\begin{align*}
	\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})} & \geq\frac{1}{p}(\frac{\alpha-1}{\alpha+1})^{2}\kappa(D)
	\end{align*}
	\hfill \Halmos
\endproof
We have thus shown that when the correlation matrix $\Sigma_{0}$
is $\alpha$-diagonally dominant, the ratio of condition numbers $\frac{\kappa(D^{\frac{1}{2}}\Sigma_{0}D^{\frac{1}{2}})}{\kappa(\Sigma_{0})}$
is bounded below by $\frac{1}{p}(\frac{\alpha-1}{\alpha+1})^{2}\kappa(D)$.
For a design matrix with sub-Gaussian rows with covariance matrix
satisfying this condition, the reduction of condition number is on
the order of $\sqrt{\kappa(D)}$ with high probability. \textbf{}%
\begin{comment}
\textbf{It may be possible to relax the conditions $\sqrt{\Sigma_{ii}}\ge\alpha\sum_{j\neq i}|\frac{\Sigma{}_{ij}}{\sqrt{\Sigma_{jj}}}|$
to obtain a similar result for larger class of covariance matrices.
Extend this! }
\end{comment}

\textbf{}%
\begin{comment}
\begin{conjecture}
\textbf{Assume $\Sigma$ is positive definite and there exists $0<\alpha<1$
such that for all (or just some?) $i$, there exists some $j$ with
\begin{align*}
|\Sigma_{ii}| & <\alpha|\Sigma_{ij}|
\end{align*}
}

\textbf{then we have }

\textbf{
\begin{align*}
\kappa(\Sigma) & \geq\frac{1+\alpha}{1-\alpha}\cdot\frac{\max_{i}|\Sigma_{ii}|}{\min_{i}|\Sigma_{ii}|}
\end{align*}
}
\end{conjecture}
\textbf{}
%
\textbf{Claim: If $|a_{ii}|<\alpha|a_{ij}|$ for $j\neq i$ and all
$i$, where $\alpha\in(0,1)$, then 
\begin{align*}
\kappa(\begin{pmatrix}a_{11} & a_{12} & \dots\\
a_{21}\\
\dots
\end{pmatrix}) & \geq\kappa(\begin{pmatrix}a_{11} & \frac{1}{\alpha}a_{11} & \dots\\
\frac{1}{\alpha}a_{11}\\
\\
\\
\end{pmatrix})\\
& =\frac{1+\alpha}{1-\alpha}\kappa(\begin{pmatrix}a_{11}\\
& \dots\\
\\
&  & a_{n}
\end{pmatrix})
\end{align*}
First note 
\begin{align*}
\kappa(\begin{pmatrix}a_{11} & \frac{1}{\alpha}a_{11}\\
\frac{1}{\alpha}a_{22} & a_{22}
\end{pmatrix}) & =\frac{1+\frac{1}{\alpha}}{}\\
\end{align*}
}
\end{comment}

==> dsdp-old.tex <==
\section{Optimal Preconditioning via Dual SDP}
\label{sec:DSDP}
In this section, we propose a practical approach to efficiently find optimal diagonal preconditioners via solving a dual SDP problem. Although the theoretical computational complexity of this DSDP approach is higher than the potential reduction algorithm, in practice, we are able to find optimal diagonal preconditioners for matrices with size $\sim$5000 within reasonable time, using a customized DSDP solver \textbf{add reference here}. We will explore in depth the empirical performance of the DSDP approach on matrices from the SuiteSparse Collection. 

\subsection{A Dual SDP Formulation of Optimal Preconditioning}

Recall the optimal diagonal preconditioning problem given a PD matrix $M$:
\begin{align*}
\min_{\kappa,D}\kappa\\
s.t.M\succeq D\\
\kappa D\succeq M\\
D\succeq0
\end{align*}
Due to the fact that $\kappa$ and $D$ are both variables, this problem is not in standard SDP form. However, there is a simple way to transform it into an SDP problem. Specifically, we can do a change of variables $\kappa\rightarrow1/\kappa$ to obtain
\begin{align*}
\max_{(\tau,d)}\tau\\
s.t.D-M\preceq0\\
\tau M-D\preceq0
\end{align*}
 which is in standard dual SDP form, with $D$ the diagonal matrix
with $d$ on the diagonal. 

Note that a feasible solution for this SDP is $(\tau, d) = (-1, \mathbf{0})$, and although the optimal objective value is always positive, using this feasible solution as a starting point in the DSDP solver can lead to significant improvements. Moreover, for very ill-conditioned matrices with the minimum eigenvalue $\lambda_{\min}$ close to 0, we propose to use the initialization $(\tau, d) = (-1/\delta, \mathbf{0})$ for $\delta=O(\lambda_{\min})$ to further improve the stability of the DSDP solver.

\subsection{HDSDP: A Customized DSDP Solver}

Here can include a brief introduction to the HDSDP solver.

\subsection{Empirical Performance on SuiteSpare Matrices}
Here can consider reporting the following metrics:

\begin{itemize}
    \item Clock Time
    \item Suboptimality Gap vs. Iteration
    \item Reduction in Condition Number
\end{itemize}

==> experiments-old.tex <==
\section{Numerical Experiments}
\label{sec:experiments}

In this section, we perform numerical experiments to compare the performance
of diagonal preconditioning methods at accelerating gradient and stochastic
gradient descent applied to regression and classification problems. 

\subsection{Simulated Dataset}

For our simulated dataset, we randomly generate design matrix $X$
whose rows are i.i.d. Gaussian vectors with covariance matrix $\Sigma$.
The covariance matrix itself is generated using the sklearn package
in python, and has condition numbers in the range of 100-1000. We
consider the regression problem 
\begin{align*}
\min_{\theta}\frac{1}{n}\|X\theta-Y\|_{2}^{2}
\end{align*}
where $Y$ is generated using a ground-truth parameter $\theta^{\ast}$,
and we assess the speed of convergence by looking at the distance
of estimate to the optimal solution of the quadratic problem, namely
the OLS estimate $\theta_{OLS}$ of $\theta$: we declare convergence
when $\|\theta^{(k)}-\theta_{OLS}\|_{2}/\|\theta_{OLS}\|_{2}$ is
below some threshold, usually set to be $0.01$. 

We consider the following modified problem 
\begin{align*}
\min_{\tilde{\theta}}\frac{1}{n}\|XD\tilde{\theta}-D_{0}Y\|_{2}^{2}
\end{align*}
where $D$ is one of the following diagonal preconditioners: 
\begin{itemize}
	\item Normalization: $D$ is the diagonal matrix of column standard deviations
	or norms of $X$.
	\item Optimal diagonal preconditioning: $D$ minimizes $\kappa(DX^{T}XD)$
	among all positive diagonal matrices.
	\item (full) Batch normalization: $D_{0}=I$, and $D_{1}^{(0)}$ is the
	diagonal matrix of column standard deviations of $X$. At the $k$th
	iteartion, update $\theta^{(k+1)}$ by solving $\min_{\theta}\frac{1}{n}\|XD^{(k)}\theta-y\|_{2}^{2}$
	and then form $D_{1}^{(k+1)}$ by solving $\min_{D}\frac{1}{n}\|XD\theta^{(k+1)}-y\|_{2}^{2}$.
\end{itemize}
We compare the convergence speeds of gradient and stochastic gradient
descent methods with these preconditioners. Step size is determined
by backtracking line search using the Armijo-Goldstein conditions.

For stochastic gradient descent, since $X$ is not directly available,
we use the corresponding adaptive versions of the above procedures:

\begin{comment}
\begin{itemize}
\item Optimal diagonal preconditioning: $D_{0}=I$ and $D_{1}$ minimizes
$\kappa(DX^{T}XD)$.
\item Normalization: $D_{0}=I$ and $D_{1}$ is the diagonal matrix of column
standard deviations of $X$
\item Matrix equilibriation: $D_{0}^{-1}=\text{diag}(\sum_{j}|X_{1j}|,\dots,\sum_{j}|X_{nj}|)$,
$D_{1}^{-1}=\text{diag}(\sum_{i}|(D_{0}X)_{i1}|,\dots,\sum_{i}|(D_{0}X)_{ip}|)$.
\item (full) Batch normalization: $D_{0}=I$, and $D_{1}^{(0)}$ is the
diagonal matrix of column standard deviations of $X$. At the $k$th
iteartion, update $\theta^{(k+1)}$ by solving 
\begin{align*}
& \min_{\theta}\frac{1}{n}\|XD^{(k)}\theta-y\|_{2}^{2}
\end{align*}
and then form $D_{1}^{(k+1)}$ by solving
\begin{align*}
& \min_{D}\frac{1}{n}\|XD\theta^{(k+1)}-y\|_{2}^{2}
\end{align*}
\end{itemize}
\end{comment}
%
\begin{itemize}
	\item Normalization: $D$ is the diagonal matrix of column standard deviations
	or norms of $X^{(k)}$, the batch of data in the $k$-th iteration.
	\item Adaptive optimal diagonal preconditioning: at $k$th iteration, form
	the cumulative design matrix $\overline{X}^{(k)}$ by concatenating
	$X^{(k)}$ with $\overline{X}^{(k-1)}$ and retaining unique rows,
	and find $D$ that minimizes $\kappa(D(\overline{X}^{(k)T}\overline{X}^{(k)}D)$.
	\item Batch normalization: $D^{(0)}=I$. At the $k$th iteartion, update
	$\theta^{(k+1)}$ by solving $\min_{\theta}\frac{1}{n}\|X^{(k)}D^{(k)}\theta-y\|_{2}^{2}$
	and then form $D^{(k+1)}$ by solving $\min_{D}\frac{1}{n}\|X^{(k)}D\theta^{(k+1)}-y\|_{2}^{2}$
	where $X^{(k)}$ is the batch of samples at the $k$th iteration. 
\end{itemize}
Tables \ref{tab:iterations_gd} and \ref{tab:iterations_sgd} summarize
the number of iterations before convergence for various methods and
problems of various sizes. We note that in many cases the optimal
diagonal preconditioner returns a preconditioned matrix with significantly
smaller condition number, as guaranteed by our theoretical analyses.
This is also manifested through the acceleration in convergence of
steepest descent. On the other hand, preconditioning with column statistics
does not always guarantee reduction in condition number. In general,
steepest descent with optimal diagonal preconditioning achieves comparable
performance to batch normalization when it performs well. On the other
hand, there are specific cases where stochastic gradient descent with
batch normalization takes considerably longer time than optimal preconditioning.
The tradoff here is that for large matrices ($p$ large), finding
an approximate optimal diagonal preconditioner may take a non-negligible
amount of time, whereas batch normalization only adds one extra step
of gradient update for the preconditioner $D$. The numerical simulations
also confirm that although batch normalization speeds up first order
optimization methods, the effective condition number of the design
matrix is not actually decreased. This suggests that although the
performance of batch normalization is comparable to that of optimal
diagonal preconditioning, the exact mechanism through which it speeds
up convergence remains to be investigated further. 

\begin{table}
	\begin{centering}
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline 
			$(n,p)$ & \multicolumn{2}{c|}{$(1000,20)$} & \multicolumn{2}{c|}{$(1000,40)$} & \multicolumn{2}{c|}{$(1000,100)$}\tabularnewline
			\hline 
			& iterations & $\kappa$ & iterations & $\kappa$ & iterations & $\kappa$\tabularnewline
			\hline 
			No preconditioning & 44529 & 278.30 & 39709 & 870.81 & 72795 & 1129.80\tabularnewline
			\hline 
			Fixed preconditioning & 16639 & 230.36 & 148954 & 909.80 & 62915 & 1087.84\tabularnewline
			\hline 
			Optimal preconditioning & 10230 & 144.81 & 29835 & 746.99 & 29881 & 858.46\tabularnewline
			\hline 
			Batch normalization & 11721 & 470.12 & 31032 & 1226.79 & 47654 & 1192.45\tabularnewline
			\hline 
		\end{tabular}
		\par\end{centering}
	\caption{\label{tab:iterations_gd}Number of iterations till convergence for
		preconditioning methods for gradient descent, with step size determined
		through backtracking line search. Convergence is declared when $\|\theta-\theta^{\ast}\|$
		is within a small constant factor of $\|\theta^{\ast}\|$, where $\theta^{\ast}$
		is the OLS solution, and $\theta$ is the effective coefficient taking
		into account the preconditioning on $X$. The covariance matrix $\Sigma$
		is randomly generated using python package sklearn and the condition
		number of the effective design matrix $X\sim\mathcal{N}(0,\Sigma)$
		is also reported above as $\kappa$. For example, for preconditioning
		with diagonal matrix $D$, the condition number of $XD$ is given.
		For batch normalization, since the condition number of the effective
		deisgn matrix changes every iteration, the median of those numbers
		are given. We see that preconditioning with column standard deviation
		does not always reduce the condition number of the design matrix,
		and indeed in such cases convergence of steepest descent is slowed
		down. }
\end{table}

\begin{table}
	\begin{centering}
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline 
			$(n,p)$ & \multicolumn{2}{c|}{$(1000,20)$} & \multicolumn{2}{c|}{$(1000,40)$} & \multicolumn{2}{c|}{$(1000,100)$}\tabularnewline
			\hline 
			& iterations & $\kappa$ & iterations & $\kappa$ & iterations & $\kappa$\tabularnewline
			\hline 
			No preconditioning & 12350 & 166.53 & 43712 & 986.51 & 96619 & 1637.54\tabularnewline
			\hline 
			Fixed preconditioning & 11825 & 140.86 & 100547 & 1149.97 & 54646 & 1594.44\tabularnewline
			\hline 
			Optimal preconditioning & 10791 & 126.07 & 31202 & 868.13 & 47310 & 1313.44\tabularnewline
			\hline 
			Batch normalization & 11189 & 251.85 & 35999 & 1280.45 & 48448 & 2012.47\tabularnewline
			\hline 
		\end{tabular}
		\par\end{centering}
	\caption{\label{tab:iterations_sgd}Number of iterations till convergence for
		adaptive preconditioning methods for mini-batch stochastic gradient
		descent, with step size determined through backtracking line search.
		Batch size is between 10-20\% of the training set size. The last two
		preconditioning methods, i.e. optimal preconditioning and batch normalization,
		are adaptive, whereas the first two only requires preconditioning
		once before the start of the optimization routine. For adaptive optimal
		diagonal preconditioning, the diagonal preconditioner is updated once
		every 100 iterations, using the most up to date cumulative design
		matrix. All reported condition numbers are medians of the sequence
		of condition numbers of the effective design matrix during training. }
\end{table}

\subsection{MNIST Dataset}

To compare the preconditioning procedures on a real dataset, we use
the MNIST handwritten digit classification dataset, consisting of
70000 handwritten digits in the format of $28\times28$ binary pixel
photos, with a train-validation split of $6:1$. As a preprocessing
step, we reshape each two-dimensional datapoint into a $784$-dimensional
vector. As the design matrix is rank-deficient due to linear dependency
and duplicate rows, we select the subset of linearly independent columns,
and also perturb the entries with iid Gaussian noise with standard
deviation 0.01. The resulting design matrix has a condition number
of $73288.03$, i.e. a very ill-conditioned system. Applying the optimal
diagonal preconditioner yields a design matrix with condition number
$102.27$, a significant reduction. To assess the convergence speeds
of gradient and stochastic gradient descent methods, we run multinomial
logistic regression with cross-entropy loss, $f(\theta)=\frac{1}{n}\sum_{i=1}^{n}-\log p_{i}^{y_{i}}$
where $p_{i}^{k}$ is the probability of the $k$-th class of the
$i$th sample, predicted by the model: $p_{i}^{k}=\frac{\exp(\theta_{k}^{T}x_{i})}{\sum_{k=1}^{K}\exp(\theta_{k}^{T}x_{i})}$,
with the descent direction given by $\nabla_{\theta_{k}}f(\theta)=-\frac{1}{n}\sum_{y_{i}=k}x_{i}+\frac{1}{n}\sum_{i}\frac{x_{i}\exp(\theta_{k}^{T}x_{i})}{\sum_{k=1}^{K}\exp(\theta_{k}^{T}x_{i})}$.

Because the problem is non-convex, we declare convergence when the
number of iterations reached a maximum value, or when the norm of
gradient drops below the threshold $0.001$. We then report the log-gap
$\log(f(\theta)-f(\theta^{\ast}))$ of the various methods, where
$\theta^{\ast}$ is a pre-computed optimal solution. 

\begin{table}
	\begin{centering}
		\begin{tabular}{|c|c|c|}
			\hline 
			$(n,p)$ & \multicolumn{1}{c|}{iterations} & \multicolumn{1}{c|}{log-gap}\tabularnewline
			\hline 
			No preconditioning & 2000 & -2.74\tabularnewline
			\hline 
			Fixed preconditioning & 1823 & -2.90\tabularnewline
			\hline 
			Optimal preconditioning & 1503 & -3.12\tabularnewline
			\hline 
			Batch normalization & 1621 & -3.35\tabularnewline
			\hline 
		\end{tabular}
		\par\end{centering}
	\caption{Number of iterations till convergence of diagonal preconditioning
		methods for gradient descent and the log-gap at convergence. We see
		that while the log-gaps are comparable among the three diagonal conditioners,
		the number of iterations required is the smallest for optimal diagonal
		preconditioner. }
\end{table}
We see that while the log-gaps are comparable among the three diagonal
conditioners, the number of iterations required till convergence is
the smallest for optimal diagonal preconditioner. All methods are
able to achieve a test accuracy of at least 88\%. 

\section{Conclusion}

In this paper, we studied diagonal preconditioning and its impact
on the condition number and convergence speed of linear systems and
quadratic and general convex optimization problems. We first showed
that the popular preconditioning technique of normalization by column
standard deviation/norm reduces the condition number of the design
matrix $X$ by $\sqrt{\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}}$
for $X$ with independent sub-Gaussian rows and convariance matrix
$\Sigma$, where $D=\text{diag}(\Sigma)$. We then gave a diagonal
dominance condition that guarantees that this reduction is large.
Next, for any fixed design matrix, we developed bisection and interior
point algorithms that guarantee a diagonal preconditioner that reduces
the condition number of the preconditioned matrix, with $O(\frac{1}{\epsilon})$
iteration complexity, and each iteration consists of an SDP feasibility
problem or a Newton update step with Nesterov-Todd directions. These
results have direct implications for the effect of preconditioning
on speeding up the convergence of iterative algorithms for linear
systems and first order methods for quadratic optimization problems,
as the linear convergence rates have explicit dependence on the condition
number. For general convex optimization problems, it is less clear
how improvements in the condition number of the design matrix translate
into speedup of first order methods. We showed that for a particular
class of strongly convex and smooth objectives, the reduction in the
condition number of the objective function enjoys the same order $\sqrt{\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}}$
of reduction as that of the design matrix. Finally, we established
connections of batch normalization to adaptive preconditioning, and
extended our optimal diagonal preconditioning algorithm to an adaptive
setting compatible with stochastic first order methods. Numerical
experiments on real and simulated datasets with regression and classification
tasks show that the optimal diagonal preconditioner speeds up convergence
compared to preconditioning with heuristics such as column standard
deviation, and is comparable to the performance of batch normalization.
On the other hand, batch normalization does not seem to reduce the
effective condition number of the system, so its mechanism of speeding
up convergence remains to be investigated further. 

==> major revision/concentration.tex <==
\section{Diagonal Preconditioning and Reduction in Condition Number}
\label{sec:concentration}


In this section, we study the problem of when applying the diagonal
preconditioning method with normalization by column norm is effective
at reducing the condition number. When applying such methods, the
matrix being transformed is often a data or design matrix with i.i.d.
rows drawn from some common distribution. In this case the condition
number can also be viewed as a random variable. We first use matrix
concentration to show that with high probability, the reduction of
condition number using column normalization is close to that achieved
by transforming the population covariance matrix to the population
correlation matrix. Then we give sufficient conditions on when the
corresponding procedure on the population covariance matrix reduces
condition number significantly.

\subsection{Concentration of Condition Numbers}

We consider the setting where each row of the $n\times p$ design
matrix $X$ is an i.i.d. observation of a $p$-dimensional sub-Gaussian
vector. We are interested in how the procedure of normalizing by column
norm/standard deviation affects the condition number of the design
matrix. Because the condition number is a random variable in this
setting, we would like to simplify the analysis by first proving that
it concentrates around the condition number of population parameters
with high probability, from which we can conclude how much the condition
number can be reduced with this procedure. 

For ease of presentation, we assume for now that the sub-Gaussian
vector has mean zero and covariance matrix $\Sigma$. One of the most
common diagonal preconditioning procedures is to normalize each column
of $X$ by its mean or standard deviation. Thus we first analyze the
concentration behavior of the condition number under this particular
diagonal preconditioning, which takes the form 
\begin{align*}
X_{0} & =XD^{-\frac{1}{2}}
\end{align*}
where $D$ is the diagonal matrix with 
\begin{align*}
D_{jj} & =\frac{1}{n-1}\sum_{i=1}^{n}(X_{ij}-\mu_{j})^{2}\\
\mu_{j} & =\frac{1}{n}\sum_{i=1}^{n}X_{ij}\text{ or }\mu_{j}\equiv0
\end{align*}
corresponding to column variance or norm squared. 

We recall the definition of sub-Gaussian random vectors and some results
from matrix concentration and analysis that are useful in the proof
of our main result. 
\begin{definition}
	Define the sub-Gaussian norm of a random variable $x$ to be 
	\begin{align*}
	\|x\|_{\psi_{2}} & =\sup_{p\geq1}p^{-1/2}(\mathbb{E}|x|^{p})^{1/p}
	\end{align*}
	and the sub-Gaussian norm of a random vector $X\in\mathbb{R}^{n}$
	to be 
	\begin{align*}
	\|X\|_{\psi_{2}} & =\sup_{x\in S^{n-1}}\|\langle X,x\rangle\|_{\psi_{2}}
	\end{align*}
	
	Equivalently, the sub-Gaussian norm of $X$ is given by the smallest
	$K$ such that
	\begin{align*}
	\mathbb{E}\left[\exp(s\cdot u^{T}X)\right] & \leq\exp(K^{2}s^{2}/2),\forall s\in\mathbb{R},\|u\|=1
	\end{align*}
\end{definition}
\begin{lemma}
	(sub-Gaussian matrix concentration \cite{rudelson2010non} \label{lem:sub-Gaussian-concentration})
	Let $X$ be an $n\times p$ random matrix with $n>p$ and i.i.d sub-Gaussian
	rows $X_{i}$ with sub-Gaussian norm $K=\|X_{i}\|_{\psi_{2}}$ and
	$\Sigma=\mathbb{E}X_{i}^{T}X_{i}=\frac{1}{n}\mathbb{E}X^{T}X$ its
	second moment matrix. Then with probability at least $1-2\exp(-\frac{ct^{2}}{K^{4}})$,
	\begin{align*}
	\|\frac{1}{n}X^{T}X-\Sigma\|_{op} & \leq\max(\delta,\delta^{2})\\
	\delta & =CK^{2}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}
	\end{align*}
	where $c$ and $C$ are universal constants. Moreover, the above
	also implies
	\begin{align*}
	\sqrt{n}-(CK^{2})\sqrt{p}-t\leq\sigma_{\min}(X)\leq\sigma_{\max}(X) & \leq\sqrt{n}+(CK^{2})\sqrt{p}+t
	\end{align*}
\end{lemma}
%
\begin{lemma}
	(Weyl inequality \label{lem:weyl}) Let $\lambda_{i}(X)$ be the $i$-th
	eigenavlue of a self-adjoint matrix $X$. Then 
	\begin{align*}
	|\lambda_{i}(X)-\lambda_{i}(Y)| & \leq\|X-Y\|_{op}
	\end{align*}
	for all $i$. In other words, the eigenvalue map is 1-Lipschitz on
	the space of self-adjoint matrices with respect to the metric induced
	by the operator norm.
\end{lemma}
Our main result is that the condition number of $X_{0}^{T}X_{0}$
where $X=X_{0}D^{-\frac{1}{2}}$ concentrates around that of $D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}$,
where $D$ is the diagonal of $\Sigma$, i.e. $D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}$
is the population correlation matrix. Since $\kappa(X_{0}^{T}X_{0})=\kappa(X_{0})^{2}$,
this implies that $\frac{\kappa(X)}{\kappa(X_{0})}$ is on the order
of $\frac{\sqrt{\kappa(\Sigma)}}{\sqrt{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}}$
with high probability. 
\begin{theorem}
	\label{thm:concentration_1}Let $X$ be an $n\times p$ random matrix
	with $n>p$ and i.i.d. sub-Gaussian rows $X_{i}$ with $K=\|X_{i}\|_{\psi_{2}}$
	the sub-Gaussian norm of its rows, $\mathbb{E}X_{i}=0$, and let $\Sigma=\mathbb{E}X_{i}^{T}X_{i}=\frac{1}{n}\mathbb{E}X^{T}X$
	be the population covariance matrix. Let $\hat{D}$ be the diagonal
	matrix with $\hat{D}_{ii}=(X^{T}X)_{ii}$, i.e. $\hat{D}_{ii}$ is
	the norm squared of the $i$-th column of $X$, and let $X_{0}:=X\hat{D}^{-\frac{1}{2}}$
	be the matrix normalized with diagonal entries of $\hat{D}$. Then
	with probability at least $1-2\exp(-\frac{ct^{2}(\min_{i}(\Sigma)_{ii})^{2}}{K^{4}})-2\exp(-\frac{ct^{2}}{K^{4}})-2p\exp(-\frac{c}{K^{4}}\left[K^{2}+\frac{\min_{i}(\Sigma)_{ii}}{\sqrt{p}}\cdot t\right]^{2})$,
	we have
	\begin{align*}
	|\frac{\kappa(X^{T}X)}{\kappa(\Sigma)}- & \frac{\kappa(X_{0}^{T}X_{0})}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}|\leq\frac{2}{(1-(CK^{2})\sqrt{\frac{p}{n}}-\frac{t}{\sqrt{n}})^{2}}\cdot\left[CK^{2}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}\right]\\
	& +\frac{2}{(1-(C\frac{K^{2}}{\min_{i}(\Sigma)_{ii}})\sqrt{\frac{p}{n}}-3\frac{t}{\sqrt{n}})^{2}}\cdot\left[C\frac{K^{2}}{\min_{i}(\Sigma)_{ii}}\sqrt{\frac{p}{n}}+3\frac{t}{\sqrt{n}}\right]
	\end{align*}
\end{theorem}
\proof{Proof}
	See the appendix.\textbf{}%
	\begin{comment}
	\textbf{Note: dependence on $p$ may be refined. Refine it!}
	\end{comment}
	\hfill \Halmos
\endproof
\begin{comment}
\begin{proof}
Since the rows of $X$ are independent, its columns are sub-Gaussian
vectors with independent entries with sub-Gaussian norm bounded above
by $K$. Standard concentration result of the norm implies that with
probability at least $1-2\exp(-\frac{cT^{2}}{K^{4}})$, 
\begin{align*}
|\hat{D}_{ii}^{\frac{1}{2}}-D_{ii}^{\frac{1}{2}}| & \leq T
\end{align*}
for all large $T$. Union bound then gives that with probability
at least $1-2p\exp(-\frac{cT^{2}}{K^{4}})$, 
\begin{align*}
|\hat{D}_{ii}^{\frac{1}{2}}-D_{ii}^{\frac{1}{2}}| & \leq T,\forall i
\end{align*}
so that 
\begin{align*}
|\frac{\hat{D}_{ii}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}}-1| & \leq T\frac{1}{\sqrt{\min_{i}(\Sigma)_{ii}}}
\end{align*}
For any $i,j$, we have 
\begin{align*}
|\hat{D}_{ii}^{-\frac{1}{2}}X_{i}^{T}X_{j}\hat{D}_{jj}^{-\frac{1}{2}}-D_{ii}^{-\frac{1}{2}}X_{i}^{T}X_{j}D_{jj}^{-\frac{1}{2}}| & \leq\|X_{i}^{T}\|_{2}\|X_{j}^{T}\|_{2}|\hat{D}_{ii}^{-\frac{1}{2}}\hat{D}_{jj}^{-\frac{1}{2}}-D_{ii}^{-\frac{1}{2}}D_{jj}^{-\frac{1}{2}}|\\
& =|\hat{D}_{ii}^{\frac{1}{2}}\hat{D}_{jj}^{\frac{1}{2}}|\cdot|\hat{D}_{ii}^{-\frac{1}{2}}\hat{D}_{jj}^{-\frac{1}{2}}-D_{ii}^{-\frac{1}{2}}D_{jj}^{-\frac{1}{2}}|\\
& =|1-\frac{\hat{D}_{ii}^{\frac{1}{2}}\hat{D}_{jj}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}D_{jj}^{\frac{1}{2}}}|\\
& =|1-\frac{\hat{D}_{ii}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}}+\frac{\hat{D}_{ii}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}}-\frac{\hat{D}_{ii}^{\frac{1}{2}}\hat{D}_{jj}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}D_{jj}^{\frac{1}{2}}}|\\
& \leq|1-\frac{\hat{D}_{ii}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}}|+|\frac{\hat{D}_{ii}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}}-\frac{\hat{D}_{ii}^{\frac{1}{2}}\hat{D}_{jj}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}D_{jj}^{\frac{1}{2}}}|\\
& \leq T\frac{1}{\sqrt{\min_{i}(\Sigma)_{ii}}}(1+\frac{\hat{D}_{ii}^{\frac{1}{2}}}{D_{ii}^{\frac{1}{2}}})\\
& \le2\frac{T^{2}}{\min_{i}(\Sigma)_{ii}}
\end{align*}
for all large $T$. 

The relation between operator norm and maximum entry of a matrix $A$,
$\|A\|_{op}\leq\sqrt{np}\cdot\max_{i,j}|A_{ij}|$ then implies that 

\begin{align*}
\|\frac{1}{n}D^{-\frac{1}{2}}X^{T}XD^{-\frac{1}{2}}-\frac{1}{n}\hat{D}^{-\frac{1}{2}}X^{T}X\hat{D}^{-\frac{1}{2}}\|_{op} & \leq\sqrt{np}\cdot\frac{1}{n}\max_{i,j}|\hat{D}_{ii}^{-\frac{1}{2}}X_{i}^{T}X_{j}\hat{D}_{jj}^{-\frac{1}{2}}-D_{ii}^{-\frac{1}{2}}X_{i}^{T}X_{j}D_{jj}^{-\frac{1}{2}}|\\
& \leq2\frac{T^{2}}{\min_{i}(\Sigma)_{ii}}\cdot\sqrt{\frac{p}{n}}
\end{align*}

Now recall the result from Theorem 5, that with probability at least
$1-2\exp(-\frac{ct^{2}(\min_{i}(\Sigma)_{ii})^{2}}{K^{4}})-2\exp(-\frac{ct^{2}}{K^{4}})$,
the following two inequalities hold simultaneously
\begin{align*}
\|\frac{1}{n}D^{-\frac{1}{2}}X^{T}XD^{-\frac{1}{2}}-D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}\|_{op} & \leq C\frac{K^{2}}{\min_{i}(\Sigma)_{ii}}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}\\
\|\frac{1}{n}X^{T}X-\Sigma\|_{op} & \leq CK^{2}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}
\end{align*}
Now choose $T$ such that $T^{2}=K^{2}+\frac{\min_{i}(\Sigma)_{ii}}{\sqrt{p}}\cdot t$,
we see that 
\begin{align*}
\|\frac{1}{n}D^{-\frac{1}{2}}X^{T}XD^{-\frac{1}{2}}-\frac{1}{n}\hat{D}^{-\frac{1}{2}}X^{T}X\hat{D}^{-\frac{1}{2}}\|_{op} & \leq2\frac{K^{2}}{\min_{i}(\Sigma)_{ii}}\cdot\sqrt{\frac{p}{n}}+2\frac{t}{\sqrt{n}}
\end{align*}
so that 
\begin{align*}
\|\frac{1}{n}\hat{D}^{-\frac{1}{2}}X^{T}X\hat{D}^{-\frac{1}{2}}-D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}\|_{op} & \leq C\frac{K^{2}}{\min_{i}(\Sigma)_{ii}}\sqrt{\frac{p}{n}}+3\frac{t}{\sqrt{n}}\\
\|\frac{1}{n}X^{T}X-\Sigma\|_{op} & \leq CK^{2}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}
\end{align*}
and eigenvalue stability result allows us to conclude that 
\begin{align*}
|\frac{\kappa(X^{T}X)}{\kappa(\Sigma)}-\frac{\kappa(X_{0}^{T}X_{0})}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}| & \leq\frac{2}{(1-(CK^{2})\sqrt{\frac{p}{n}}-\frac{t}{\sqrt{n}})^{2}}\cdot\left[CK^{2}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}\right]\\
& +\frac{2}{(1-(C\frac{K^{2}}{\min_{i}(\Sigma)_{ii}})\sqrt{\frac{p}{n}}-3\frac{t}{\sqrt{n}})^{2}}\cdot\left[C\frac{K^{2}}{\min_{i}(\Sigma)_{ii}}\sqrt{\frac{p}{n}}+3\frac{t}{\sqrt{n}}\right]
\end{align*}
with probability at least 
\begin{align*}
1-2\exp(-\frac{ct^{2}(\min_{i}(\Sigma)_{ii})^{2}}{K^{4}})-2\exp(-\frac{ct^{2}}{K^{4}})-2p\exp(-\frac{c}{K^{4}}\left[K^{2}+\frac{\min_{i}(\Sigma)_{ii}}{\sqrt{p}}\cdot t\right]^{2})
\end{align*}
\end{proof}
\end{comment}
%
If we assume that the diagonal of $\Sigma$ is lower bounded, we can
further simplify the bound. 
\begin{corollary}
	Same assumptions as the previous theorem, and additionally $\min_{i}(\Sigma)_{ii}\geq1$.
	Then 
	\begin{align*}
	|\frac{\kappa(X^{T}X)}{\kappa(\Sigma)}- & \frac{\kappa(X_{0}^{T}X_{0})}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}|\leq\frac{6}{(1-(CK^{2})\sqrt{\frac{p}{n}}-3\frac{t}{\sqrt{n}})^{2}}\cdot\left[CK^{2}\sqrt{\frac{p}{n}}+\frac{t}{\sqrt{n}}\right]
	\end{align*}
	with probability at least 
	\begin{align*}
	1-4\exp(-\frac{ct^{2}}{K^{4}})-2p\exp(-\frac{c}{K^{4}}\left[K^{2}+\frac{t}{\sqrt{p}}\right]^{2})
	\end{align*}
\end{corollary}
It is straightforward to extend these results to the case of sub-Gaussian
matrices with independent rows and non-zero mean. The above results
imply that with high probability, the ``reduction'' in condition
number of a sub-Gaussian design matrix with column normalization is
on the order of $\sqrt{\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}}$.
Therefore we can shift the focus of our analysis to the problem of
comparing the condition numbers of population covariance and correlation
matrices. 

\textbf{Proof Strategy} Because the scaling matrix $D=\hat{D}$ is
a function of sample statistics, namely the column-wise sample standard
deviations or column norm, the analysis with $\hat{D}$ directly is
cumbersome. Our strategy for showing the main result is to start with
the simplest possible case for $D$ and gradually increase the complexity
of the scaling matrix. More precisely, we show a sequence of concentration
results, each one built on top of the other, with the following scaling
matrices:
\begin{itemize}
	\item $D$ is equal to the population covariance matrix $\Sigma$, with
	general non-diagonal $\Sigma$.
	\item $D$ is the sample column-wise standard deviation, under the assumption
	that $\Sigma$ is diagonal. 
	\item $D$ is the diagonal of the population covariance matrix, with general
	non-diagonal $\Sigma$.
	\item $D$ is the sample standard deviation, with general non-diagonal $\Sigma$. 
\end{itemize}
For details of the proof, see the appendix. 

\begin{remark}
	The diagonal preconditioning considered in the above results is widely
	used in practice. It is common knowledge that when variables have
	different scales, the condition number of the design matrix (whose
	columns correspond to variables) tends to be large. This can be alleviated
	by rescaling the columns of the design matrix by its norm, so that
	each column has norm 1. This procedure does not guarantee, however,
	that there is always a significant reduction in condition number.
	In the next subsection, we study conditions under which such a procedure
	does result in a significant reduction in condition number, or equivalently
	that $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}\gg1$. 
	
	\begin{comment}
	\begin{rem}
	We have shown that diagonal pre-conditioning with batch standard deviations
	yields matrices with condition numbers close to the population correlation
	matrix. The next question is then: When does a covariance matrix have
	a much larger condition number than its corresponding correlation
	matrix. 
	
	The condition number of a correlation matrix and a covariance matrix
	are related in the following way. Let $\Sigma_{0}$ be a correlation
	matrix, and let $\Sigma_{0}=LL^{T}$ be the Cholesky decomposition
	of $\Sigma$ with $L$ a lower triangular matrix. Then 
	\begin{align*}
	\kappa(\Sigma_{0}) & =\kappa^{2}(L)=\kappa^{2}(L^{T})
	\end{align*}
	and 
	\begin{align*}
	\kappa(D^{\frac{1}{2}}\Sigma_{0}D^{\frac{1}{2}}) & =\kappa^{2}(L^{T}D^{\frac{1}{2}})=\kappa^{2}(D^{\frac{1}{2}}L)
	\end{align*}
	Because $\Sigma_{0}$ is a correlation matrix, the diagonal entries
	of $L$ have norm bounded above by 1. If the spectrum of $D$ satisfy
	$\sigma_{\max}(D^{\frac{1}{2}})\cdot\sigma_{\min}(L)\gg1$, then
	\begin{align*}
	\kappa(D^{\frac{1}{2}}L) & \approx\kappa(D^{\frac{1}{2}})\cdot\kappa(L)
	\end{align*}
	
	\textbf{(Need to write formal analysis of the statement)}
	
	The Cholesky factorization also tells us when a correlation matrix
	is ill-conditioned. Consider $LL^{T}$, with the condition that the
	norm of every column is 1. Then the off diagonal of $LL^{T}$ is large
	if and only if the corresponding diagonal of $L$ is small (so that
	the mass of that row is concentrated on the off-diagonal), i.e. $L$
	is ill-conditioned. 
	
	So the condition number of a covariance matrix is largely dependent
	on the scale difference between the largest standard deviation and
	smallest standard deviation. If the diagonal matrix with standard
	deviations is ill-conditioned, so will be the covariance matrix.
	
	Assume $U$ is square invertible with $|u_{ii}|\ge\alpha\sum_{j\neq i}|u_{ij}|\geq0$,
	then 
	\begin{align*}
	\kappa(U) & \leq\frac{\alpha+1}{\alpha-1}\cdot\frac{\max_{i}|u_{ii}|}{\min_{i}|u_{ii}|}
	\end{align*}
	so what we are looking for is a lower bound, that says if the matrix
	is not diagonally dominant, then it is ill-conditioned. This can then
	be applied to conclude that covariance matrix with columns of different
	scales generally is much more ill-conditioned than correlation matrix.
	\begin{align*}
	\frac{\kappa(\Sigma)}{\kappa(D)}\leq\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}) & \leq\kappa(D^{-1})\cdot\kappa(\Sigma)
	\end{align*}
	and we would like to show 
	\begin{align*}
	\frac{\kappa(\Sigma)}{\kappa(D)} & \approx\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})
	\end{align*}
	for a suitable class of matrices $\Sigma$. 
	
	Is $\frac{\alpha+1}{\alpha-1}$ a proxy of the condition number of
	$\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})$? Yes-- the larger
	$\alpha$ is, the closer $D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}$
	is to the identity matrix, and the closer its condition number is
	to 1. Hence the what we are looking for is a result that connects
	$\alpha$ to the condition number of the scaled matrix.
	\end{rem}
	\end{comment}
\end{remark}

\subsection{Diagonal Dominance and Condition Number}

In the previous subsection, we showed that diagonal pre-conditioning
with sample column norms yields matrices with condition numbers close
to the population correlation matrix, so that $\frac{\kappa(X^{T}X)}{\kappa(\Sigma)}$
and $\frac{\kappa(X_{0}^{T}X_{0})}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}$
are both close to 1 with high probability. In other words, the reduction
in condition number by diagonal preconditioning is on the order of
$\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}$.
This ratio, however, is not always large. In fact, it is not even
bounded below by 1. To study when the diagonal preconditioning procedure
is effective in reducing condition number, we pose the next question
in our analysis of diagonal preconditioning and condition numbers: 
\begin{question}
	For what covariance matrices $\Sigma$ is the ratio $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}$
	large, where $D=\text{diag}(\Sigma)$?
\end{question}
\begin{comment}
\textbf{connection with Jacobi method}
\end{comment}
It is well-known that a matrix whose columns have different scales
tends to have a large condition number. This is the reason behind
normalization procedures used to process data in a variety of contexts
such as PCA and first order optimization methods. However, the answer
to our question about whether the correlation matrix has a much smaller
condition number will depend on the structure of the correlation matrix
as well. 

As a first step to explore this dependence, we randomly generate some
covariance matrices and look for those with small ratio $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}$.
In Table \ref{tab:bad covariance} we present some examples of covariance
matrices with $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}<1$,
i.e. the correlation matrix is more ill-conditioned than the covariance
matrix.

\textbf{}
\begin{table}
	\begin{centering}
		\textbf{}%
		\begin{tabular}{|c|c|}
			\hline 
			$\Sigma$ & $D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}$\tabularnewline
			\hline 
			\hline 
			$\begin{bmatrix}0.17 & -0.49 & -0.19 & -0.36\\
			& 2.34 & 0.71 & 1.79\\
			&  & 0.32 & 0.53\\
			&  &  & 1.44
			\end{bmatrix}$ & $\begin{bmatrix}1 & -0.77 & -0.80 & -0.73\\
			& 1 & 0.81 & 0.97\\
			&  & 1 & 0.78\\
			&  &  & 1
			\end{bmatrix}$\tabularnewline
			\hline 
			$\begin{bmatrix}1.76 & -0.41 & -0.61 & -1.86\\
			& 0.21 & -0.11 & -0.45\\
			&  & 0.28 & 0.64\\
			&  &  & 1.99
			\end{bmatrix}$ & $\begin{bmatrix}1 & -0.66 & -0.86 & 0.99\\
			& 1 & -0.47 & -0.68\\
			&  & 1 & 0.85\\
			&  &  & 1
			\end{bmatrix}$\tabularnewline
			\hline 
		\end{tabular}
		\par\end{centering}
	\textbf{\caption{\label{tab:bad covariance}Examples of covariance matrices whose corresponding
			correlation matrices have larger condition number.}
	}
\end{table}
We see that the correlation matrices with large condition numbers
all have off-diagonal entries that are close to 1, which is confirmed
by other examples. %
\begin{comment}
We conjecture that if a covariance matrix $\Sigma$ satisfies $\Sigma_{ij}\approx\sqrt{\Sigma_{ii}\Sigma_{jj}}$,
the associated correlation matrix has a large condition number.\textbf{
In particular, we show first that if the correlation matrix has large
off-diagonal terms, its condition number tends to be large. In this
case, diagonal preconditioning does not help much.}
\end{comment}

In this section, we show that if a covariance matrix $\Sigma$ has
columns (and rows) that are of different scales, but its corresponding
correlation matrix is diagonally dominant, then diagonal preconditioning
can achieve a reduction in condition number on the order of $\kappa(D)$
with high probability, where $D$ is the matrix consisting of the
diagonal entries of $\Sigma$. To put the result in perspective, note
that $\kappa(\Sigma)\leq\kappa(D)\cdot\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})$
is always true. We are interested in sufficient conditions that guarantee
a matching lower bound, so that $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}\approx\kappa(D)$,
i.e. the reduction is on the order of $\kappa(D)$ with high probability
for a class of matrices. 
\begin{remark}
	\begin{comment}
	\textbf{Need to clean up.}
	\end{comment}
	One useful tool that helps us to understand the condition numbers
	of correlation and covariance matrices is the Cholesky decomposition:
	any positive definite matrix $M$ can be written as $M=LL^{T}$ where
	$L$ is a lower triangular matrix with non-negative diagonal entries. 
	
	Let $\Sigma_{0}$ be a correlation matrix, that is $\Sigma_{0}$ is
	positive definite with diagonal entries equal to 1 and off-diagonal
	entries in $[-1,1]$ and let $D$ be a diagonal matrix with strictly
	positive entries. Then $D^{\frac{1}{2}}\Sigma_{0}D^{\frac{1}{2}}$
	defines a covariance matrix whose diagonal is equal to $D$. 
	
	Let $\Sigma_{0}=LL^{T}$ be the Cholesky decomposition of $\Sigma_{0}$.
	This decomposition gives us some intuition about when a correlation
	matrix is ill-conditioned. Since $\Sigma_{0}$ has diagonal entries
	equal to 1, the norm of every row of $L$ is 1. Suppose $(\Sigma_{0})_{ij}$
	has large magnitude for some $i<j$. Since $(\Sigma_{0})_{ij}=\ell_{i}^{T}\ell_{j}$
	where $\ell_{i}$ denotes the $i$th row of $\Sigma_{0}$, and $L_{ij}=0$
	for $j>i$ because $L$ is lower triangular, $|\ell_{i}^{T}\ell_{j}|$
	is large only if the first $i$ entries of $\ell_{j}$ has large norm,
	which forces $L_{jj}$ to be small. The condition number of $L$,
	$\kappa(L)$, is not equal to $\frac{\max_{i}|L_{ii}|}{\min_{i}|L_{ii}|}$,
	which is only true for diagonal matrices. However, as we have seen,
	$\kappa(L)\geq\frac{\max_{i}|L_{ii}|}{\min_{i}|L_{ii}|}$, which implies
	that $\kappa(L)$ is likely to be large, i.e. $\Sigma_{0}$ is ill-conditioned.
	This heuristic argument will be made rigorous, but it provides the
	main intuition that a correlation matrix is ill-conditioned if and
	only if it has off-diagonal term with magnitude close to 1. 
	
	By the basic properties of condition number, $\kappa(\Sigma_{0})=\kappa^{2}(L)=\kappa^{2}(L^{T})$
	and 
	\begin{align*}
	\kappa(\Sigma) & =\kappa(D^{\frac{1}{2}}\Sigma_{0}D^{\frac{1}{2}})
	=\kappa^{2}(L^{T}D^{\frac{1}{2}})=\kappa^{2}(D^{\frac{1}{2}}L)
	\end{align*}
	Again, since $\kappa(D^{\frac{1}{2}}L)\geq\frac{\max_{i}|L_{ii}D_{ii}^{\frac{1}{2}}|}{\min_{i}|L_{ii}D_{ii}^{\frac{1}{2}}|}$
	and $L_{ii}$ are bounded above by 1, the right hand side will be
	dominated by $\frac{\max_{i}(D_{ii}^{\frac{1}{2}})}{\min_{i}(D_{ii}^{\frac{1}{2}})}=\kappa(D^{\frac{1}{2}})$
	if $\max_{i}(D_{ii}^{\frac{1}{2}})\gg1$ and $\frac{\max_{i}L_{ii}}{\min_{i}L_{ii}}$
	is not too large. On the other hand, if $\frac{\max_{i}L_{ii}}{\min_{i}L_{ii}}$
	is large, in which case $\Sigma_{0}$ is ill conditioned, then the
	right hand side may well be dominated by this quantity instead of
	$\kappa(D^{\frac{1}{2}})$.
	
	So the intuition here is that the condition number of a covariance
	matrix also depends on the scale difference between the largest standard
	deviation and smallest standard deviation. If the diagonal matrix
	$D$ of variances is ill-conditioned but the correlation matrix is
	well conditioned, the condition number of the covariance matrix is
	close to that of its diagonal. 
\end{remark}
The Cholesky decomposition has thus provided us with the following
two intuitions. First, a correlation matrix is ill conditioned if
it has off diagonal entries with magnitude close to 1. Second, if
the diagonal of a covariance matrix has a large condition number,
then likely so does the covariance matrix itself. We now make these
intuitions rigorous. 

We start with a result on the condition number of diagonally dominant
matrices. 
\begin{lemma}
\label{lem:diagonal dominance}Assume $M\in\mathbb{R}^{p\times p}$
is square invertible with $|M_{ii}|\ge\alpha\sum_{j\neq i}|M_{ij}|$
for all $i$ and some $\alpha>1$, then 
\begin{align*}
\kappa_{\infty}(M) & \leq\frac{\alpha+1}{\alpha-1}\cdot\frac{\max_{i}|M_{ii}|}{\min_{i}|M_{ii}|}
\end{align*}
for $\kappa_{\infty}$ defined based on the sup norm $\|M\|_{\infty}=\sup_{i,j}|M_{ij}|$,
and 
\begin{align*}
\kappa_{q}(M) & \leq p{}^{2/q}\frac{\alpha+1}{\alpha-1}\cdot\frac{\max_{i}|M_{ii}|}{\min_{i}|M_{ii}|}
\end{align*}
for $\kappa_{q}$ defined based on the $q$-norm $\|M\|_{q}=\sup_{\|v\|_{q}=1}\|Mv\|_{q}$
for $1\leq q<\infty$.
\end{lemma}
\proof{Proof}
For a fixed vector $x\in\mathbb{R}^{p}$, let $\|x\|_{\infty}=|x_{i}|$.
We have 
\begin{align*}
|(Mx)_{i}| & \geq|M_{ii}||x_{i}|-\sum_{j\neq i}|M_{ij}||x_{j}| \geq|M_{ii}||x_{i}|-\sum_{j\neq i}|M_{ij}||x_{i}|\\
& \geq(1-\frac{1}{\alpha})|M_{ii}||x_{i}|=(1-\frac{1}{\alpha})|M_{ii}|\|x\|_{\infty}
 \geq(1-\frac{1}{\alpha})\min_{i}|M_{ii}|\|x\|_{\infty}
\end{align*}
which implies $\frac{\|Mx\|_{\infty}}{\|x\|_{\infty}}\geq(1-\frac{1}{\alpha})\min_{i}|M_{ii}|$,
so that 
\begin{align*}
\|M^{-1}\|_{\infty} & =\max_{x\neq0}\frac{\|M^{-1}x\|_{\infty}}{\|x\|_{\infty}}=\max_{x\neq0}\frac{\|M^{-1}Mx\|_{\infty}}{\|Mx\|_{\infty}}\\
& =\max_{x\neq0}\frac{\|x\|_{\infty}}{\|Mx\|_{\infty}}\leq\frac{\alpha}{\alpha-1}\cdot\frac{1}{\min_{i}|M_{ii}|}
\end{align*}
On the other hand, 
\begin{align*}
\|M_{i}\|_{\infty} & \leq\sum_{j}|M_{ij}|\leq(1+\frac{1}{\alpha})|M_{ii}| \leq(1+\frac{1}{\alpha})\max_{i}|M_{ii}|
\end{align*}
from which we can conclude that $\kappa_{\infty}(M)\leq\frac{\alpha+1}{\alpha-1}\frac{\max_{i}|M_{ii}|}{\min_{i}|M_{ii}|}$.

Based on the upper bound for $\kappa_{\infty}$ and equivalence of
matrix norms, we can obtain upper bounds for condition numbers based
on $q$-norms. By Holder's inequality, $\|M\|_{q}\leq n^{1/q-1/q'}\|M\|_{q'}$
for $q\leq q'\leq\infty$. This suggests that $\|M\|_{q}\leq n^{1/q}\|M\|_{\infty}$
and so 
\begin{align*}
\kappa_{q}(M) & \leq p^{2/q}\kappa_{\infty}(M)\leq p^{2/q}\cdot\frac{\alpha+1}{\alpha-1}\frac{\max_{i}|M_{ii}|}{\min_{i}|M_{ii}|}
\end{align*}
	\hfill \Halmos
\endproof
To understand the above lemma in the context of covariance and correlation
matrices, compare $\kappa(\Sigma) \leq\kappa(\Sigma_{0})\cdot\kappa(D)$ with the bound 
\begin{align*}
\kappa(\Sigma) & \leq p\frac{\alpha+1}{\alpha-1}\frac{\max_{i}|\Sigma_{ii}|}{\min_{i}|\Sigma_{ii}|}=p\frac{\alpha+1}{\alpha-1}\cdot\kappa(D)
\end{align*}
from the lemma. We can see $\frac{\alpha+1}{\alpha-1}$ as a proxy
of the condition number $\kappa(\Sigma_{0})$ of the correlation matrix.
The larger $\alpha$ is, the closer $\Sigma_{0}$ is to the identity
matrix, and the closer its condition number is to 1. In the limit,
we should have $\lim_{\alpha\rightarrow\infty}\kappa(\Sigma_{0})=1=\lim_{\alpha\rightarrow\infty}\frac{\alpha+1}{\alpha-1}$.%
\begin{comment}
\textbf{Hence the what we are looking for is a result that connects
$\alpha$ to the condition number of the scaled matrix. }

There are analogous bounds if we assume similar diagonal dominance
properties in $p$-norm.\textbf{ The upper bounds for $\kappa_{p}$
are not very satifactory because of the dependence on dimension. If
instead of $|M_{ii}|\ge\alpha\sum_{j\neq i}|M_{ij}|$, we have an
analogous diagonal dominance condition in $p$-norm, we can obtain
dimension independent bounds.}
\begin{lem}
Assume $M\in\mathbb{R}^{n\times n}$ is square invertible with $|M_{ii}|\ge\alpha\cdot n^{\frac{1}{p}}\cdot(\sum_{j\neq i}|M_{ij}|^{q})^{1/q}$
for $\alpha>1$ and all $i$, then 
\begin{align*}
\kappa_{p}(M) & \leq\frac{(1+\frac{1}{\alpha^{q}n^{\frac{q}{p}}})^{\frac{1}{q}}\cdot n^{\frac{1}{p}}}{(1-\frac{1}{\alpha})}\cdot\frac{\max_{i}|M_{ii}|}{\min_{i}|M_{ii}|}
\end{align*}
for $1\leq q<\infty$ and $\frac{1}{p}+\frac{1}{q}=1$. 
\end{lem}
\begin{proof}
We have
\begin{align*}
|(Mx)_{i}| & =|\sum_{j}M_{ij}x_{j}|\\
& \leq|\sum_{j}|M_{ij}|^{q}|^{\frac{1}{q}}\cdot\|x\|_{p}\\
& =||M_{ii}|^{q}+\sum_{j\neq i}|M_{ij}|^{q}|^{\frac{1}{q}}\cdot\|x\|_{p}\\
& \leq((1+\frac{1}{\alpha^{q}n^{\frac{q}{p}}})|M_{ii}|^{q})^{\frac{1}{q}}\cdot\|x\|_{p}
\end{align*}
which implies 
\begin{align*}
\|M\|_{p} & \leq(1+\frac{1}{\alpha^{q}n^{\frac{q}{p}}})^{\frac{1}{q}}\cdot n^{\frac{1}{p}}\cdot\max_{i}|M_{ii}|
\end{align*}
On the other hand, for each fixed $x$, let $i$ be the coordinate
such that $|x_{i}|\geq n^{-\frac{1}{p}}\|x\|_{p}$. We know that such
$i$ exists, because otherwise $\sum_{i}|x_{i}|^{p}<\|x\|_{p}^{p}$,
a contradiction. With this $i$, we have
\begin{align*}
|(Mx)_{i}| & \geq|M_{ii}|\cdot|x_{i}|-(\sum_{j\neq i}|M_{ij}|^{q})^{\frac{1}{q}}\cdot(\sum_{j\neq i}|x_{j}|^{p})^{\frac{1}{p}}\\
& \geq|M_{ii}|\cdot|x_{i}|-\frac{1}{\alpha}\cdot n^{-\frac{1}{p}}\cdot|M_{ii}|\cdot(\sum_{j\neq i}|x_{j}|^{p})^{\frac{1}{p}}\\
& \geq|M_{ii}|\cdot n^{-\frac{1}{p}}\|x\|_{p}-n^{-\frac{1}{p}}\frac{1}{\alpha}|M_{ii}|\cdot\|x\|_{p}\\
& \geq n^{-\frac{1}{p}}\cdot(1-\frac{1}{\alpha})|M_{ii}|\cdot\|x\|_{p}
\end{align*}
so that 
\begin{align*}
\frac{\|Mx\|_{p}}{\|x\|_{p}} & \geq(1-\frac{1}{\alpha})\cdot\min_{i}|M_{ii}|
\end{align*}
and so 
\begin{align*}
\|M^{-1}\|_{p} & =\max_{x\neq0}\frac{\|x\|_{p}}{\|Mx\|_{p}}\\
& \leq\frac{1}{(1-\frac{1}{\alpha})}\cdot\frac{1}{\min_{i}|M_{ii}|}
\end{align*}
from which we have 
\begin{align*}
\kappa_{p}(M) & \leq\frac{(1+\frac{1}{\alpha^{q}n^{\frac{q}{p}}})^{\frac{1}{q}}\cdot n^{\frac{1}{p}}}{(1-\frac{1}{\alpha})}\cdot\frac{\max_{i}|M_{ii}|}{\min_{i}|M_{ii}|}
\end{align*}
\end{proof}
%
\end{comment}

\begin{comment}
The above lemmas show that diagonally dominant matrices tend to be
well conditioned. Conversely, our heuristic argument suggested that
if a matrix has a large off-diagonal element, it tends to be ill conditioned.
We specialize these ideas in the following result for correlation
matrices. 
\end{comment}
\begin{comment}
\begin{prop}
\textbf{Let $M$ be a correlation matrix. Suppose $|M_{ij}|\geq\beta$
for some $\beta\in(0,1)$. Then 
\begin{align*}
\kappa(\Sigma_{0}) & \geq
\end{align*}
Conversely, if $|M_{ij}|\leq\gamma$ for some $\gamma\in(0,1)$ and
all $i,j$, then }
\end{prop}
\begin{proof}
\textbf{Let $M=LL^{T}$ be the Cholesky decomposition of $M$, and
let $\ell_{i}$ be the $i$th row of $L$. We have 
\begin{align*}
\geq|\ell_{i}^{T}\ell_{j}|=|\Sigma_{ij}| & \geq\beta\cdot\sqrt{\Sigma_{ii}\Sigma_{jj}}
\end{align*}
}

\textbf{We have 
\begin{align*}
\kappa(D^{\frac{1}{2}}L) & \geq\frac{\max_{i}D_{ii}^{\frac{1}{2}}L_{ii}}{\min_{i}D_{ii}^{\frac{1}{2}}L_{ii}}\\
\end{align*}
and 
\begin{align*}
\kappa(L) & \geq\frac{\max_{i}L_{ii}}{\min_{i}L_{ii}}\\
\end{align*}
}
\end{proof}
\textbf{}
%
\textbf{Is it true that $\kappa(\Sigma)\geq\min(\kappa(\Sigma_{0}),\kappa(D))$???}
\end{comment}

\textbf{}%
\begin{comment}
\textbf{so what we are looking for is a lower bound, that says if
the matrix is not diagonally dominant, then it is ill-conditioned.
This can then be applied to conclude that covariance matrix with columns
of different scales generally is much more ill-conditioned than correlation
matrix. 
\begin{align*}
\frac{\kappa(\Sigma)}{\kappa(D)}\leq\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}) & \leq\kappa(D^{-1})\cdot\kappa(\Sigma)
\end{align*}
and we would like to show 
\begin{align*}
\frac{\kappa(\Sigma)}{\kappa(D)} & \approx\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})
\end{align*}
for a suitable class of matrices $\Sigma$. }
\end{comment}

We shall use the above result to give a sufficient condition on when
the ratio $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}$
is large, i.e. when diagonal preconditioning with column standard
deviation/norm achieves a significant reduction in condition number
with high probability. 

More specifically, we show that if the correlation matrix is diagonally
dominant, then the ratio $\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}$
is bounded below by $\frac{1}{p}(\frac{\alpha-1}{\alpha+1})^{2}\kappa(D)$.
\begin{theorem}
	For a covariance matrix $\Sigma$, if $\sqrt{\Sigma_{ii}}\ge\alpha\sum_{j\neq i}|\frac{\Sigma{}_{ij}}{\sqrt{\Sigma_{jj}}}|$,
	then we have 
	\begin{align*}
	\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})} & \geq\frac{1}{p}(\frac{\alpha-1}{\alpha+1})^{2}\kappa(D)
	\end{align*}
	
	\begin{comment}
	\textbf{Conversely, ...}
	\end{comment}
\end{theorem}
\proof{Proof}
	Let $\Sigma_{0}=D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}}$. The conditions
	$\sqrt{\Sigma_{ii}}\ge\alpha\sum_{j\neq i}|\frac{\Sigma{}_{ij}}{\sqrt{\Sigma_{jj}}}|$
	imply that $\Sigma_{0}$ is diagonally dominant, so that by the previous
	lemma $\kappa(\Sigma_{0})  \leq p\frac{\alpha+1}{\alpha-1}$ since $\Sigma_{0}$ has diagonal equal to 1. 
	
	The main ingredient of the proof is to use the Cholesky decomposition
	of the correlation matrix and the fact that for a triangular matrix
	$L$, the following condition holds:
	\begin{align*}
	\kappa(L) & \geq\frac{\max_{i}L_{ii}}{\min_{i}L_{ii}}
	\end{align*}
	
	Now let $\Sigma_{0}=L_{0}L_{0}^{T}$ be the Cholesky factorization
	of $\Sigma_{0}$where $L_{0}$ is a lower triangular matrix. It then
	follows that $\Sigma=LL^{T}$ where $L=D^{\frac{1}{2}}L_{0}$ is also
	a lower triangular matrix. We have 
	\begin{align*}
	(\frac{\alpha+1}{\alpha-1})^{2}\cdot\kappa(\Sigma) & =(\frac{\alpha+1}{\alpha-1})^{2}\cdot(\kappa(D^{\frac{1}{2}}L_{0}))^{2} \geq(\frac{\alpha+1}{\alpha-1})^{2}\cdot(\frac{\max_{i}(D^{\frac{1}{2}}L_{0})_{ii}}{\min_{i}(D^{\frac{1}{2}}L_{0})_{ii}})^{2}\\
	& \geq(\frac{\alpha+1}{\alpha-1})^{2}\cdot(\frac{\max_{i}(D^{\frac{1}{2}})_{ii}}{\min_{i}(D^{\frac{1}{2}})_{ii}})^{2}\cdot(\frac{\min_{i}(L_{0})_{ii}}{\max_{i}(L_{0})_{ii}})^{2}\\
	& =(\frac{\alpha+1}{\alpha-1})^{2}\cdot\kappa^{-2}(L_{0})\cdot\kappa^{2}(D^{\frac{1}{2}}) =(\frac{\alpha+1}{\alpha-1})^{2}\cdot\kappa^{-1}(\Sigma_{0})\cdot\kappa(D)\\
	& \geq(\frac{\alpha+1}{\alpha-1})\cdot\kappa(D)\geq\frac{1}{p}\kappa(\Sigma_{0})\cdot\kappa(D)
	\end{align*}
	where we have used the inequality $\|f\cdot g\|_{\infty}\geq\|f\|_{\infty}/\|g^{-1}\|_{\infty}$
	for vectors $f,g\in\mathbb{R}_{++}^{p}$ and $f\cdot g$ is element-wise
	multiplication. 
	
	Rewriting the inequality gives the desired inequality
	\begin{align*}
	\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})} & \geq\frac{1}{p}(\frac{\alpha-1}{\alpha+1})^{2}\kappa(D)
	\end{align*}
	\hfill \Halmos
\endproof
We have thus shown that when the correlation matrix $\Sigma_{0}$
is $\alpha$-diagonally dominant, the ratio of condition numbers $\frac{\kappa(D^{\frac{1}{2}}\Sigma_{0}D^{\frac{1}{2}})}{\kappa(\Sigma_{0})}$
is bounded below by $\frac{1}{p}(\frac{\alpha-1}{\alpha+1})^{2}\kappa(D)$.
For a design matrix with sub-Gaussian rows with covariance matrix
satisfying this condition, the reduction of condition number is on
the order of $\sqrt{\kappa(D)}$ with high probability. \textbf{}%
\begin{comment}
\textbf{It may be possible to relax the conditions $\sqrt{\Sigma_{ii}}\ge\alpha\sum_{j\neq i}|\frac{\Sigma{}_{ij}}{\sqrt{\Sigma_{jj}}}|$
to obtain a similar result for larger class of covariance matrices.
Extend this! }
\end{comment}

\textbf{}%
\begin{comment}
\begin{conjecture}
\textbf{Assume $\Sigma$ is positive definite and there exists $0<\alpha<1$
such that for all (or just some?) $i$, there exists some $j$ with
\begin{align*}
|\Sigma_{ii}| & <\alpha|\Sigma_{ij}|
\end{align*}
}

\textbf{then we have }

\textbf{
\begin{align*}
\kappa(\Sigma) & \geq\frac{1+\alpha}{1-\alpha}\cdot\frac{\max_{i}|\Sigma_{ii}|}{\min_{i}|\Sigma_{ii}|}
\end{align*}
}
\end{conjecture}
\textbf{}
%
\textbf{Claim: If $|a_{ii}|<\alpha|a_{ij}|$ for $j\neq i$ and all
$i$, where $\alpha\in(0,1)$, then 
\begin{align*}
\kappa(\begin{pmatrix}a_{11} & a_{12} & \dots\\
a_{21}\\
\dots
\end{pmatrix}) & \geq\kappa(\begin{pmatrix}a_{11} & \frac{1}{\alpha}a_{11} & \dots\\
\frac{1}{\alpha}a_{11}\\
\\
\\
\end{pmatrix})\\
& =\frac{1+\alpha}{1-\alpha}\kappa(\begin{pmatrix}a_{11}\\
& \dots\\
\\
&  & a_{n}
\end{pmatrix})
\end{align*}
First note 
\begin{align*}
\kappa(\begin{pmatrix}a_{11} & \frac{1}{\alpha}a_{11}\\
\frac{1}{\alpha}a_{22} & a_{22}
\end{pmatrix}) & =\frac{1+\frac{1}{\alpha}}{}\\
\end{align*}
}
\end{comment}

==> major revision/dsdp-old.tex <==
\section{Optimal Preconditioning via Dual SDP}
\label{sec:DSDP}
In this section, we propose a practical approach to efficiently find optimal diagonal preconditioners via solving a dual SDP problem. Although the theoretical computational complexity of this DSDP approach is higher than the potential reduction algorithm, in practice, we are able to find optimal diagonal preconditioners for matrices with size $\sim$5000 within reasonable time, using a customized DSDP solver \textbf{add reference here}. We will explore in depth the empirical performance of the DSDP approach on matrices from the SuiteSparse Collection. 

\subsection{A Dual SDP Formulation of Optimal Preconditioning}

Recall the optimal diagonal preconditioning problem given a PD matrix $M$:
\begin{align*}
\min_{\kappa,D}\kappa\\
s.t.M\succeq D\\
\kappa D\succeq M\\
D\succeq0
\end{align*}
Due to the fact that $\kappa$ and $D$ are both variables, this problem is not in standard SDP form. However, there is a simple way to transform it into an SDP problem. Specifically, we can do a change of variables $\kappa\rightarrow1/\kappa$ to obtain
\begin{align*}
\max_{(\tau,d)}\tau\\
s.t.D-M\preceq0\\
\tau M-D\preceq0
\end{align*}
 which is in standard dual SDP form, with $D$ the diagonal matrix
with $d$ on the diagonal. 

Note that a feasible solution for this SDP is $(\tau, d) = (-1, \mathbf{0})$, and although the optimal objective value is always positive, using this feasible solution as a starting point in the DSDP solver can lead to significant improvements. Moreover, for very ill-conditioned matrices with the minimum eigenvalue $\lambda_{\min}$ close to 0, we propose to use the initialization $(\tau, d) = (-1/\delta, \mathbf{0})$ for $\delta=O(\lambda_{\min})$ to further improve the stability of the DSDP solver.

\subsection{HDSDP: A Customized DSDP Solver}

Here can include a brief introduction to the HDSDP solver.

\subsection{Empirical Performance on SuiteSpare Matrices}
Here can consider reporting the following metrics:

\begin{itemize}
    \item Clock Time
    \item Suboptimality Gap vs. Iteration
    \item Reduction in Condition Number
\end{itemize}

==> major revision/dsdp.tex <==


\section{Optimal Diagonal Preconditioning via Semi-Definite Programming}

\label{sec:DSDP}

So far, we have focused on the two-side optimal diagonal preconditioning problem \begin{align*}
\min_{D_{1},D_{2}\succ0}\kappa(D_{1}^{1/2}AD_{2}^{-1/2}).
\end{align*}
In this section, we turn our attention to the one-sided optimal diagonal preconditioning problems:
\begin{align*}
\min_{D_{1}\succ0}&\kappa(D_{1}^{1/2}A)\\
\min_{D_{2}\succ0}&\kappa(AD_{2}^{-1/2}),
\end{align*} 
and propose an alternative approach to efficiently find optimal one-sided diagonal preconditioners via solving dual SDP problems. Although the
theoretical complexity of this dual SDP approach is higher than the
potential reduction algorithm we proposed in Section \ref{sec:optimal}, in practice, we are able to find optimal
diagonal preconditioners for matrices with size 5000 within reasonable time,
using an efficient customized dual SDP solver \citep{gao2022hdsdp}. Moreover, combined with a row/column sampling technique, the proposed approach can find near-optimal diagonal preconditioners for even larger (size $\geq 200,000$) problems. In Section \ref{sec:experiments}, we conduct massive numerical
experiments to explore the empirical performance of the dual SDP approach on
matrices from the \texttt{SuiteSparse} \citep{kolodziej2019suitesparse} matrix collection, as well as \texttt{LIBSVM} \citep{chang2011libsvm} and large machine learning datasets from
\texttt{OPENML} \citep{rijn2013openml}. %See Section \ref{sec:experiments} for details on our experiments based on the dual SDP approach.

\subsection{Dual SDP Formulation of Optimal Diagonal Preconditioning}
\label{subsec:dual-SDP}
Recall the following reformulation of the two-sided optimal diagonal preconditioning problem:
\begin{align*}
    \min_{\kappa\geq0} \kappa \\
A^{T}D_{1}A\succeq D_{2}\\
\kappa D_{2}\succeq A^{T}D_{1}A \\
D_1 \succeq I_m 
\end{align*}
Suppose now we are instead interested in finding optimal \emph{one-sided} diagonal preconditioners. This means setting either $D_1 = I_m$ or $D_2=I_n$ in the two-sided problem above. We will see that the resulting problems admit reformulations as standard dual SDP problems. This opens up the possibility of using efficient customized SDP solvers to find optimal diagonal preconditioners. First, setting $D_1=I_m$ gives the following optimal \emph{right} preconditioning problem:
\begin{align*}
  \min_{\kappa, D_2} \kappa \\
   A^TA \succeq D_2  \\
   \kappa D_2 \succeq A^TA  \\
   D_2 \succeq 0  
\end{align*}
where $D_2$ is restricted to be a diagonal matrix. Note that the strict lower bound $D_2 \succ 0$ is no longer necessary, since the condition that $\kappa D_2 \succeq A^TA$ will automatically enforce $\kappa > 0$ and $ D_2 \succ 0$, because we assume $A$ has full rank, and so $M:=A^TA \succ 0$.  

The key now is to do a change of variable $\tau: = 1 / \kappa$, and introduce $d:= \text{diag} (D_2 )$. Then minimization of $\kappa$ becomes \emph{maximization} of $\tau$, and with $M=A^TA$, the problem is equivalent to
\begin{align}
\label{eq:DSDP-right}
\begin{split}
      \max_{\tau, d}  \tau \\
  \text{s.t.}  \sum_{i = 1}^m e_i e_i^T d_i  \preceq M  \\
   \tau M - \sum_{i = 1}^m e_i e_i^T d_i  \preceq 0  \\
   d  \succeq 0 ,
  \end{split}
\end{align}
where $e_i$ is the $i$-th column of the identity matrix. Note that problem \eqref{eq:DSDP-right} is in standard dual SDP form (a.k.a. inequality form) \citep{luenberger1984linear}, and can be solved efficiently by customized dual SDP solvers. As we demonstrate in experiments in Section \ref{sec:experiments}, an important idea that allows us to further speed up this approach in practice for very tall matrices ($m$ very large) is to randomly \emph{sub-sample} the rows of $A$ before forming $M=A^TA$ in \eqref{eq:DSDP-right}.

Similarly, the optimal \emph{left} diagonal preconditioning problem 
\begin{align*}
    \min_{\kappa\geq0} \kappa \\
A^{T}D_{1}A\succeq I_n\\
\kappa I_n\succeq A^{T}D_{1}A \\
D_1 \succeq 0 
\end{align*}
can be transformed into a standard dual SDP with the change of variables $\tau = 1/\kappa$, $D_1/\kappa = \text{diag}(d)$:
\begin{align}
\label{eq:DSDP-left}
\begin{split}
     \max_{\tau,d}\tau\\
\text{s.t.}\sum_{i}A_{i}A_{i}^{T}d_{i} \succeq\tau I_n	\\
I_n\succeq \sum_{i}A_{i}A_{i}^{T}d_{i} \\
d\succeq0
\end{split}	
\end{align}
where we have used the identity that $A^{T}D_1A=\sum_{i}A_{i}A_{i}^{T}(D_{1})_{ii}$, where $A_{i}$ is the $i$-th row of $A$.
\begin{theorem}
The one-sided optimal diagonal preconditioning problems \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem} are equivalent to the standard dual SDP problems \eqref{eq:DSDP-left} and \eqref{eq:DSDP-right}, respectively.
\end{theorem}

Importantly, the dual SDP formulations \eqref{eq:DSDP-right} and \eqref{eq:DSDP-left} of the one-sided problems
enjoy low-rank or sparse data matrices, and are therefore particularly amenable
to efficient customized dual SDP solvers such as \texttt{DSDP} \citep{benson2008algorithm} and \texttt{HDSDP} \citep{gao2022hdsdp}.
In Section \ref{subsec:hdsdp}, we give a brief introduction to the \texttt{HSDSP} solver, and discuss
how this dual SDP solver can solve the one-sided optimal diagonal
preconditioning problems efficiently by combining randomization and
customized numerical linear algebra.

Before we move on to discuss solving large one-sided preconditioning problems in practice, we remark on the two-sided problem. One may wonder whether the two-sided optimal diagonal preconditioning problem \eqref{eq:SDP-two-sided} also admits a reformulation as a dual SDP problem. However, because now variables $D_1$ and $D_2$ appear simultaneously on different sides of the constraint $\kappa D_{2}\succeq A^{T}D_{1}A$, it is not possible to use the same change of variable $\tau=1/\kappa$ to circumvent the product of variables as before. The equivalent quasi-convex problem \eqref{eq:quasi-convex} suggests that it may be impossible to cast the problem as an SDP. However, there exists a simple iterative procedure to obtain two-sided optimal diagonal preconditioners based on solving one-sided problems. More precisely, let $A_0 := A$. At the $k$-th step for odd $k$, we solve the left-sided problem $\min_{D_{1}\succ0}\kappa(D_{1}^{1/2}A_{k-1})$ by solving the equivalent SDP \eqref{eq:DSDP-left}, and update $A_{k}:=D_{1}^{1/2}A_{k-1}$, where $D_{1}$ is the optimal left diagonal preconditioner we just obtained. At the $k$-th step for even $k$, we solve the right-sided problem $\min_{D_{2}\succ0}\kappa(A_{k-1}D_{2}^{-1/2})$ by solving the equivalent SDP \eqref{eq:DSDP-right}, and then update $A_{k}:=A_{k-1}D_{2}^{-1/2}$.
We can then repeat the process, solving one-sided problems for the updated scaled matrix $A_k$ obtained from the previous step.
It is obvious that any fixed point of this iterative procedure is a solution to the two-sided problem. One should expect the procedure to converge, although we do not formally prove it in this paper.

\subsection{HDSDP: A Customized Dual SDP Solver}
\label{subsec:hdsdp}

In this section, we introduce the dual semi-definite programming solver
\texttt{HDSDP} \citep{gao2022hdsdp} and its internal customization mechanisms for the
optimal diagonal preconditioning problem. \texttt{HDSDP} implements a dual
potential reduction interior point method that exploits both low-rankness and
sparsity and is specifically optimized for the above preconditioning problem via
randomization.

In practice, when \texttt{HDSDP} receives $A \in \mathbb{R}^{m \times
n}$, it randomly samples $\tilde{m}$ rows without replacement and constructs a
submatrix $\tilde{A} \in \mathbb{R}^{\tilde{m} \times n}$. Then it
computes $\tilde{M} = \tilde{A}^T \tilde{A}$ and solves the right preconditioning
problems using the dual SDP \eqref{eq:DSDP-right}. Using special data
structures, the flops in each main iteration of the interior point method is
reduced to $O (n^3)$ and if $m \gg n$, we
compute the preconditioner with $O (n^3 + \tilde{m}n^2)$ complexity. We note that
when $A$ is dense and $m$ is large, computing and factorizing $A^T A$ becomes
prohibitive and the only viable method to solve $A^T A x = A^Tb$ is using
iterative solvers. By applying optimal diagonal right preconditioners, we can significantly reduce the computation time of such iterative solvers for the modified system.

Random row sampling is an important component of our solver at finding optimal preconditioners efficiently in practice, and as the empirical results in Section \ref{sec:experiments} suggest, we often only need
$\tilde{m} = O(\log{m})$ to give a high-quality preconditioner, and the overall complexity is then $O (n^3 + n^2 \log{m})$. Row sampling works particularly well when the rows of $A$ are generated from a common statistical distribution.
Note, however, that the row sampling technique only applies when finding right preconditioners.  For left preconditioning problems, we can similarly employ column sampling, although this may not yield as significant reductions in computation time since $m\geq n$.

Lastly, we note that the \texttt{HDSDP} solver we used can be modified to be a first-order type solver, where each iteration is solved by the diagonal-preconditioned conjugate gradient
method (here we just use heuristic diagonal preconditioners). Since the SDPs from large real datasets we consider are sparse, the associated SDP problems are generally handled better by 
the Cholesky method.


==> major revision/experiments-old.tex <==
\section{Numerical Experiments}
\label{sec:experiments}

In this section, we perform numerical experiments to compare the performance
of diagonal preconditioning methods at accelerating gradient and stochastic
gradient descent applied to regression and classification problems. 

\subsection{Simulated Dataset}

For our simulated dataset, we randomly generate design matrix $X$
whose rows are i.i.d. Gaussian vectors with covariance matrix $\Sigma$.
The covariance matrix itself is generated using the sklearn package
in python, and has condition numbers in the range of 100-1000. We
consider the regression problem 
\begin{align*}
\min_{\theta}\frac{1}{n}\|X\theta-Y\|_{2}^{2}
\end{align*}
where $Y$ is generated using a ground-truth parameter $\theta^{\ast}$,
and we assess the speed of convergence by looking at the distance
of estimate to the optimal solution of the quadratic problem, namely
the OLS estimate $\theta_{OLS}$ of $\theta$: we declare convergence
when $\|\theta^{(k)}-\theta_{OLS}\|_{2}/\|\theta_{OLS}\|_{2}$ is
below some threshold, usually set to be $0.01$. 

We consider the following modified problem 
\begin{align*}
\min_{\tilde{\theta}}\frac{1}{n}\|XD\tilde{\theta}-D_{0}Y\|_{2}^{2}
\end{align*}
where $D$ is one of the following diagonal preconditioners: 
\begin{itemize}
	\item Normalization: $D$ is the diagonal matrix of column standard deviations
	or norms of $X$.
	\item Optimal diagonal preconditioning: $D$ minimizes $\kappa(DX^{T}XD)$
	among all positive diagonal matrices.
	\item (full) Batch normalization: $D_{0}=I$, and $D_{1}^{(0)}$ is the
	diagonal matrix of column standard deviations of $X$. At the $k$th
	iteartion, update $\theta^{(k+1)}$ by solving $\min_{\theta}\frac{1}{n}\|XD^{(k)}\theta-y\|_{2}^{2}$
	and then form $D_{1}^{(k+1)}$ by solving $\min_{D}\frac{1}{n}\|XD\theta^{(k+1)}-y\|_{2}^{2}$.
\end{itemize}
We compare the convergence speeds of gradient and stochastic gradient
descent methods with these preconditioners. Step size is determined
by backtracking line search using the Armijo-Goldstein conditions.

For stochastic gradient descent, since $X$ is not directly available,
we use the corresponding adaptive versions of the above procedures:

\begin{comment}
\begin{itemize}
\item Optimal diagonal preconditioning: $D_{0}=I$ and $D_{1}$ minimizes
$\kappa(DX^{T}XD)$.
\item Normalization: $D_{0}=I$ and $D_{1}$ is the diagonal matrix of column
standard deviations of $X$
\item Matrix equilibriation: $D_{0}^{-1}=\text{diag}(\sum_{j}|X_{1j}|,\dots,\sum_{j}|X_{nj}|)$,
$D_{1}^{-1}=\text{diag}(\sum_{i}|(D_{0}X)_{i1}|,\dots,\sum_{i}|(D_{0}X)_{ip}|)$.
\item (full) Batch normalization: $D_{0}=I$, and $D_{1}^{(0)}$ is the
diagonal matrix of column standard deviations of $X$. At the $k$th
iteartion, update $\theta^{(k+1)}$ by solving 
\begin{align*}
& \min_{\theta}\frac{1}{n}\|XD^{(k)}\theta-y\|_{2}^{2}
\end{align*}
and then form $D_{1}^{(k+1)}$ by solving
\begin{align*}
& \min_{D}\frac{1}{n}\|XD\theta^{(k+1)}-y\|_{2}^{2}
\end{align*}
\end{itemize}
\end{comment}
%
\begin{itemize}
	\item Normalization: $D$ is the diagonal matrix of column standard deviations
	or norms of $X^{(k)}$, the batch of data in the $k$-th iteration.
	\item Adaptive optimal diagonal preconditioning: at $k$th iteration, form
	the cumulative design matrix $\overline{X}^{(k)}$ by concatenating
	$X^{(k)}$ with $\overline{X}^{(k-1)}$ and retaining unique rows,
	and find $D$ that minimizes $\kappa(D(\overline{X}^{(k)T}\overline{X}^{(k)}D)$.
	\item Batch normalization: $D^{(0)}=I$. At the $k$th iteartion, update
	$\theta^{(k+1)}$ by solving $\min_{\theta}\frac{1}{n}\|X^{(k)}D^{(k)}\theta-y\|_{2}^{2}$
	and then form $D^{(k+1)}$ by solving $\min_{D}\frac{1}{n}\|X^{(k)}D\theta^{(k+1)}-y\|_{2}^{2}$
	where $X^{(k)}$ is the batch of samples at the $k$th iteration. 
\end{itemize}
Tables \ref{tab:iterations_gd} and \ref{tab:iterations_sgd} summarize
the number of iterations before convergence for various methods and
problems of various sizes. We note that in many cases the optimal
diagonal preconditioner returns a preconditioned matrix with significantly
smaller condition number, as guaranteed by our theoretical analyses.
This is also manifested through the acceleration in convergence of
steepest descent. On the other hand, preconditioning with column statistics
does not always guarantee reduction in condition number. In general,
steepest descent with optimal diagonal preconditioning achieves comparable
performance to batch normalization when it performs well. On the other
hand, there are specific cases where stochastic gradient descent with
batch normalization takes considerably longer time than optimal preconditioning.
The tradoff here is that for large matrices ($p$ large), finding
an approximate optimal diagonal preconditioner may take a non-negligible
amount of time, whereas batch normalization only adds one extra step
of gradient update for the preconditioner $D$. The numerical simulations
also confirm that although batch normalization speeds up first order
optimization methods, the effective condition number of the design
matrix is not actually decreased. This suggests that although the
performance of batch normalization is comparable to that of optimal
diagonal preconditioning, the exact mechanism through which it speeds
up convergence remains to be investigated further. 

\begin{table}
	\begin{centering}
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline 
			$(n,p)$ & \multicolumn{2}{c|}{$(1000,20)$} & \multicolumn{2}{c|}{$(1000,40)$} & \multicolumn{2}{c|}{$(1000,100)$}\tabularnewline
			\hline 
			& iterations & $\kappa$ & iterations & $\kappa$ & iterations & $\kappa$\tabularnewline
			\hline 
			No preconditioning & 44529 & 278.30 & 39709 & 870.81 & 72795 & 1129.80\tabularnewline
			\hline 
			Fixed preconditioning & 16639 & 230.36 & 148954 & 909.80 & 62915 & 1087.84\tabularnewline
			\hline 
			Optimal preconditioning & 10230 & 144.81 & 29835 & 746.99 & 29881 & 858.46\tabularnewline
			\hline 
			Batch normalization & 11721 & 470.12 & 31032 & 1226.79 & 47654 & 1192.45\tabularnewline
			\hline 
		\end{tabular}
		\par\end{centering}
	\caption{\label{tab:iterations_gd}Number of iterations till convergence for
		preconditioning methods for gradient descent, with step size determined
		through backtracking line search. Convergence is declared when $\|\theta-\theta^{\ast}\|$
		is within a small constant factor of $\|\theta^{\ast}\|$, where $\theta^{\ast}$
		is the OLS solution, and $\theta$ is the effective coefficient taking
		into account the preconditioning on $X$. The covariance matrix $\Sigma$
		is randomly generated using python package sklearn and the condition
		number of the effective design matrix $X\sim\mathcal{N}(0,\Sigma)$
		is also reported above as $\kappa$. For example, for preconditioning
		with diagonal matrix $D$, the condition number of $XD$ is given.
		For batch normalization, since the condition number of the effective
		deisgn matrix changes every iteration, the median of those numbers
		are given. We see that preconditioning with column standard deviation
		does not always reduce the condition number of the design matrix,
		and indeed in such cases convergence of steepest descent is slowed
		down. }
\end{table}

\begin{table}
	\begin{centering}
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline 
			$(n,p)$ & \multicolumn{2}{c|}{$(1000,20)$} & \multicolumn{2}{c|}{$(1000,40)$} & \multicolumn{2}{c|}{$(1000,100)$}\tabularnewline
			\hline 
			& iterations & $\kappa$ & iterations & $\kappa$ & iterations & $\kappa$\tabularnewline
			\hline 
			No preconditioning & 12350 & 166.53 & 43712 & 986.51 & 96619 & 1637.54\tabularnewline
			\hline 
			Fixed preconditioning & 11825 & 140.86 & 100547 & 1149.97 & 54646 & 1594.44\tabularnewline
			\hline 
			Optimal preconditioning & 10791 & 126.07 & 31202 & 868.13 & 47310 & 1313.44\tabularnewline
			\hline 
			Batch normalization & 11189 & 251.85 & 35999 & 1280.45 & 48448 & 2012.47\tabularnewline
			\hline 
		\end{tabular}
		\par\end{centering}
	\caption{\label{tab:iterations_sgd}Number of iterations till convergence for
		adaptive preconditioning methods for mini-batch stochastic gradient
		descent, with step size determined through backtracking line search.
		Batch size is between 10-20\% of the training set size. The last two
		preconditioning methods, i.e. optimal preconditioning and batch normalization,
		are adaptive, whereas the first two only requires preconditioning
		once before the start of the optimization routine. For adaptive optimal
		diagonal preconditioning, the diagonal preconditioner is updated once
		every 100 iterations, using the most up to date cumulative design
		matrix. All reported condition numbers are medians of the sequence
		of condition numbers of the effective design matrix during training. }
\end{table}

\subsection{MNIST Dataset}

To compare the preconditioning procedures on a real dataset, we use
the MNIST handwritten digit classification dataset, consisting of
70000 handwritten digits in the format of $28\times28$ binary pixel
photos, with a train-validation split of $6:1$. As a preprocessing
step, we reshape each two-dimensional datapoint into a $784$-dimensional
vector. As the design matrix is rank-deficient due to linear dependency
and duplicate rows, we select the subset of linearly independent columns,
and also perturb the entries with iid Gaussian noise with standard
deviation 0.01. The resulting design matrix has a condition number
of $73288.03$, i.e. a very ill-conditioned system. Applying the optimal
diagonal preconditioner yields a design matrix with condition number
$102.27$, a significant reduction. To assess the convergence speeds
of gradient and stochastic gradient descent methods, we run multinomial
logistic regression with cross-entropy loss, $f(\theta)=\frac{1}{n}\sum_{i=1}^{n}-\log p_{i}^{y_{i}}$
where $p_{i}^{k}$ is the probability of the $k$-th class of the
$i$th sample, predicted by the model: $p_{i}^{k}=\frac{\exp(\theta_{k}^{T}x_{i})}{\sum_{k=1}^{K}\exp(\theta_{k}^{T}x_{i})}$,
with the descent direction given by $\nabla_{\theta_{k}}f(\theta)=-\frac{1}{n}\sum_{y_{i}=k}x_{i}+\frac{1}{n}\sum_{i}\frac{x_{i}\exp(\theta_{k}^{T}x_{i})}{\sum_{k=1}^{K}\exp(\theta_{k}^{T}x_{i})}$.

Because the problem is non-convex, we declare convergence when the
number of iterations reached a maximum value, or when the norm of
gradient drops below the threshold $0.001$. We then report the log-gap
$\log(f(\theta)-f(\theta^{\ast}))$ of the various methods, where
$\theta^{\ast}$ is a pre-computed optimal solution. 

\begin{table}
	\begin{centering}
		\begin{tabular}{|c|c|c|}
			\hline 
			$(n,p)$ & \multicolumn{1}{c|}{iterations} & \multicolumn{1}{c|}{log-gap}\tabularnewline
			\hline 
			No preconditioning & 2000 & -2.74\tabularnewline
			\hline 
			Fixed preconditioning & 1823 & -2.90\tabularnewline
			\hline 
			Optimal preconditioning & 1503 & -3.12\tabularnewline
			\hline 
			Batch normalization & 1621 & -3.35\tabularnewline
			\hline 
		\end{tabular}
		\par\end{centering}
	\caption{Number of iterations till convergence of diagonal preconditioning
		methods for gradient descent and the log-gap at convergence. We see
		that while the log-gaps are comparable among the three diagonal conditioners,
		the number of iterations required is the smallest for optimal diagonal
		preconditioner. }
\end{table}
We see that while the log-gaps are comparable among the three diagonal
conditioners, the number of iterations required till convergence is
the smallest for optimal diagonal preconditioner. All methods are
able to achieve a test accuracy of at least 88\%. 

\section{Conclusion}

In this paper, we studied diagonal preconditioning and its impact
on the condition number and convergence speed of linear systems and
quadratic and general convex optimization problems. We first showed
that the popular preconditioning technique of normalization by column
standard deviation/norm reduces the condition number of the design
matrix $X$ by $\sqrt{\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}}$
for $X$ with independent sub-Gaussian rows and convariance matrix
$\Sigma$, where $D=\text{diag}(\Sigma)$. We then gave a diagonal
dominance condition that guarantees that this reduction is large.
Next, for any fixed design matrix, we developed bisection and interior
point algorithms that guarantee a diagonal preconditioner that reduces
the condition number of the preconditioned matrix, with $O(\frac{1}{\epsilon})$
iteration complexity, and each iteration consists of an SDP feasibility
problem or a Newton update step with Nesterov-Todd directions. These
results have direct implications for the effect of preconditioning
on speeding up the convergence of iterative algorithms for linear
systems and first order methods for quadratic optimization problems,
as the linear convergence rates have explicit dependence on the condition
number. For general convex optimization problems, it is less clear
how improvements in the condition number of the design matrix translate
into speedup of first order methods. We showed that for a particular
class of strongly convex and smooth objectives, the reduction in the
condition number of the objective function enjoys the same order $\sqrt{\frac{\kappa(\Sigma)}{\kappa(D^{-\frac{1}{2}}\Sigma D^{-\frac{1}{2}})}}$
of reduction as that of the design matrix. Finally, we established
connections of batch normalization to adaptive preconditioning, and
extended our optimal diagonal preconditioning algorithm to an adaptive
setting compatible with stochastic first order methods. Numerical
experiments on real and simulated datasets with regression and classification
tasks show that the optimal diagonal preconditioner speeds up convergence
compared to preconditioning with heuristics such as column standard
deviation, and is comparable to the performance of batch normalization.
On the other hand, batch normalization does not seem to reduce the
effective condition number of the system, so its mechanism of speeding
up convergence remains to be investigated further. 

==> major revision/experiments.tex <==
\section{Numerical Experiments}
\label{sec:experiments}

% \setlength{\parindent}{0pt}

To empirically validate the performance of the optimal two-sided preconditioners discussed in Section \ref{sec:optimal} and the optimal one-sided preconditioners via the
dual SDP approach in Section \ref{sec:DSDP}, we conduct
extensive numerical experiments over \texttt{SuiteSparse},
\texttt{LIBSVM} and large machine learning datasets from
\texttt{OPENML}.\footnote{Code and detailed results can be found in the Github repository at \href{https://github.com/Gwzwpxz/opt\_dpcond}{https://github.com/Gwzwpxz/opt\_dpcond}} For the sake of brevity, given a matrix $A$, recall that we refer to $D_1^{1/2}A$, $AD_2^{-1/2}$ and $D_1^{1/2}AD_2^{-1/2}$ as the left, right, and two-sided preconditionings, respectively.

\subsection{Experimental Setup}

We first describe our experiment setup and implementation details.

\paragraph{Dataset.}
We use matrices from the following sources:
\begin{itemize}
  \item Tim Davis \texttt{SuiteSparse} Dataset \citep{kolodziej2019suitesparse}
  
  \item \texttt{LIBSVM} \citep{chang2011libsvm}
  
  \item \texttt{OPENML} Machine Learning Dataset Repository  \citep{rijn2013openml}

 \item Randomly generated dataset
\end{itemize}

\paragraph{Data Generation, Selection, and Processing.}
For \texttt{LIBSVM} and \texttt{OPENML}, we select their
regression datasets. Given a matrix $A$, when doing right preconditioning, if $M = A^T A$ is available, we compute $\kappa (M)$, and if it is too large, we regularize it setting $M \leftarrow M + \varepsilon I$ with $\varepsilon$ large enough such that
$\kappa (M) \leq 10^8$. This is to ensure that the associated dual SDPs are solvable by \texttt{HDSDP}. No processing is done for left or two-sided preconditionings, and if the solver fails due to ill-conditioning, we drop the matrix. For randomly generated data, we obtain their nonzero entries from $\mathcal{N} (0, 1)$.

\paragraph{Matrix Statistics.} We take matrices of different sizes from the three external
sources and record their statistics below. Details on \texttt{SuiteSparse} can be found in the Github repository.

\begin{itemize}
  \item \texttt{SuiteSparse}. We choose 391 matrices with $m, n \leq 1000$.
  
  \item \texttt{LIBSVM}. We summarize the sizes of the matrices below.
  
  \begin{table}[h]
  \centering
    \begin{tabular}{cccccc}
      \hline
      Matrix & $m$ & $n$ & Matrix & $m$ & $n$\\
            \hline
      YearPredictionMSD & 463715 & 90 & eunite2001.txt & 336 & 16\\
      YearPredictionMSD.t & 51630 & 90 & housing\_scale.txt & 506 & 13\\
      abalone\_scale.txt & 4177 & 8 & mg\_scale.txt & 1385 & 6\\
      bodyfat\_scale.txt & 252 & 14 & mpg\_scale.txt & 392 & 7\\
      cadata.txt & 20640 & 8 & pyrim\_scale.txt & 74 & 27\\
      cpusmall\_scale.txt & 8192 & 12 & space\_ga\_scale.txt & 3107 & 6\\
      eunite2001.t & 31 & 16 & triazines\_scale.txt & 186 & 60\\
      \hline
    \end{tabular}
    \caption{\texttt{LIBSVM} datasets}
  \end{table}
  \item \texttt{OPENML.} We selected the following three datasets summarized in Table \ref{tab:OPENML}.
  \begin{table}[h]
  \centering
    \begin{tabular}{ccc}
      \hline
      Matrix & $m$ & $n$\\
      \hline
      MNIST & 70000 & 784\\
      credit & 284807 & 29\\
      IMDB & 120919 & 1001\\
      \hline
    \end{tabular}
    \caption{\texttt{OPENML} datasets}
    \label{tab:OPENML}
  \end{table}
\end{itemize}

\paragraph{Subproblem Solution.}
In the experiments for right preconditioning, we adopt \texttt{HDSDP} with and without random sampling for the SDPs; for left preconditioning, we adopt \texttt{HDSDP} without random sampling;
to compute the two-sided preconditioner using bisection, we employ the better option between \texttt{Sedumi} and \texttt{SDPT3} for the feasibility problems.

\paragraph{Evaluation and Performance Metrics.} We report different statistics and metrics for the three types of preconditioning problems.

\textbf{R}ight preconditioning:

\begin{enumerate}[label={R\arabic*:},leftmargin=40pt]
  \item $\kappa (M)$: Condition number of $M=A^TA$
  
  \item $\kappa (D_2^{- 1 / 2} M D_2^{- 1 / 2})$: Condition number after optimal right preconditioning
  
  \item $\kappa (D_M^{- 1 / 2} M D_M^{- 1 / 2})$ : Condition number after Jacobi preconditioning $D_M=\text{diag}(M)$
  
  \item Improvement: Relative improvement in condition number $
  \frac{\kappa(M)}{\kappa (D_2^{- 1 / 2} M D_2^{- 1 / 2})}$
  \item Time: The CPU time spent solving the SDP problem
\end{enumerate}

\textbf{L}eft preconditioning:
\begin{enumerate}[label={L\arabic*:},leftmargin=40pt]
  \item $\kappa (M)$: Condition number of $M=A^TA$
  \item $\kappa (A^T D_1 A)$: Condition number after optimal left preconditioning  
  \item Improvement: Relative improvement in condition number $
  \frac{\kappa(M)}{\kappa (A^T D_1A)}$
  \item Time: The CPU time spent solving the SDP problem
\end{enumerate}

\textbf{T}wo-sided preconditioning:
\begin{enumerate}[label={T\arabic*:}, leftmargin=40pt]
  \item $\kappa (M)$: Condition number of $M=A^TA$
  \item $\kappa(D_2^{- 1 / 2}  A^T D_1A D_2^{- 1 / 2}) $: Condition number after optimal two-sided preconditioning  
  \item Improvement: Relative improvement in condition number $
  \frac{\kappa(M)}{\kappa(D_2^{- 1 / 2}  A^T D_1A D_2^{- 1 / 2})}$
  \item $\kappa(D_{R_1}^{- 1 / 2}  A^T D_{R_2}A D_{R_1}^{- 1 / 2}) $: Condition number after $\ell_\infty$-Ruiz preconditioning \citep{ruiz2001scaling}
%   \item Time: The CPU time spent in bisection
\end{enumerate}

For convenience, we sometimes use Cbef, Caft to denote condition number of a matrix before and after preconditioning.

\paragraph{Conjugate Gradient Solver.}
We adopt the \texttt{MATLAB pcg} function to test the efficacy of different preconditioners at speeding up CG. The relative tolerance is set to $10^{-6}$, starting from the all-zero vector, and the right-hand-side vector is generated with a fixed random seed. When comparing the conjugate gradient method against the direct solvers, we also adopt a relative tolerance of $10^{-6}$.

\paragraph{Environment.} All experiments in this paper are carried out using \texttt{MATLAB} on
Mac Mini with Apple Silicon and 16 GB memory. The \texttt{HDSDP} solver is
implemented in \texttt{ANSI C}.

\subsection{Experiment Results for Right Preconditioning}

Our experiments for right preconditioning are into three parts. In the first part, we consider exact optimal preconditioning without randomly sampling rows of a matrix to explore the advantage of optimal preconditioners over preconditioning by the diagonal of a matrix (the Jacobi preconditioner).
In particular, we give an example where diagonal
preconditioning fails completely, but our optimal right preconditioner greatly reduces the condition number. In the
second part, we validate our randomization scheme using large realistic
regression datasets. In particular, we demonstrate that solving the dual SDP based on a sub-sampled matrix generally produces high quality approximate preconditioners for the original matrix, which has important practical implications. In the third part, we explore some cases where the time to
set up $A^T A$ is dominant, but our dual SDP approach based on random sampling can still find near-optimal preconditioners efficiently.

\paragraph{Preconditioning Evaluation.}
In this part of the experiment, we use $A$ to construct the pre-conditioner without randomly sampling its rows. The detailed results for each matrix are available in the Github repository. Here we record the summary statistics for \texttt{SuiteSparse} in Table \ref{tab:suite-right}. Note that ``improvement'' is defined as $
  \frac{\kappa(M)}{\kappa (D_2^{- 1 / 2} M D_2^{- 1 / 2})}$, so that, e.g., an improvement equal to 2 corresponds to a 2-fold improvement in the condition number.
\begin{table}[h]
\centering
  \begin{tabular}{c|c}
    \hline
    Improvement & Number\\
    \hline
    $\geq$5.00 & 121\\
    % \hline
    $\geq$2.00 & 190\\
    % \hline
    $\geq$1.25 & 261\\
    \hline
  \end{tabular}\quad\begin{tabular}{r|c}
    \hline
    Median imp. & 2.17 \\
    \hline
    Median imp. over Jacobi & 1.49 \\
    \hline
    Average time & 1.29\\
    \hline
  \end{tabular}
  \caption{Summary for right preconditioning on the \texttt{SuiteSparse} dataset}
  \label{tab:suite-right}
\end{table}

As the results suggest, the dual SDP approach improves the condition number of half of the matrices by at least a factor of 2.00, and the median of the improvement is 1.49. Additionally, in Figure \ref{fig:reduction-pdf}, we plot the distribution of improvements in condition numbers for \texttt{SuiteSparse} matrices from optimal preconditioners. Moreover, compared to the baseline (Jacobi) diagonal preconditioning, the optimal preconditioning
achieves a further median improvement of 1.29. See Figure \ref{fig:comparison} for the distribution of improvements over Jacobi preconditioning. Among the \texttt{SuiteSparse} datasets, we also find a large sparse
matrix \texttt{m3plates}, whose condition number diverges after
Jacobi preconditioning, while our optimal preconditioning reduces the condition number to
close to 1.

\begin{figure}
    \centering
    \includegraphics[scale=0.175]{figs/pdf_right_over_none.pdf}
    \includegraphics[scale=0.175]{figs/pdf_left_over_none.pdf}
    \includegraphics[scale=0.175]{figs/pdf_two_over_none.pdf}
    \caption{Distribution of logarithm of condition number improvements achieved by optimal right, left, and two-sided preconditioners on \texttt{SuiteSparse} matrices, respectively}
    \label{fig:reduction-pdf}
\end{figure}

\begin{table}[h]
\centering
  \begin{tabular}{ccccccc}
    \hline
    Mat & Size & Cbef & Caft & Cdiag & Imp. & Time\\
    \hline
    m3plates (perturbed) & 11107 & 2.651e+04 & 1.02 & $\infty$ & $>10^4$ &
    492.1\\
    \hline
  \end{tabular}
  \caption{A special example from \texttt{SuiteSparse}}
\end{table}
%\vspace{-0.8cm}
\paragraph{Randomized Sampling.}
In this part, we demonstrate the effectiveness of the randomization procedure on four large
real regression datasets from \texttt{LIBSVM} and \texttt{OPENML}. We summarize the results in Figure \ref{fig:sampling}.
The $x$-axis always indicates the sub-sampling ratio $\tilde{m} / m$; the red line plots $\|
A^T A - \tilde{A}^T \tilde{A} \|$ and the blue line plots the condition number
of the preconditioned matrix, using optimal right preconditioners for $A$ based on solving the dual SDP problems for the \emph{sub-sampled} matrix $\tilde A$.

\begin{figure}[h]
\centering
{\includegraphics[scale=0.22]{figs/YearPredictionMSD.pdf}}{\includegraphics[scale=0.22]{figs/YearPredictionMSD.t.pdf}}{\includegraphics[scale=0.22]{figs/mnist.pdf}}{\includegraphics[scale=0.22]{figs/credit.pdf}}
  \caption{Preconditioning with sampling on
  \texttt{YearPredictionMSD}, \texttt{YearPredictionMSD.t},
  \texttt{MNIST} and \texttt{credit} \ }
  \label{fig:sampling}
\end{figure}
\vspace{-1cm}
As the results suggest, we generally only need to randomly sample 1\% to 10\% of the rows of the original matrix $A$ in order to give
a good preconditioner for the iterative solvers. This greatly extends the
applicability of our proposed approach via solving dual SDPs, since we can efficiently find high quality right preconditioners for matrices of size 50,000 or larger (280,000 in the case of the credit dataset in \texttt{OPENL}) via random row sampling.

\paragraph{Extreme Cases} In this part, we provide random instances where the time to set up $A^TA$ is dominant and our preconditioning procedure with random row sampling can significantly reduce the condition number efficiently with less computation time.
\begin{table}[h]
\centering
  \begin{tabular}{cccccc}
    \hline
    $m$ & $n$ & Time of $A^T A$ & Time of $\tilde{A}^T \tilde{A}$ +
    computing $D_2^{-1 / 2}$  & Cbef & CAft \\
    \hline
    $10^7$ & 5 & 0.053 & 0.0004 + 0.0250 & 9.9844e+05 & 5.4020\\
    $10^7$ & 10 & 0.0999 & 0.0006 + 0.0500 & 9.9968e+05 & 1.0713\\
    $10^7$ & 20 & 0.6589 & 0.0024 + 0.4564 & 9.9889e+05 & 1.1500\\
    \hline
  \end{tabular}
  \caption{Some large random instances where randomization is efficient}
\end{table}
\subsection{Experiment Results for Left Preconditioning}
Our experiments for left preconditioning mainly focus on evaluating the reduction in condition number from left preconditioning. Since we cannot use the regularization $M+\varepsilon I$ for extremely ill-conditioned matrices as we do in right preconditioning, we present the results on 89 matrices whose associated dual SDP problems \eqref{eq:DSDP-left} are solved successfully by our solver. The summary statistics are given in Table \ref{tab:suite-left}. Detailed results can be found in the online repository.

\begin{table}[H]
\centering
  \begin{tabular}{c|c}
    \hline
    Improvement & Number\\
    \hline
    $\geq$5.00 & 31\\
    % \hline
    $\geq$2.00 & 55\\
    % \hline
    $\geq$1.25 & 81\\
    \hline
  \end{tabular}\quad\begin{tabular}{r|c}
    \hline
    Median imp. & 2.51 \\
    \hline
    Average time & 1.10\\
    \hline
  \end{tabular}
  \caption{Summary for left preconditioning on the \texttt{SuiteSparse} dataset}
  \label{tab:suite-left}
\end{table}
\vspace{-0.8cm}
Compared to right preconditioning, the dual SDPs for left preconditioning are more sensitive to the original data matrix $A$. Still, we also observe remarkable reductions in condition numbers on more than half of the tested matrices. See Figure \ref{fig:reduction-pdf} for the distribution of improvements.

\subsection{Experiment Results for Two-sided Preconditioning}
Our experiments for two-sided preconditioning compare the performance of our optimal two-sided preconditioners to the popular two-sided preconditioners based on the Ruiz scaling method \citep{ruiz2001scaling}. Since computing the two-sided preconditioner involves solving several feasibility SDPs, we restrict our attention to smaller matrices. See Table \ref{tab:two-sided} for summarized results.%, and Github repository for detailed experimental results for each matrix. 

\begin{figure}
    \centering
    \includegraphics[scale=0.18]{figs/pdf_right_over_jacobi.pdf}
    \includegraphics[scale=0.18]{figs/pdf_two_over_ruiz.pdf}
    \caption{Comparison of log condition number improvements achieved by optimal right and two-sided preconditioners over baseline preconditioners on \texttt{SuiteSparse} matrices}
    \label{fig:comparison}
\end{figure}

\begin{table}[h]
\centering
  \begin{tabular}{c|c}
    \hline
    Improvement & Number\\
    \hline
    $\geq$5.00 & 18\\
    % \hline
    $\geq$2.00 & 35\\
    % \hline
    $\geq$1.25 & 43\\
    \hline
  \end{tabular}\quad\begin{tabular}{r|c}
    \hline
    Median imp. & 3.60 \\
    \hline
    Median imp. over Ruiz & 2.10 \\
    \hline
  \end{tabular}
  \caption{Summary for two-sided preconditioning on the \texttt{SuiteSparse} dataset}
  \label{tab:two-sided}
\end{table}
%\vspace{-0.8cm}
As the experiment results suggest, the optimal two-sided diagonal preconditioners work at least as well as the Ruiz scaling and, on average, an improvement of over 30\% is observed on the tested data. Moreover, the two-sided preconditioners also achieve more significant improvements in condition number compared to one-sided preconditioners (see repository for detailed comparisons). Interestingly, the Ruiz scaling does not improve much on the condition number at all for many instances. This suggests that may be room for significant improvements over current practices.
%(see Table \ref{tab:two-sided-comparison} in Appendix \ref{app:two-sided} for detailed comparisons).
%\textbf{Distribution of condition number reduction}
%The following are three figures that plot the distribution (pdf.) of the reduction of condition number of matrices.

\begin{comment}
The following figure integrates the above three figures into one.
\begin{figure}
    \centering
    \includegraphics[scale=0.6]{major revision/figs/pdf_all.pdf}
    \caption{Three pdfs integrated}
    \label{fig:my_label}
\end{figure}
\end{comment}

\subsection{Experiment Results for Iterative Methods}

In this section, we evaluate the practical efficiency of our optimal preconditioner at speeding up iterative methods. We focus on the right-preconditioners whose improvements are greater than 2 and use the number of preconditioned conjugate gradient iterations as the evaluation metric.
The testing matrices are selected such that $\kappa (D_2^{- 1 / 2} M D_2^{- 1 / 2}) \ll \kappa (D_M^{- 1 / 2} M D_M^{- 1 / 2})$. We end up with a collection of 148 matrices. In Table \ref{tab:iterative-comparison}, we report the number of instances for which the optimal and
the baseline Jacobi preconditioners perform better.
\begin{table}[h]
\centering
\begin{tabular}{r|c}
    \hline
    Preconditioner & \# of instances\\
    \hline
    Jacobi & 46\\
    \hline
    Optimal & 102\\
    \hline
    Total & 148\\
    \hline
  \end{tabular}
  \caption{Instances where each preconditioning technique yields fastest convergence}
  \label{tab:iterative-comparison}
\end{table}
Figure \ref{fig:iterative-comparison} illustrates the relative improvements in terms of number of iterations using optimal diagonal preconditioners over Jacobi preconditioners.
\begin{figure}
    \centering
    \includegraphics[scale=0.3]{figs/pdf_iter.pdf}
    \caption{Improvements in iteration numbers of the preconditioned conjugate gradient method on the testing collection using optimal right diagonal preconditioners vs. Jacobi preconditioners}
    \label{fig:iterative-comparison}
\end{figure}

%\textbf{Remark.} Due to current limits on testing matrix sizes, our numerical experiments suggest that condition number of the un-preconditioned matrix is benign and PCG without pre-conditioning is sometimes a better choice. Since we focus on the comparison between preconditioners, the un-preconditioned case is not present in this section.

\subsection{Comparing Iterative and Direct Methods}
In this section, we further test the applicability of optimal preconditioners to iterative methods as a potential substitute for sparse direct methods, especially if we need to solve linear systems with identical LHS matrix and varying RHSs. We simulate the scenario, given a matrix $A$, as follows: 
\begin{enumerate}
    \item Compute the optimal diagonal left/right preconditioner and explicitly evaluate the pre-conditioned matrix.
    \item Compute the symbolic ordering $P$ and factorize $P^TA^TAP= LL^T$.
\end{enumerate}
Since the time of the above two operations can be amortized by the large number of solves, we exclude them from our time statistics. Also, we explicitly compute the preconditioned matrix since 1) diagonal preconditioners have no impact on the sparsity pattern of the matrix, and 2) computational time for the preconditioning step is amortized.

Then 12800 linear systems with identical LHSs are solved and the time statistics for both sparse and direct methods are collected. In our setup, we adopt the native routine from \texttt{MATLAB} to perform forward/backward substitution and the \texttt{Intel MKL Reverse Communication Interface} to implement the CG solver. We found that in 35 instances, right optimally preconditioned iterative solvers are faster than direct solvers, and in 14 instances left optimally-conditioned preconditioners are faster than direct solvers. See the Github repository for detailed experimental results. Even though our primary focus is on maximal condition number reduction with diagonal preconditioners, we have demonstrated that they can also speed up iterative methods significantly and, in some cases, outperform sparse direct methods on instances from \texttt{SuiteSparse}.
%After going through 408 matrices from the SuiteSparse collection, we finally arrive at 18 of them where the preconditioned iterative solvers outperform direct solvers. 
\begin{comment}

\begin{table}[h]
\centering
  \begin{tabular}{cc|cc|ccc}
    \hline
    Matrix & Size & $\kappa_M$ & $\kappa_{D_2^{- 1 / 2} A^TA D_2^{- 1 / 2}}$ &
    $T_{\text{CG}}$ & $T_{\text{Direct}}$ & Imp.\\
    \hline
    ash219 & 85 & 9.1e+00 & 4.1e+00 & 0.05 & 0.07 & 1.43\\
    ash331 & 104 & 9.5e+00 & 3.6e+00  & 0.58 & 0.66 & 1.14\\
    bcsstm01 & 48 & 7.7e+07 & 1.0e+00 & 0.02 & 0.04 & 2.41\\
    bcsstm02 & 66 & 7.6e+01 & 1.0e+00 & 0.02 & 0.04 & 2.09\\
    bcsstm03 & 112 & 5.5e+07 & 1.0e+00 & 0.03 & 0.05 & 1.81\\
    bcsstm04 & 132 & 2.9e+04 & 1.0e+00 & 0.03 & 0.05 & 1.63\\
    bcsstm05 & 153 & 1.6e+02 & 1.0e+00 & 0.03 & 0.05 & 1.54\\
    bcsstm06 & 420 & 5.5e+07 & 1.0e+00 & 0.07 & 0.09 & 1.16\\
    bcsstm22 & 138 & 8.8e+05 & 1.0e+00 & 0.03 & 0.05 & 1.58\\
    can{2}4 & 24 & 6.0e+03 & 4.0e+03 & 0.04 & 0.04 & 1.02\\
    GlossGT & 72 & 2.9e+07 & 3.6e+01 & 0.05 & 0.06 & 1.14 \\ 
    mesh1e1 & 48 & 2.7e+01 & 1.5e+01 & 0.05 & 0.05 & 1.01\\
    Stranke94 & 10 & 2.6e+03 & 2.3e+03 & 0.02 & 0.03 & 1.88\\
    Tina{A}skCog & 11 & 3.9e+02 & 2.4e+02 & 0.02 & 0.03 & 1.88\\
    Tina{D}isCal & 11 & 2.2e+07 & 2.0e+02 & 0.02 & 0.03 & 1.88\\
    Trefethen20b & 19 & 9.2e+02 & 8.6e+00 & 0.03 & 0.04 & 1.37\\
    Trefethen20 & 20 & 3.9e+03 & 2.8e+01 & 0.03 & 0.04 & 1.27\\
    mycielskian4 & 11 & 9.3e+01 & 8.4e+01 & 0.02 & 0.04 & 2.05\\
    mycielskian5 & 23 & 7.6e+02 & 6.1e+02 & 0.03 & 0.04 & 1.25\\
    odepb400 & 400 & 1.0e+00 & 1.0e+00 & 0.07 & 0.08 & 1.14\\
  lpi\_galenet &  14 & 5.8e+06 & 5.3e+06 & 0.02 & 0.03 & 1.50\\
   lpi\_itest2 &  13 & 1.7e+07 & 5.9e+06 & 0.02 & 0.03 & 1.50\\
   lpi\_itest6 &  17 & 1.1e+07 & 6.5e+06 & 0.04 & 0.04 & 1.00\\
     lp\_nug05 & 225 & 9.4e+06 & 9.4e+06 & 0.20 & 0.27 & 1.35\\
     lp\_nug06 & 486 & 5.8e+06 & 5.8e+06 & 0.48 & 1.05 & 2.19\\
         LF10 &  18 & 5.1e+07 & 4.9e+04 & 0.03 & 0.04 & 1.33\\
     football &  35 & 2.9e+07 & 2.8e+05 & 0.04 & 0.05 & 1.25\\
       GD01\_b &  18 & 5.5e+06 & 3.2e+06 & 0.03 & 0.04 & 1.33\\
       GD95\_a &  36 & 1.2e+07 & 5.9e+06 & 0.03 & 0.04 & 1.33\\
       GD96\_b & 111 & 7.4e+07 & 4.0e+06 & 0.06 & 0.06 & 1.00\\
      GlossGT &  72 & 2.9e+07 & 3.6e+01 & 0.04 & 0.05 & 1.25\\
     Ragusa18 &  23 & 4.8e+07 & 5.2e+06 & 0.03 & 0.04 & 1.33\\
  Tina\_AskCal &  11 & 1.2e+07 & 4.4e+06 & 0.02 & 0.03 & 1.50\\
     klein-b1 &  10 & 1.0e+07 & 8.5e+06 & 0.02 & 0.03 & 1.50\\
     football &  35 & 2.9e+07 & 2.8e+05 & 0.04 & 0.05 & 1.25\\
    \hline
  \end{tabular}
  \caption{Cases where iterative methods are faster (Right-preconditioning) }
\end{table}

\begin{table}[h]
\centering
  \begin{tabular}{cc|cc|ccc}
    \hline
    Matrix & Size & $\kappa_M$ & $\kappa_{{A^T D_1 A}}$ &
    $T_{\text{CG}}$ & $T_{\text{Direct}}$ & Imp.\\
    \hline
            ash219  &  219 & 9.1e+00 & 4.5e+00 & 0.04 & 0.06 & 1.27 \\
        ash331  &  331 & 9.5e+00 & 3.6e+00 & 0.05 & 0.06 & 1.15 \\
      bcsstm02  &   66 & 7.6e+01 & 1.0e+00 & 0.02 & 0.04 & 2.25 \\
      bcsstm05  &  153 & 1.6e+02 & 1.0e+00 & 0.03 & 0.05 & 1.57 \\
      bcsstm22  &  138 & 8.8e+05 & 8.3e+02 & 0.04 & 0.05 & 1.08 \\
         ibm32  &   32 & 1.6e+05 & 1.0e+05 & 0.04 & 0.04 & 1.02 \\
        pivtol  &  102 & 1.2e+04 & 1.0e+01 & 0.05 & 0.06 & 1.25 \\
         cage5  &   37 & 2.3e+02 & 3.6e+01 & 0.04 & 0.04 & 1.04 \\
     Stranke94  &   10 & 2.6e+03 & 2.3e+03 & 0.01 & 0.03 & 1.77 \\
   Tina\_AskCog  &   11 & 3.9e+02 & 2.8e+02 & 0.01 & 0.03 & 1.77 \\
 Trefethen\_20b  &   19 & 9.2e+02 & 8.6e+00 & 0.02 & 0.03 & 1.28 \\
  Trefethen\_20  &   20 & 3.9e+03 & 2.8e+01 & 0.03 & 0.03 & 1.20 \\
  mycielskian4  &   11 & 9.3e+01 & 8.4e+01 & 0.01 & 0.03 & 2.06 \\
  mycielskian5  &   23 & 7.6e+02 & 6.1e+02 & 0.03 & 0.03 & 1.15 \\
    \hline
  \end{tabular}
  \caption{Cases where iterative methods are faster (Left-preconditioning) }
\end{table}
\end{comment}

\subsection{Scalability of the Dual SDP Approach}

To conclude this section, we make a few remarks on the scalability of our dual SDP
solver in solving optimal diagonal preconditioning problems for $A \in \mathbb{R}^{m \times n}$ %$D_1^{1 / 2} A D_2^{- 1 / 2}, A \in \mathbb{R}^{m \times n}$ 
as a reference for practical
use.
\begin{enumerate}[leftmargin=15pt]
  \item The complexity (or CPU time) of the three SDP formulations ranks as
  Two-sided $\gg$ Left $\geq$ Right, where $=$ holds if $m \approx n$. Correspondingly, the reduction in condition number ranks as Two-sided $>$
  Right $\approx$ Left. 
  
  Although two-sided scaling is most powerful and results in the greatest
  reduction in condition numbers, its high computation cost restricts its use
  to matrices with $\max \{ m, n \} \leq 300$. But as our computational
  experience suggests, left or right preconditioners suffice in most cases.
  
  \item Left and Right preconditioners benefit from sparsity.
  
  If $A$ is extremely sparse, SDP solvers could exploit this to accelerate the solution of the dual SDPs \eqref{eq:DSDP-right} and \eqref{eq:DSDP-left}. In our experiments, sparsity makes it possible to compute preconditioners of
  a $10000 \times 10000$ matrix very efficiently. In general cases, solvers of the dual SDP \eqref{eq:DSDP-left} for left
  preconditioners can handle matrices $A \in \mathbb{R}^{m \times n}$ satisfying $\max \{ m, n \} \leq 2000$ and solvers of the dual SDP \eqref{eq:DSDP-right} for
  right preconditioners can handle cases where $n \leq 5000$.
  
  \item Right preconditioners benefit from statistical properties.
  
  If the rows of $A$ are generated from some statistical distribution, as is the case for data matrices in practice, then right preconditioners can
  handle very tall matrices with large $m$ quite efficiently using the aforementioned random sampling
  procedure. Especially when $m \gg n =\mathcal{O} (1)$, a right
  preconditioner with high quality can be found even faster than computing $A^T A$.
\end{enumerate}

\section{Concluding Remarks}
In this paper, we study the problem of optimal diagonal preconditioning for any matrix $A$ with full rank. More precisely, the goal is to achieve maximal condition number reduction of $A$ by scaling its rows and/or columns. This problem is relevant to the optimization and OR community both from a scientific standpoint and from a practical standpoint. First, as existing popular diagonal preconditioners often do not have guarantees on condition number reductions, it is important to know to what extent we may improve upon existing heuristics-based diagonal preconditioners. Second, since condition numbers often affect the convergence speed of algorithms, we are interested in efficient methods to find near optimal diagonal preconditioners for large systems, so that they could be applied to speed up the convergence. Starting from a quasi-convex reformulation of the general two-sided optimal diagonal preconditioning problem, we provide bisection and interior point algorithms based on potential reduction, which are also applicable to other quasi-convex problems with PSD matrix variables. Specializing to one-sided optimal diagonal preconditioning problems, we demonstrate they are equivalent to standard dual SDP problems with sparse and low rank structures. We then develop efficient customized solvers incorporating randomization, which are able to handle problems of size as large as 200,000 efficiently. Based on our extensive experiments, we demonstrate that there is indeed a large room of improvement over existing diagonal preconditioners in terms of condition number reduction. Moreover, on large real datasets, our optimal diagonal preconditioners with customized solvers are shown to improve over heuristic preconditioners at speeding up iterative methods and can also outperform sparse direct methods when the problem requires solving linear systems with identical LHS and multiple RHSs. Although the computational overhead of finding optimal diagonal preconditioners is a potential concern, many modern optimization settings can benefit from optimal diagonal preconditioners of smaller subsystems, such as in ADMM or Federated Learning, or a system that needs to be repeatedly solved, such as preconditioned CG in the Newton step of interior point methods or solving multi-scale numerical PDEs. We therefore see our results as both theoretically and scientifically interesting, and also practically relevant to problems that may benefit from better preconditioning. %Because we took a general approach that finds optimal diagonal preconditioners for any matrix, an interesting future direction is to improve the efficiency of finding such preconditioners for problems with special structures, such as sparse or near-diagonal matrices.

==> major revision/first-order-methods.tex <==
\section{First Order Methods for Optimal Diagonal Preconditioning}
\label{sec:first-order-methods}
In this section, we briefly discuss two first order algorithms for finding (right) optimal diagonal preconditioners that do not rely on solving SDPs with Newton updates. They can be easily generalized to the two-sided problem. Their feasibilities have been confirmed in numerical experiments on small matrices, although we leave their customization and optimization on larger problems to future works.

\subsection{A Projected Sub-gradient Descent Algorithm}

To find an optimal (right) diagonal preconditioner for a positive definite
matrix $M=A^TA$, we propose to use projected subgradient descent to solve
the following problem:
\begin{align*}
\min\log(\kappa(DMD))\\
D\succeq I\\
C\succeq D
\end{align*}
 where, for some pre-specified large $C$, the projection step simply
truncates the updated $D_{k}$ at the $k$-th step by an upper bound
$C$ and lower bound $1$. The computation of the subgradient is simple
for this problem, since for the largest eigenvalue $\lambda_{\max}(X)$
of a matrix $X$ and any eigenvector $v$ associated with $\lambda_{\max}(X)$,
$vv^{T}\in\partial\lambda_{\max}(X)$, and similarly $uu^{T}\in\partial(\lambda_{\min}(X))$
for any eigenvector $u$ associated with $\lambda_{\min}(X)$. Thus,
\begin{align*}
(\frac{v(DMD)v^{T}(DMD)}{\lambda_{\max}(DMD)}\times MD)\cdot\mathbf{1}+\mathbf{1}^{T}\cdot(DM\times\frac{v(DMD)v^{T}(DMD)}{\lambda_{\max}(DMD)}) & \in\partial_{D}\log\lambda_{\max}(DMD)\\
(\frac{u(DMD)u^{T}(DMD)}{\lambda_{\min}(DMD)}\times MD)\cdot\mathbf{1}+\mathbf{1}^{T}\cdot(DM\times\frac{u(DMD)u^{T}(DMD)}{\lambda_{\min}(DMD)}) & \in\partial_{D}(\log\lambda_{\min}(DMD))
\end{align*}
where $\times$ is the entry-wise matrix multiplication and $\cdot$
is the usual matrix-vector multiplication. The update at the $k$-th
step is then
\begin{align*}
D_{k}-\alpha_{k}(\mathbf{1}^{T}\cdot D_{k}M\times P_{k}+P_{k}\times MD_{k}\cdot\mathbf{1})\\
P_{k}=\frac{v(DMD)v^{T}(DMD)}{\lambda_{\max}(DMD)}-\frac{u(DMD)u^{T}(DMD)}{\lambda_{\min}(DMD)}
\end{align*}
Extreme eigenvectors and eigenvalues in the subgradient can be efficiently computed with the Lanczos algorithm \citep{lanczos1950iteration}.
For step sizes, we can choose $\alpha_{k}=1/k$ or $\alpha_{k}=1/\sqrt{k}$. The corresponding projected sub-gradient algorithms for left and two-sided preconditionings can be derived similarly.

\subsection{A First-Order Potential Reduction Algorithm}
Recall the potential reduction algorithm introduced in Section \ref{sec:optimal}, which aims to minimize the following potential function:
\begin{align*}
P(\kappa) =\max_{D\succeq0} & \log\det(M-D)+\log\det(\kappa D-M)+\log\det D
\end{align*}
As an alternative to Algorithms \ref{alg:exact} and \ref{alg:approximate} which are based on Newton updates with Nesterov-Todd directions, we suggest to achieve potential reduction using projected alternating gradient descent-ascent on the following min-max objective: 
\begin{align*}
\min_{\kappa\geq1} \max_{D\succeq0} & \log\det(M-D)+\log\det(\kappa D-M)+\log\det D
\end{align*}
using projected updates of $D$ whenever necessary to ensure that the inner maximization problem has finite value. A detailed study of this proposal is left for future work.


==> major revision/intro.tex <==
\begin{comment}
Wenzhi to do:
\begin{enumerate}
    \item Fix Table 4, 7, 8, update csv files.
    \item Add base 10 in Figure 1 and 3. Change Figure 3 to be single distribution of improvement over baseline.
    \item Add comparison of iterative method runtimes with heuristic/optimal diagonal preconditioners.
    \item Try ash219 vs. factorization method. 
\end{enumerate}

Zhaonan To do:
\begin{enumerate}
    \item Reorganize intro to emphasize two goals of the paper: 1. scientific inquiry 2. potential improvement of iterative methods. Add goal of paper to improve quality of diagonal preconditioners.
\end{enumerate}
\end{comment}

\section{Introduction}
\label{sec:intro} 
Preconditioning, and \emph{diagonal} preconditioning in particular,
is a popular technique used in a wide range of disciplines and applications. %, sometimes under different names and in different forms. 
Although the term ``preconditioning'' was first used in \cite{turing1948rounding}, the concept of preconditioning to improve the convergence of iterative methods traces its origins all the way back to \cite{jacobi1845ueber}, who proposed the eponymous preconditioner, which is still one of the most popular preconditioning techniques in use today. Such preconditioners are often used to speed up the convergence and improve the accuracy of iterative solvers of large linear systems, such as
as the Jacobi method \citep{saad2003iterative}, the conjugate gradient
(CG) method \citep{hestenes1952methods,barrett1994templates,concus1985block}, which is often used in Newton steps of interior point algorithms
\citep{nocedal2006numerical}, and other stationary iteration methods \citep{young1954iterative,young2014iterative} or Krylov subspace methods \citep{liesen2013krylov}.

Many first order optimization
methods also involve some form of (diagonal) preconditioning or benefit
from preconditioning. These include the ADMM method \citep{lin2018admm,takapoui2016preconditioning,boyd2011distributed}
and steepest descent methods with preconditioned gradients, such as
mirror descent with quadratic distance functions \citep{beck2003mirror},
online Newton methods, and Quasi-Newton methods \citep{broyden1970convergence,goldfarb1970family,gao2019quasi}. Intuitively, preconditioning changes the local landscape of the objective function by making its level sets more ``rounded'' so that local minima are more accessible.  %Preconditioning is also essential when solving large linear systems, especially those arising from the discretization of PDEs, with stationary iteration methods \citep{young1954iterative,young2014iterative} or Krylov subspace methods \citep{liesen2013krylov}.%, such as the conjugate gradient descent \citep{hestenes1952methods,lanczos1952solution,concus1976generalized}.

\begin{comment}
Diagonal preconditioners in particular are widely used in adaptive
gradient methods such as AdaGrad \citep{duchi2011adaptive} and Adam
\citep{kingma2014adam}, because they can adapt to the geometry of
the problem and not only accelerate the rate of convergence, but also
achieve low regret for problems with certain geometries \citep{levy2019necessary}.
In machine learning, it is widely acknowledged that adaptive normalization
techniques such as batch normalization \citep{ioffe2015batch} and
layer normalization \citep{ba2016layer} are essential for achieving
good empirical performance in terms of convergence speed of training,
as well as better generalization power on test sets. Such methods
can be understood as a form of adaptive diagonal preconditioning on
the outputs of intermediate layers of a neural network.
\end{comment}

To understand the benefit of preconditioning more
precisely and to motivate the current paper, we start with the simple
setting of solving linear systems with iterative methods. Consider
the problem of solving 
\begin{equation}
\label{eq:linear-system}
Ax =b
\end{equation}
given a matrix $A\in\mathbb{R}^{m\times n}$ with full rank and $b\in\mathbb{R}^{n}$.
For large and sparse matrices $A$, iterative methods 
are very popular, in part due to parallelization. Under appropriate conditions, they often converge linearly with rates of convergence depending explicitly
on the condition number $\kappa(A)$ of $A$, defined as the ratio
of the extreme singular values of $A$:
\begin{align*}
\kappa(A) & :=\frac{\sigma_{\max}(A)}{\sigma_{\min}(A)}.
\end{align*}

\begin{comment}
\textbf{Jacobi Method} The Jacobi method for solving linear system
$Ax=b$ is the iteration 
\begin{align*}
x^{(k+1)} & =D^{-1}(b-Rx^{(k)})
\end{align*}
where $A=D+R$ and $D$ is the diagonal of $A$. When $A$ is diagonally
dominant, the method converges linearly with a rate of $\rho(D^{-1}R)=\rho(I-D^{-1}A)$,
which is bounded above by $\frac{\kappa(A)-1}{\kappa(A)+1}$\citep{arioli1985relations}.\\
\textbf{Gauss-Seidel Method}  Similar to the Jacobi method, the Gauss-Seidel Method uses the decomposition $A=L+U$ where $U$
is the strict upper triangular part of $A$. The iteration then updates
\begin{align*}
x^{(k+1)} & =L^{-1}(b-Ux^{(k)})
\end{align*}
where the inverse operation can done through forward substitution
due to the triangular structure of $L$. Like the Jacobi method,
two sufficient conditions for convergence are $A$ being symmetric positive
definite, or strictly diagonally dominant. In such cases, the linear
convergence rate is again given by $\frac{\kappa(A)-1}{\kappa(A)+1}$.
\\
\textbf{Kaczmarz Method} The Kaczmarz iteration for the linear
system $Ax=b$ consists of the updates 
\begin{align*}
x^{(k+1)} & =x^{(k)}+\frac{b_{i}-\langle a_{i},x^{(k)}\rangle}{\|a_{i}\|^{2}}a_{i}
\end{align*}
where $i=k\mod m$, the number of rows of $A$, and $a_{i}$
is the $i$th row of $A$. A randomized version that chooses the update
with $a_{i}$ at each step with probability proportional to $\|a_{i}\|^{2}$
has been shown to converge linearly in expectation with a rate of
$\frac{1}{1-\kappa(A)^{-2}}$ \citep{strohmer2009randomized}. Other
variants of the Kaczmarcz method such as the block Kaczmarz method
and sketch-and-project methods have been shown to have similar convergence
rates \citep{needell2019block}. \\
\textbf{Gradient Methods} First order optimization methods can also
be applied to solve the square linear system $Ax=b$, which is equivalent
to minimizing the quadratic objective $f(x)=\frac{1}{2}x^{T}Ax-x^{T}b$.
Steepest descent with optimal step sizes has linear convergence given
by
\begin{align*}
\|x^{(k)}-x^{\ast}\|_{A} & \leq(\frac{\kappa(A)-1}{\kappa(A)+1})^{2k}\|x^{(0)}-x^{\ast}\|_{A}
\end{align*}
where $\|v\|_{A}=v^{T}Av$ \citep{luenberger1984linear}. Similarly,
conjugate gradient (CG) has a linear convergence rate of $\frac{\sqrt{\kappa(A)}-1}{\sqrt{\kappa(A)}+1}$.\\
\textbf{Quasi-Newton Methods} Quasi-Newton methods such as BFGS and
Anderson mixing accelerate the gradient method by premultiplying $\nabla f(x)$
with an approximate inverse Hessian $B$. The exact dependence of
convergence rate on the condition number of $B$ is not well-studied,
but it has been known that when $B$ is ill-conditioned, the algorithm
suffers slowdown or divergence.
\end{comment}

\begin{table}
	\begin{centering}
	\begin{tabular}{|c|c|c|c|c|}
			\hline 
			& Jacobi & Gauss-Seidel & Steepest Descent & Conjugate Gradient\tabularnewline
			\hline 
			\hline 
			linear convergence rates &  $\frac{\kappa(A)-1}{\kappa(A)+1}$ &  $\frac{\kappa(A)-1}{\kappa(A)+1}$ &  $(\frac{\kappa(A)-1}{\kappa(A)+1})^{2}$ & $\frac{\sqrt{\kappa(A)}-1}{\sqrt{\kappa(A)}+1}$\tabularnewline
			\hline 
		\end{tabular}
		\par\end{centering}
	\caption{Rates of linear convergence of some iterative methods
		for solving the system $Ax=b$%, under respective conditions such as
		%diagonal dominance for Jacobi and Gauss-Seidel
		}
	\label{tab:rates}
\end{table}
 In Table \ref{tab:rates}, we summarize the linear convergence rates of some common iterative methods
used to solve large linear systems $Ax=b$, under their respective conditions necessary for convergence. We see that the rates are faster when the matrix $A$ has a smaller condition
number $\kappa(A)$. This phenomenon is more general.
For optimization problems, it is well known that the condition
number of the Hessian matrix of the objective plays a similar role
in the rates of convergence of first order methods. For example, for
general strongly convex objectives, gradient descent has the same
asymptotic linear convergence rate of $(\frac{\kappa(A)-1}{\kappa(A)+1})^{2}$
where $A$ is now the Hessian of the objective at optimal point $x^{\ast}$,
i.e. $A=\nabla^{2}f(x^{\ast})$. %Thus the larger the condition number
%of $A$, the slower the convergence. 
In order to accelerate the convergence
of iterative solvers and optimization methods, it is then essential
to ensure that the condition number of the coefficient or Hessian
matrix is small, i.e., the system is well-conditioned. Preconditioning achieves this by multiplying the
a matrix $A$ by simple matrices $D$ and $E$, such that the matrices $DA$,
$AE$, or $DAE$ have a smaller condition number than $A$. For example,
the preconditioned conjugate gradient method solves the equivalent
system
\begin{align*}
M^{-1}(Ax) & =M^{-1}b
\end{align*}
with $M$ given by the incomplete Cholesky factorization of $A$,
often resulting in $\kappa(M^{-1}A)\ll\kappa(A)$.

A large class of preconditioning methods uses matrices $D,E$ that
are \emph{diagonal}. In many applications, diagonal preconditioners are desirable, because applying them amounts to scaling the rows or columns of the matrix of interest, which does not incur much additional computational cost. In the context of solving linear systems, recovering the solution of the original system from the solution of the preconditioned system is also straightforward.

There exist many heuristics for finding
good diagonal preconditioners to achieve reductions in condition numbers.
We mention the following commonly used diagonal preconditioning procedures:
\begin{itemize}
	\item Jacobi preconditioner \citep{jacobi1845ueber}: for square matrices $A\rightarrow A(\text{diag}(A))^{-1}$ is the
	simplest diagonal preconditioner, and it works well when $A$ is diagonally
	dominant. 
	\item Matrix equilibration \citep{bradley2010algorithms, takapoui2016preconditioning}: find diagonal
	matrices $D,E$ such that columns of $DAE$ have equal $\ell_{p}$
	norms, and rows of $DAE$ have equal $\ell_{p}$ norms. A popular algorithm to achieve this is the Sinkhorn-Knopp algorithm
	\citep{sinkhorn1964relationship}. 
	\item Column (row) normalization: $A\rightarrow AD^{-1}$ where $D$ is
	the diagonal matrix of column standard deviations or column $\ell_{2}$
	norms. 
\end{itemize}
%The third method is also commonly used as a normalization procedure for data augmentation/processing. Compared to matrix equilibration, it is easier to compute. It also has an interesting connection with the method of batch normalization that is ubiquitous in machine learning.

Even though the preconditioning methods discussed above are popular in practice,
they are based on heuristics and do not always guarantee reductions in the
condition number of the matrix $A$. Moreover, in many cases, an optimal diagonal preconditioner can potentially achieve a much larger reduction in condition number compared to that achieved by heuristic methods, although a detailed study of how much improvement is possible has not been conducted. This is a practically relevant issue, because it informs practitioners on whether existing popular preconditioners are sufficient for their applications. Therefore, it remains an important problem to provide an efficient and practical algorithm that provides diagonal
preconditioners which are guaranteed to achieve optimal reductions in condition numbers.

%When we cannot effectively reduce the condition number of $A$ with existing diagonal preconditioners, it is important to have a practical algorithm that provides diagonals preconditioner which are guaranteed to reduce the condition number.

%Finally, in stochastic optimization settings,
%lack of access to the full matrix requires adaptive diagonal preconditioners
%that make use of data accessed so far. 
%In this paper, we attempt to
%address these problems. We first study the problem of when the column
%normalization method is effective at reducing the condition number
%of the data matrix. We provide a concentration result for the condition
%number of sub-Gaussian matrices and show that the reduction in condition
%number using column normalization is on the order of the ratio between
%the condition numbers of the population covariance matrix and the
%population correlation matrix, and then give sufficient conditions
%on when this ratio is large, i.e. diagonal preconditioning with column
%norm/standard deviation is effective. 
In this paper, we study the problem of
finding \emph{optimal} diagonal preconditioners for \emph{any} matrix $A$ with full rank. We are motivated by two objectives. First, we are interested in studying how much optimal diagonal preconditioners can improve over heuristic diagonal preconditioners for large systems, in terms of condition number reduction as well as speeding up iterative methods. Second, we want to develop fast and practical algorithms to find optimal diagonal preconditioners, so that when they are applied to large systems, the computational overhead to find optimal preconditioners can be potentially mitigated by overall accelerations as a result of their application. 

Our contributions are as follows. We reformulate the optimal diagonal preconditioning problem as a quasi-convex problem, and propose a bisection algorithm and  interior point algorithms with $O(\log\frac{1}{\epsilon})$
iteration complexities, that can find one-sided and two-sided diagonal preconditioners guaranteed to achieve
a condition number within $\epsilon$ of the optimal value. For one-sided preconditionings, we also provide alterantive formulations of the problem as dual SDPs, and apply customized solvers to solve large systems efficiently. We conduct extensive numerical experiments on datasets from \texttt{SuiteSparse}, \texttt{LIBSVM}, and \texttt{OPENML} to empirically evaluate the proposed procedures. Our algorithms can find near-optimal diagonal preconditioners efficiently for matrices of size up to 200,000 with the help of a row sampling scheme in the customized solver. Experiment results suggest that there is indeed a large gap between reductions in condition numbers achieved by existing popular diagonal preconditioning methods and those achieved by optimal diagonal preconditioners, suggesting to practitioners that algorithms that rely on preconditioning could be further improved. Our experiments also demonstrate that optimally-preconditioned iterative methods can outperform heuristically-preconditioned iterative methods as well as direct methods for solving linear systems.

%We also give results on the effect of reduction in condition number of the data matrix on the condition number of a class of strongly convex and smooth functions. Finally, we extend our optimal diagonal preconditioner to an adaptive setting, and compare it with batch normalization, a common adaptive preconditioning method used in machine learning, on regression and classification problems, and find that gradient methods with adaptive optimal diagonal preconditioning generally requires fewer iterations compared to batch normalization. The tradeoff is that the computation of the optimal diagonal conditioner requires using a full-rank matrix, and that its practical implementation based on the bisection algorithm may take a long time.

While constructing optimal (diagonal) preconditioners incurs extra computational cost, depending on the application, it may result in reduced overall computation time. For example, if we need to solve a sequence of linear systems with identical or almost identical coefficient matrices and different right hand sides, we can use the same preconditioners repeatedly, amortizing the overhead cost of constructing them. Some applications where this is the case include: 1. solving evolution problems with implicit methods; 2. solving mildly
nonlinear problems with Newton’s method \citep{benzi2002preconditioning}; 3. solving linear systems associated with multi-scale PDE problems. Moreover, although optimal preconditioners are harder to compute for large systems, the sub-problem to which a preconditioner can be applied may not always be very large. For example, if a block-coordinate algorithm is used in an optimization procedure, each step solves a small sub-problem that may benefit from preconditioning. Likewise, the increasingly popular paradigm of Federated Learning \citep{konevcny2016federated,kairouz2021advances} requires that data be stored locally on servers, and only local parameter updates are aggregated. In this setting, each server solves a unique problem of small to moderate size, and good local preconditioners can speed up the system considerably. As another motivating example, modern interior point algorithms for solving SDPs often rely on preconditioned conjugate gradient methods in each iteration, where the system matrix remains unchanged and is usually dense \citep{andersen2011interior}. Currently, simple heuristics are used to construct diagonal preconditioners, and better preconditioners would certainly help.
%\subsection{Brief Review of Existing Preconditioning Methods}

Before we turn to our main problem, we briefly discuss some existing  preconditioning methods as context for the current work.
%There has been a number of diagonal preconditioning techniques that are popular in practice.
Much of the existing preconditioning literature is driven by the motivation to accelerate iterative methods, most notably the conjugate gradient, for solving large linear systems. These include the incomplete factorization methods \citep{saad2003iterative} and sparse approximate inverse methods \citep{benzi1999comparative}. The resulting preconditioners, which are generally non-diagonal, can be shown to accelerate these iterative methods. However, it is not always the case that the \emph{condition numbers} of the matrices associated with the linear system \eqref{eq:linear-system} can be provably reduced. Popular heuristics-based preconditioners such as the Jacobi preconditioner generally require diagonal dominance conditions to guarantee reductions in condition number.
In contrast, in this paper, we focus on the \emph{optimal} diagonal  preconditioning of a matrix, independent of the particular application from which it arises. This general purpose perspective allows us to develop algorithms that are guaranteed to achieve (near) optimal diagonal preconditioning for any matrix $A$ with full rank. Optimal preconditioners of this type have not been studied as much in the literature. For symmetric positive definite matrices, optimal polynomial preconditioners have been considered by \cite{cesari1937sulla,dubois1979approximating,johnson1983polynomial}. In contrast, the current work studies preconditioning for matrices of arbitrary shape, provided they have full ranks. 
The work of \cite{kaszkurewicz1995control} establishes an interesting control-theoretic interpretation of the optimal diagonal preconditioning problem for square invertible matrices, and provides a mostly theoretical algorithm by solving the associated constrained LQR problem.
The most closely related contemporary work to ours is that of \cite{jambulapati2020fast}, which considers one-sided optimal diagonal preconditioning and designs algorithms based on structured
mixed packing and covering SDPs. While \cite{jambulapati2020fast} provides theoretical guarantees on the runtime of their algorithm, it is unclear if their algorithm is practical. In contrast, we consider two-sided optimal diagonal preconditionings in addition to one-sided preconditionings, and also provide alternative SDP-based algorithms that our numerical experiments demonstrate to be effective in practice on medium to large size problems.  %Their approach was demonstrated to work well for a matrix of size 9, but at great computation costs. 

Finally, we mention a few additional preconditioning methods that can serve as potential baselines with which one may compare optimal diagonal preconditioners. The first is a popular Frobenius norm minimization method \citep{benson1982iterative} to find sparse preconditioners:
\begin{align*}
    \min_{M\in \mathcal{S}}\|I-AM\|_F,
\end{align*}
where $\mathcal{S}$ is a space of sparse matrices, which we may restrict to be positive diagonal matrices, and compare the resulting diagonal preconditioners to the optimal ones, in terms of condition number reduction as well as computation cost. Another class of popular two-sided preconditioners is based on the principle of \emph{matrix equilibration} \citep{ruiz2001scaling,takapoui2016preconditioning,sinkhorn1964relationship}, among which the Ruiz scaling algorithm \citep{ruiz2001scaling} is known to perform well in practice. In our numerical experiments in Section \ref{sec:experiments}, we consider some of these baseline preconditioners when assessing the performance of our optimal preconditioners.

\begin{comment}
\textbf{In the rest of this introduction, we discuss several examples
in optimization and machine learning where some form of diagonal preconditioning
is used. }
\begin{example}
Principal component analysis (PCA) is a simple tool used for dimension
reduction and exploratory analysis of data. In PCA, one forms the
empirical covariance matrix $\hat{\Sigma}$ from design matrix $X$,
and perform an eigenvalue decomposition of $\hat{\Sigma}=V\Lambda V^{T}$
and retain only the top few eigenvalues to obtain a low-rank approximation
to $\hat{\Sigma}$ that nevertheless captures most of the variations
in the data. The top eigenvectors are interpreted as the directions
in the dataset with the most variations. In general, if some variables
in the dataset are rescaled due to a change of units, the resulting
PCA analysis will yield different results. It is known that carrying
out the analysis on the correlation matrix $\hat{R}=\hat{D}^{-\frac{1}{2}}\hat{\Sigma}\hat{D}^{-\frac{1}{2}}$,
where $\hat{D}$ is the diagonal of $\hat{\Sigma}$, is sometimes
more informative than on the covariance itself, especially when variables
are of different scales that are not substantially important, e.g.
differences in measurement units. The normalization of $\hat{\Sigma}$
into a correlation matrix can be seen as a preconditioning step on
the design matrix $X$. 
\end{example}
%
\begin{example}
In optimization, preconditioning is often used to accelerate first
order optimzation algorithms. For example, in gradient descent instead
of taking a step in the direction of $-\nabla f(x_{n})$, one may
instead use the update $-M\nabla f(x_{n})$ where $M$ is the preconditioner.
For quadratic problems such as 
\begin{align*}
\min_{x} & \|Ax-y\|^{2}
\end{align*}
the $M$ is chosen so that the Hessian of the objective has a reduced
condition number, i.e. $\kappa(M^{T}A^{T}AM)\ll\kappa(A^{T}A)$. In
general, preconditioning in first order methods can be seen as an
attempt to improve the shape of level sets so they look close to circles. 
\end{example}
%
\begin{example}
In deep learning models with neural nets, batch normalization \cite{ioffe2015batch}
has become an increasingly standard method to ensure faster convergence
of stochastic gradient descent. Let $x^{(m,k)}\in\mathbb{R}^{n\times p_{m}}$
denote the output of the $m$-th layer, consisting of $n$ $p_{m}$-dimensional
vectors, at the $k$th iteration of stochastic gradient descent. Batch
normalization involves applying a centering operation and a scaling
operation to $x^{(m,k)}$, followed by reverse operations with parameters
$\gamma\in\mathbb{R}_{++}^{p_{m}},\beta\in\mathbb{R}^{p_{m}}$, to
obtain 
\begin{align*}
\tilde{x}_{i}^{(m,k)} & =\frac{(x_{i}^{(m,k)}-\mu_{i})}{\sigma_{i}}\cdot\gamma_{i}+\beta_{i}
\end{align*}
 for the $i$th column of $x^{(m,k)}$, where $\mu_{i}$ is the mean
of the $i$th column, and $\sigma_{i}$ is the standard deviation.
The parameters $\gamma,\beta$ are updated through SGD together with
the original parameters of the neural network. This procedure can
be seen as a variable preconditioning, where each SGD update uses
a different diagonal preconditioner $\gamma$. 
\end{example}
%
\begin{example}
It has been observed that neural network based classification models
have improved test accuracy when data normalization is used. This
suggests that preconditioning not only has a positive effect on the
optimization performance of algorithms, but also improves the generalization
power of the trained models, likely due to the fact that the converged
point is a better local optima. 
\end{example}
%
We see that many procedures used in optimization and machine learning
are in essence some form of preconditioning, and condition number
is the central quantity of interest in the analysis of convergence
of algorithms. In the next section, we briefly recall some basic facts
about the condition number and its importance in optimization, and
then review some commonly used preconditioning methods. 

\paragraph*{Quasi-Newton Methods \textmd{Quasi-Newton methods such as BFGS and
Anderson mixing accelerate the gradient method by premultiplying $\nabla f(x)$
with an approximate inverse Hessian $B$. The exact dependence of
convergence rate on the condition number of $B$ is not well-studied,
but it has been known that when $B$ is ill-conditioned, the algorithm
suffers slowdown or divergence. }}

To do: Krylov subspace methods.
\end{comment}

==> major revision/optimization.tex <==
\section{Diagonal Preconditioning and Stochastic Convex Optimization}
\label{sec:optimization}

So far we have focused on diagonal preconditioning of design matrices.
We studied how preconditioning affects the condition number of the
design matrices, and also developed algorithms to compute optimal
diagonal preconditioners. These results have direct implications on
the convergence rates of iterative solvers of linear systems and first
order methods applied to quadratic objectives, since convergence rates
depend explicitly on the condition number of the (constant) Hessian
matrix $X^{T}X$. 

For general convex objective functions, convergence rates of first
order methods depend on the smoothness and convexity constants of
the function. It is therefore more challenging to study the impact
of preconditioning on the design matrix on the convergence of first
order methods on general convex objective functions, as we need to
investigate how the reduction in condition number of the design matrix
translates to improvements in the smoothness and convexity constants
of the objective function. In this section, we first give such a result
for a class of objective functions $f$ that correspond to the (regularized)
loss of an empirical risk minimization problem (\cite{shalev2013stochastic}),
and show that when $f$ is smooth and strongly convex, reductions
in the condition number of the objective is on the order of $\frac{\kappa(X)}{\kappa(X_{0})}$
where $X$ is the design matrix and $X_{0}$ is any preconditioned
design matrix with smaller condition number. For other more general
classes of convex objectives, we leave to future work to quantify
theoretically the impact of condition number on convergence rates.
However, we make the case that the optimal diagonal preconditioning
algorithms developed in the previous section is not limited to being
applied to fixed design matrices. We establish the connection of batch
normalization, a popular technique in machine learning, to adaptive
preconditioning, and develop an adaptive version of the optimal diagonal
preconditioning algorithm. We then conduct numerical experiments that
demonstrate the effectiveness of the optimal diagonal preconditioning
algorithm at speeding up first order methods in regression and classification
problems in the next section. 

\subsection{Convergence Rates for General Convex Problems}

The relationship between the complexity of first order methods and
the smoothness and convexity properties of the objective function
has been well established in the optimization literature. Here the
complexity is usually expressed in terms of the number of iterations
required to obtain an $\epsilon$-optimal solution. We summarize the
corresponding iteration complexities of solving 
\begin{align*}
\min_{\theta}f(\theta,X)
\end{align*}
in Table \ref{tab:Optimal-iteration-complexity}, taken from \cite{zhang2013linear}. 

\begin{table}
	\begin{centering}
		\begin{tabular}{|c|c|c|c|}
			\hline 
			& Lipschitz continuous & Smooth & Smooth\&Strongly Convex\tabularnewline
			\hline 
			\hline 
			Full Gradient & $O(\frac{1}{\epsilon^{2}})$ & $O(\frac{L}{\sqrt{\epsilon}})$ & $O(\sqrt{\kappa}\log\frac{1}{\epsilon})$\tabularnewline
			\hline 
			Stochastic Gradient & $O(\frac{1}{\epsilon^{2}})$ & $O(\frac{1}{\epsilon^{2}})$ & $O(\frac{1}{\lambda\epsilon})$\tabularnewline
			\hline 
		\end{tabular}
		\par\end{centering}
	\caption{\label{tab:Optimal-iteration-complexity}Optimal iteration complexity
		of convex optimization. $L$ and $\lambda$ are the moduli of smoothness
		and convexity, i.e. $\lambda\protect\leq\|\nabla_{\theta}^{2}f\|\protect\leq L$,
		and $\kappa=L/\lambda$ is the condition number. }
	
\end{table}

The iteration complexity in stochastic optimization is generally polynomial
in $\frac{1}{\epsilon}$. However, when $f$ is of the form 
\begin{align*}
f & =\frac{1}{n}\sum_{i=1}^{n}f_{i}+g_{\lambda}
\end{align*}
where $f_{i}$ are convex and $L$-smooth, while $g_{\lambda}$ is
$L$-smooth and $\lambda$-strongly convex, the complexity can be
improved to be logarithmic in $\frac{1}{\epsilon}$. For example,
the stochastic average gradient (SAG) method has iteration complexity
$O(n\log\frac{1}{\epsilon})$ provided $n\geq8\kappa$, the stochastic
dual coordinate ascent (SDCA) method (\cite{shalev2013stochastic})
has iteration complexity $O((n+\kappa)\log\frac{1}{\epsilon})$, and
the epoch mixed gradient descent (EMGD) method (\cite{zhang2013linear})
has the complexity $O((n+\kappa^{2})\log\frac{1}{\epsilon})$. Of
the three, EMGD can be applied to general strongly convex and smooth
functions, in which case it requires $O(\log\frac{1}{\epsilon})$
full gradient queries and $O(\kappa^{2}\log\frac{1}{\epsilon})$ stochastic
gradient queries. Table \ref{tab:complexity_stochastic} compares
these stochastic gradient algorithms with the accelerated gradient
descent of Nesterov applied to stochastic gradient descent. 

\begin{table}
	\begin{centering}
		\begin{tabular}{|c|c|c|c|}
			\hline 
			Nesterov & EMGD & SAG $(n\geq8\kappa)$ & SDCA\tabularnewline
			\hline 
			\hline 
			$O(\sqrt{\kappa}n\log\frac{1}{\epsilon})$ & $O((n+\kappa^{2})\log\frac{1}{\epsilon})$ & $O(n\log\frac{1}{\epsilon})$ & $O((n+\kappa)\log\frac{1}{\epsilon})$\tabularnewline
			\hline 
		\end{tabular}
		\par\end{centering}
	\caption{\label{tab:complexity_stochastic}Computational complexity of stochastic
		first order methods for minimizing $f=\frac{1}{n}\sum_{i=1}^{n}f_{i}+g_{\lambda}$. }
\end{table}

We note the distinction between the condition number of a function
and a matrix. For a function $f(\theta,X)$, where $X$ denotes data
and $\theta$ denotes parameter, the condition number is given by
$L/\lambda$ where 
\begin{align*}
\lambda\leq\|\nabla_{\theta}^{2}f(\theta,X)\| & \leq L
\end{align*}
for all $\theta\in\Theta$ the parameter space. When $f(\theta,X,Y)=\frac{1}{n}\|X\theta-Y\|_{2}^{2}$,
the Hessian is a fixed quantity, namely the Wishart matrix $X^{T}X$.
In general, the Hessian is parameterized by $\theta$ and $\lambda$
and $L$ are the upper and lower bounds of the largest and smallest
eigenvalues of the Hesisan, respectively. 

In this section, we are interested in how diagonal preconditioning
procedures on the design matrix affect the iteration complexity through
reducing the condition number of the objective function. 

\begin{comment}
In this section, we focus on how preconditioning procedures speed
up the convergence of first order methods in optimization. Note however
that preconditioning is important for second order methods as well,
but we defer the analysis to future work. By the data matrix, we mean
the input $x$ required to evaluate the full or stochastic gradients
of $f(x;w)$, where $w$ is the variable we are trying to minimize
$f$ over. 
\end{comment}


\subsection{Accelerating Optimization through Preconditioning}

To motivate the discussion, we first examine the least squares problem
\begin{align*}
\min_{\theta}\frac{1}{n}\|X\theta-Y\|_{2}^{2}
\end{align*}
where $X\in\mathbb{R}^{n\times p}$ which has smoothness and strong
convexity moduli of $\lambda_{1}(X^{T}X)$ and $\lambda_{n}(X^{T}X)$,
respectively. Here we assume that $n>p$, so that $X^{T}X$ is invertible
and hence the objective function is both smooth and strongly convex.
For the least squares problem, an analytic solution is available,
but we consider first order methods mainly because the quadratic form
makes the effect of preconditioning procedures obvious. We may also
imagine a setting where potentially $n,p$ are large so that direct
computation of $(X^{T}X)^{-1}$ is costly, so that we can only resort
to (stochastic) first order methods. In any case, given the least
squares problem, we are interested in how diagonal preconditioning
procedures speed up the convergence of first order methods. 

There are potentially two levels of stochasticity. The data matrix
is assumed to have i.i.d. rows from some distribution. Our earlier
results show that the condition number $\kappa(X^{T}X)$ of sub-Gaussian
data matrices concentrate around that of the population covariance
matrix $\Sigma$, and that for a class of population covariance matrices,
preconditioning with column standard deviation reduces the condition
number of the data matrix by a factor on the order of $\sqrt{\kappa(\text{diag}(\Sigma))}$
with high probability. So for full gradient methods, a reduction in
computational complexity is achieved through the reduction of the
condition number on the order of $\sqrt{\kappa(\text{diag}(\Sigma))}$
with high probability if we assume sub-Gaussian data distribution
with well-behaved covariance matrix $\Sigma$, or $\sqrt{\frac{\kappa(X^{T}X)}{\kappa(D^{-1}X^{T}XD^{-1})}}$
using optimal diagonal preconditioning methods developed in the previous
section, for the least squares problem. 

For general smooth and strongly convex objectives $f(\theta,X)$ the
condition number $\kappa(\nabla_{\theta}^{2}f(\theta,X))$ of the
Hessian of the objective function is not constant, but depends on
the current estimate $\theta^{k}$ of the parameter.\textbf{ }Here
there are two types of preconditioning that can be performed. The
first type is that done on the data matrix $X$, using a variety of
conditioning algorithms including the usual data normalization procedure,
batch normalization, or the optimal diagonal preconditioning algorithm
developed in this paper. It can be done on the entire $X$ once before
the optimization procedure, or for stochastic systems, on the sub
design matrix formed by the minibatch of samples. If we are using
first order methods, only the above preconditioning on the (sub)design
matrix is possible. If we can efficiently calculate or approximate
the inverse Hessian, then a second preconditioning option is to precondition
directly on the (approximate) Hessian or inverse Hessian, evaluated
at the current estimate $\theta^{k}$. As discussed earlier, Quasi-Newton
methods and other accelerated gradient methods such as Anderson mixing
(\cite{zhang2018globally}) and Adagrad (\cite{duchi2011adaptive}) rely
crucially on some form of approximate inverse Hessian or Jacobian.
When the approximate inverse Hessian is ill-conditioned, the methods
are known to slow down or diverge both in theory and in practice (\cite{shanno1970optimal}).
Preconditioning the approximate inverse Hessian has been considered
in as early as (\cite{shanno1970conditioning}). Here we simply note
that our optimal diagonal algorithm can also be applied to the quasi-Newton
update formulae to improve the condition number of the approximate
inverse Hessian. 

We focus on the case of preconditioning on the data/design matrix
$X$, and study how the reduction in $\kappa(X^{T}X)$ translates
into that of $\kappa_{f}$, where 
\begin{align*}
\kappa_{f} & =\frac{L_{f}}{\lambda_{f}}\\
L_{f} & =\sup_{\theta}\|\nabla_{\theta}^{2}f(X,\theta)\|\\
\lambda_{f} & =\inf_{\theta}\|\nabla_{\theta}^{2}f(X,\theta)\|
\end{align*}

In order to analyze how preconditioning of the data\textbf{ }matrix
affects the condition number of the Hessian at $\theta^{k}$, we need
to make assumptions about the structure of the objective function
$f$. For example, if $f$ is of the form $f_{0}(X\theta)$ for some
$f_{0}$ with condition number $\kappa_{0}$, then the Hessian of
the objective function satisfies 
\begin{align*}
\kappa(\nabla_{\theta}^{2}f) & =\kappa(X^{T}\cdot\nabla^{2}f_{0}(X\theta)\cdot X)
\end{align*}
and we should expect improvements on the condition number of $X^{T}X$
to improve the condition number of the Hessian as well. In the following
result, we focus on the case when $f$ corresponds to the (regularized)
loss of an empirical risk minimization problem (\cite{shalev2013stochastic}).
In this case, the reduction in $\kappa_{f}$ is on the order of $\sqrt{\kappa(X^{T}X)/\kappa(DX^{T}XD)}$
for smooth and strongly convex objectives. This reduction then implies
the corresponding improvements in iteration complexities of first
order methods, thorugh their dependences on $\kappa_{f}$. 

\begin{theorem}
\label{thm:cond_number_general}If $f(X,w)=\frac{1}{n}\sum_{i}f_{i}(w^{T}x_{i})$
for scalar $\lambda$-strongly convex and $L$-smooth functions $f_{i}$.
Then replacing $x_{i}$ with $Dx_{i}$, where $D$ is a diagonal matrix
such that $\kappa(DX^{T}XD)\leq\kappa(X^{T}X)$, we have

(i) For general $f_{i}(z)$,

\begin{align*}
\kappa(\nabla_{w}^{2}f(XD,w)) & \leq\frac{\kappa(\nabla_{w}^{2}f(X,w))}{\kappa(X^{T}X)/\kappa(DX^{T}XD)}\kappa_{0}^{2}
\end{align*}
where $\kappa_{0}=\frac{L}{\lambda}$, i.e. when $f_{i}$ are well-conditioned
so $\kappa_{0}$ is small, the reduction in condition number of the
objective function with preconditioning is on the order of $\kappa(X^{T}X)/\kappa(DX^{T}XD)$.

(ii) When $f_{i}(z)=z^{2}$, the result reduces to the special case
of linear regression, where the reduction in condition number is lower
bounded by exactly $\kappa(X^{T}X)/\kappa(DX^{T}XD)$.
\end{theorem}
\proof{Proof}
	We have 
	\begin{align*}
	\nabla_{w}^{2}f(X,w) & =\frac{1}{n}\sum_{i}\nabla^{2}f_{i}(w^{T}x_{i})x_{i}x_{i}^{T}
	\end{align*}
	Moreover,
	\begin{align*}
	\frac{1}{n}LX^{T}X\succeq\frac{1}{n}\sum_{i}\nabla^{2}f_{i}(w^{T}x_{i})x_{i}x_{i}^{T} & \succeq\frac{1}{n}\lambda X^{T}X
	\end{align*}
	so that 
	\begin{align*}
	\kappa(\nabla_{w}^{2}f(XD,w)) & \leq\kappa(DX^{T}XD)\cdot\kappa_{0}\\
	& =\frac{\kappa(DX^{T}XD)}{\kappa(X^{T}X)}\cdot\kappa(X^{T}X)\cdot\kappa_{0}\\
	& \leq\kappa_{0}^{2}\cdot\kappa(\nabla_{w}^{2}f(X,w))\cdot\frac{\kappa(DX^{T}XD)}{\kappa(X^{T}X)}
	\end{align*}
	\hfill \halmos
\endproof
The above result separates out the effect of the design matrix on
the condition number of the objective function. If the objective function
itself is smooth and strongly convex, then diagonal preconditioning
on a badly-conditioned design matrix results in a reduction of the
condition number of the objective function on the order of $\sqrt{\kappa(X^{T}X)/\kappa(DX^{T}XD)}$,
which then implies improvements on the complexities of first order
methods through their dependences on the condition number. 

\subsection{Adaptive Diagonal Preconditioning}

So far, we have focused on preconditioning with a fixed preconditioner
$D$ when we have acces to all the data at once in the form of the
design matrix, where $D$ is obtained from data matrix $X$, e.g.
column-wise standard deviation of $X$ or optimal diagonal preconditioning
obtained using methods discussed in the previous section. However,
in practice such a preconditioner may not be available. For example,
in stochastic gradient descent or online learning, we may not have
prior access to the full data matrix $X$, instead only drawing random
subsets of all samples. In such settings, it is still possible to
speed up the convergence with adaptive preconditioning procedures
applied to first order methods. In fact, many first order methods
can be understood to involve some form of adaptive preconditioning.
For example, BFGS method (\cite{broyden1970convergence,goldfarb1970family})
and AdaGrad (\cite{duchi2011adaptive}) pre-multiply the gradient with
some approximate (diagonal) inverse Hessian. Other adaptive gradient
methods that perform local optimization with an adaptive metric constructed
from observed iterates have become increasingly popular in deep learning
with benefits to the convergence speed as well as statistical properties
of the iterative optimization procedures. For example, \cite{levy2019necessary} show that when the ``scale'' of the gradients
varies across dimensions, adaptive gradient methods such as AdaGrad
(\cite{duchi2011adaptive}) achieves lower regret compared to vanilla
stochastic gradient methods. 

A popular normalization technique used in deep learning, called batch
normalization (\cite{ioffe2015batch}), can also be understood as a
form of adaptive (diagonal) conditioning. 

For general neural networks, let $x^{(m,k)}\in\mathbb{R}^{n\times p_{m}}$
denote the output of the $m$-th layer, consisting of $n$ $p_{m}$-dimensional
vectors, at the $k$th iteration of stochastic gradient descent. Batch
normalization involves applying a centering operation and a scaling
operation to $x^{(m,k)}$, followed by reverse operations with parameters
$\gamma\in\mathbb{R}_{++}^{p_{m}},\beta\in\mathbb{R}^{p_{m}}$, to
obtain 
\begin{align*}
\tilde{x}_{i}^{(m,k)} & =\frac{(x_{i}^{(m,k)}-\mu_{i})}{\sigma_{i}}\cdot\gamma_{i}+\beta_{i}
\end{align*}
for the $i$th column of $x^{(m,k)}$, where $\mu_{i}$ is the mean
of the $i$th column, and $\sigma_{i}$ is the standard deviation.
The parameters $\gamma,\beta$ are updated through SGD together with
the original parameters of the neural network. The point is that population
statistics for intermediate layers are not known a priori, so $\gamma$
and $\beta$ serve as adaptive parameters that are updated at each
step of the training. 

Specialized to the least squares problem, it effectively solves the
problem $\min_{\theta,D}\frac{1}{n}\|XD\theta-y\|_{2}^{2}$ by alternating
between $\theta$ and $D$ during each iteration, i.e. at the $k$th
iteration, given $D^{(k)}$, one solves the problem $\min_{\theta}\frac{1}{n}\|XD^{(k)}\theta-y\|_{2}^{2}$
and then find $D_{1}^{(k+1)}$ by solving $\min_{D}\frac{1}{n}\|XD\theta^{(k+1)}-y\|_{2}^{2}$.

This alternating optimization procedure is present in many other convex
optimization problems with special structures, for example the ADMM
method for minimizing the sum of convex functions with block variables
(\cite{lin2015global,wen2010alternating}). It is also used in non-convex
formulations of convex problems, most notably low-rank matrix and
tensor factorization \cite{chi2019nonconvex,aswani2016low,zhao2015nonconvex},
where alternating minimization of the objective is employed to solve
a non-convex formulation of the problem. Besides convergence issues,
another recent focus of the latter literature is on the ``implicit
regularization'' (\cite{wu2019implicit}) of the alternating minimization
algorithm associated with the non-convex formulation. 

It is similarly possible to extend our optimal diagonal preconditioning
procedure to the stochastic setting. Suppose each iteration we observe
subsets of rows of a design matrix $X$. At each iteration we update
our estimate of $X^{T}X$ based on samples drawn from $X$ so far.
Then we can compute the optimal diagonal preconditioner $D$ based
on the current estimate of $X^{T}X$. As the number of iterations
increases, our estimate of $X^{T}X$ becomes more accurate, and $D$
should approach the appropriate optimal diagonal preconditioner given
$X^{T}X$. This gives the following algorithm. 

\begin{comment}
More generally, at each iteration, $D$ can be calculated based on
other heuristics depending on $X$ and current parameter estimates.
The popular batch normalization procedure can be understood as an
instance of this adaptive preconditioning. Other adaptive gradient
methods that perform local optimization with an adaptive metric constructed
from observed iterates have become increasingly popular in deep learning.
\cite{levy2019necessary} show that when the ``scale''
of the gradients varies across dimensions, adaptive gradient methods
such as AdaGrad \cite{duchi2011adaptive} achieves lower regret compared
to vanilla stochastic gradient methods. 
\end{comment}

\begin{algorithm}
	(Adaptive optimal diagonal preconditioning) Let $\overline{X}^{(0)}=[]$
	and at the $k$th iteration, form the cumulative design matrix $\overline{X}^{(k)}$
	by concatenating the $k$-th batch $X^{(k)}$ with $\overline{X}^{(k-1)}$
	and retaining unique rows. If $\overline{X}^{(k)}$ is full rank,
	then find $D_{1}^{(k)}$ that minimizes $\kappa(D(\overline{X}^{(k)T}\overline{X}^{(k)}D)$
	and perform the preconditioning$X^{(k)}D_{1}^{(k)}$. Alternatively,
	we can perform the optimal diagonal scaling every $m$ iterations,
	where $m$ is chosen to balance the tradeoff between computational
	cost and convergence speed. 
\end{algorithm}

A natural next step is to compare the performance of the optimal diagonal
preconditioning with that of batch normalization on regression and
classification problems. We take up this in the next section. We also
note that although batch normalization speeds up the convergence of
first order methods and can be viewed as a form of adaptive diagonal
preconditioning, it is not the case that the effective condition numbers
of Hessian matrices under batch normalization are reduced, since the
diagonal conditioner is selected so as to minimze the objective loss
rather than the condition number of the preconditioned matrix. This
is in contrast to our adaptive optimal preconditioning algorithm,
which speeds up convergence by reducing the effective condition number
of the design matrix. Thus it remains to further investigate the mechanism
through which batch normalization speeds up the convergence of first
order methods. 

We also mention that other adaptive methods, such adaptive regularization
of objective (\cite{jiang2017unified}) and adaptive step size \cite{gao2019quasi},
are also effective in speeding up the convergence of first order methods.
These methods are often applied to quasi-Newton methods and the step
size is determined based on information on the local curvature of
the objective function, e.g. the damped Newton method \cite{nesterov2013introductory}
of Nesterov, who derived convergence results for self-concordant functions
\cite{nesterov1994interior}. As a possible extension of the optimal
preconditioning framework, it may be interesting to consider using
an approximate optimal preconditioner of the approximate inverse Hessian,
and to explore potential connections with adaptive step size approaches
for self-concordant functions. 

==> major revision/theory-old-2.tex <==
\section{Problem Setup and Algorithms}
\label{sec:optimal}

In this section, we turn to the two-sided optimal diagonal preconditioning
problem. For a matrix $A\in\mathbb{R}^{m\times n}$ with full rank, we want to find positive \emph{diagonal} matrices $D_1,D_2$ that solve the following minimization problem (the particular choice of exponents for $D_1,D_2$ will become clear shortly):
\begin{align}
\label{eq:two-sided-problem}
\min_{D_{1},D_{2}\succ0}\kappa(D_{1}^{1/2}AD_{2}^{-1/2})
\end{align}
There are two related \emph{one-sided} optimal diagonal preconditioning problems that seek diagonal matrices $D_1$ and $D_2$ which solve the following two distinct problems, respectively:
\begin{align}
\label{eq:left-sided-problem}
\min_{D_{1}\succ0}&\kappa(D_{1}^{1/2}A)\\
\label{eq:right-sided-problem}
\min_{D_{2}\succ0}&\kappa(AD_{2}^{-1/2})
\end{align}
 Note first that without loss of generality, we can always assume $m\geq n$, so that $A$ is a \emph{tall} matrix, since otherwise we may take the transpose of $A$ without changing the optimal solution pairs to the two-sided problem \eqref{eq:two-sided-problem}. For the one-sided problems \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem}, taking the transpose of $A$ essentially transforms one problem to the other. Moreover, for square matrices,
i.e., $m=n$, the three optimal preconditioning procedures essentially
yield the same optimal diagonal preconditioners, since similar square matrices
have the same eigenvalues hence the same condition numbers. Finally, note that solutions are scale-invariant, since for any optimal
pair $(D_{1},D_{2})$ of diagonal preconditioners that achieves the
minimum objective value of \eqref{eq:two-sided-problem}, $(c_1D_{1},c_2D_{2})$ for any $c_1,c_2>0$ is also
a pair of optimal diagonal preconditioners, and similarly for \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem}. For the purpose of reducing condition numbers, any optimal solution is sufficient.

%For now, we will primarily focus on developing algorithms for the two-sided problem \eqref{eq:two-sided-problem}. 
\textbf{Overview.} We will develop a baseline algorithm based on bisection that solves the two-sided problem \eqref{eq:two-sided-problem} in this section, and then develop a polynomial time interior point algorithm in Section \ref{sec:potential-reduction}. %The corresponding algorithms and theory for the one-sided problems \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem} can be obtained with straightforward reductions. 
In Section \ref{sec:DSDP}, we show that \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem} admit reformulations as standard dual SDP problems,
to which customized solvers can be applied to obtain solutions efficiently for large matrices. We will then develop specialized algorithms for the one-sided problems based on this reformulation.
%In contrast, the two-sided problem \eqref{eq:two-sided-problem} does not admit an SDP reformulation. 
In Section \ref{sec:experiments}, we will compare the empirical performance
of these optimal preconditioning procedures. In general, one-sided optimal diagonal preconditioners are sufficient to achieve significant reductions in condition numbers, although there are instances where two-sided preconditioners are essential. In practice, we can handle large one-sided problems ($m \approx 5000$) thanks to the customized solver. %In particular, we will investigate
%when and how two-sided optimal preconditioning improves upon the
%two one-sided preconditioners significantly in
%terms of condition number reduction, as well as when the two one-sided
%methods differ from each other.

\subsection{Problem Reformulation}
 We start by rewriting the two-sided optimal diagonal preconditioning problem \eqref{eq:two-sided-problem} in a more accessible form. First, note that for any matrix $A \in \mathbb{R}^{m\times n}$ with full rank and $m\geq n$, $\kappa(A)=\sqrt{\kappa(A^{T}A)}$, so we can instead minimize the condition
number of $(D_{1}^{1/2}AD_{2}^{-1/2})^{T}(D_{1}^{1/2}AD_{2}^{-1/2})=D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2}$.
As the condition number is scale-invariant, we can introduce a new
positive \emph{variable} $\kappa$ (to be distinguished from the condition
number $\kappa(M)$ of a matrix) and rewrite the resulting problem
as
\begin{align*}
\min_{\kappa,D_{1},D_{2}\succ0}\kappa\\
I_n\preceq D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2}\preceq\kappa I_n
\end{align*}
The objective above achieves its minimum value $\kappa^\ast=(\min_{D_{1},D_{2}\succ0}\kappa(D_{1}^{1/2}AD_{2}^{-1/2}))^{2}$, and at any optimal solution $(D_1,D_2)$, $\lambda_{\min}(D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2})=1$ and $\lambda_{\max}(D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2})=\kappa^\ast$.

Next, the constraint $I_n\preceq D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2}\preceq\kappa I_n$
is equivalent to $D_{2}\preceq A^{T}D_{1}A\preceq\kappa D_{2}$, and, with diagonal matrices $D_1,D_2$, we can rewrite the problem in its final reformulation as
\begin{align}
\label{eq:SDP-two-sided}
\begin{split}
    \min_{\kappa\geq0} \kappa \\
A^{T}D_{1}A\succeq D_{2}\\
\kappa D_{2}\succeq A^{T}D_{1}A \\
D_1 \succeq I_m 
\end{split}
\end{align}
where we have replaced the strict inequalities $D_1,D_2\succ0$ by equivalently requiring $\kappa \geq 0$ and $D_1 \succeq I_m$. Since $A^TD_1A\succeq A^TA\succ 0$, $D_2$ and $\kappa$ in fact need to be both strictly positive. Note that the alternative constraint $D_2 \succeq I_n$ instead of $D_1 \succeq I_m$ does not work, however, since $m\geq n$ and $D_1$ could still have zero diagonal entries even if $D_2 \succ 0$.
The problem \eqref{eq:SDP-two-sided} is also scale-invariant, and we may further impose normalization constraints to make the solution unique. This is not necessary for the purpose of the baseline algorithm we develop in this section. For the interior point algorithm we develop in Section \ref{sec:potential-reduction}, we will impose an upper bound on $D_1$ to facilitate the definition of a potential function which we will aim to reduce. 
%However, as we will see, the interior point algorithm we develop based on potential reduction will find the unique solution with $\lambda_{\min}(D_1)=1$, so we do not need to explicitly impose the normalization constraint. 

Note that the problem in \eqref{eq:SDP-two-sided} is a quasi-convex problem. To see this more clearly, let $d_1\in\mathbb{R}^m,d_2\in\mathbb{R}^n$ be the vector representations of the diagonal matrices $D_1,D_2$, and moreover $d_3=\kappa d_2$. With $d_{1i}$ denoting the $i$-th element of $d_1$, and $d_{2j}$ the $j$-th element of $d_2$, the problem can be written as
\begin{align*}
\min_{\kappa,d_1,d_2,d_3\geq0} \sum_{j=1}^n d_{3j}/d_{2j}\\
\sum_{i=1}^{m} d_{1i} a_i a_i^T - \sum_{j=1}^n d_{2j} e_j e_j^T   \succeq 0\\
\sum_{j=1}^n d_{3j} e_j e_j^T -\sum_{i=1}^{m} d_{1i} a_i a_i^T\succeq 0\\
d_1 - \mathbf{1}_m \geq 0
\end{align*}
where vector $a_i$ is the $i$-th row of $A$ and $e_j \in \mathbb{R}^n$ is the vector whose $j$-th entry is 1 and zero otherwise. However, \eqref{eq:SDP-two-sided} is not equivalent to a standard SDP, because of the product term $\kappa D_2$.

\subsection{A Bisection Algorithm for Optimal Diagonal Preconditioning}
We start with a simple baseline algorithm for the two-sided optimal preconditioning problem \eqref{eq:SDP-two-sided} using bisection. This algorithm is easy to implement in practice, although it may be slow for larger problems. In Section \ref{sec:potential-reduction}, we will introduce an interior point algorithm with polynomial complexity, and comparison with the baseline algorithm will facilitate in understanding its improvements.

Our bisection algorithm consists of the following three steps:
\begin{enumerate}
\item Start with some large $\kappa_{0}\geq1$ such that the SDP feasibility
problem 
\begin{align*}
\min_{D_1,D_2} 0\\
A^{T}D_{1}A\succeq D_{2}\\
\kappa_{0}D_{2}\succeq A^{T}D_{1}A\\
D_1 \succeq I_m
\end{align*}
 has a solution. A choice that always works is $\kappa_{0}=\kappa(A^{T}A)$.
If we have prior information that there exists some $D_{1},D_{2}$
such that one of $\kappa(A^{T}D_{1}A)$, $\kappa(D_{2}^{-1/2}A^{T}AD_{2}^{-1/2})$,
or $\kappa(D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2})$ is smaller than
$\kappa(A^{T}A)$, we can set $\kappa_{0}$ to that number as a warm
start. Popular candidates for such $D_{1},D_{2}$ could be based on
the diagonals or row/column standard deviations of $A$, or other
matrix scaling techniques such as matrix equilibriation \citep{takapoui2016preconditioning} and Ruiz scalings \citep{ruiz2001scaling}.
Set the upper bound $\overline{\kappa}=\kappa_{0}$ and lower bound
$\underline{\kappa}=1$.
\item Solve the SDP feasibility problem 
\begin{align*}
\min_{D_{1},D_{2}}0\\
A^{T}D_{1}A\succeq D_{2}\\
\frac{\overline{\kappa}+\underline{\kappa}}{2}D_{2}\succeq A^{T}D_{1}A\\
D_1 \succeq I_m
\end{align*}
If the problem is feasible, set $\frac{\overline{\kappa}+\underline{\kappa}}{2}$
to be the new \emph{upper} bound $\overline{\kappa}$. If the problem
is infeasible, set $\frac{\overline{\kappa}+\underline{\kappa}}{2}$
to be new \emph{lower} bound $\underline{\kappa}$.
\item Solve the SDP feasibility problems iteratively while updating the
upper and lower bounds, until $\overline{\kappa}-\underline{\kappa}<\epsilon$
for some tolerance parameter $\epsilon$. The final set of feasible
solutions $D_{1},D_{2}$ will provide an $\epsilon$-optimal two-sided
preconditioning.
\end{enumerate}

The algorithm can be improved via intelligent choices of the updates to lower and upper bounds by exploiting the quasi-convexity structure.
There is also a geometric interpretation of each feasibility problem
with a fixed parameter $\kappa$: it looks for $D_{1},D_{2}$ such
that the ellipsoid defined by $D_{2}$, with axes of symmetry the
coordinate axes, is inscribed in the ellipsoid defined by $A^{T}D_{1}A$,
and such that expanding $D_{2}$ by a factor of $\kappa$ will encapsulate
the ellipsoid defined by $A^{T}D_{1}A$. Such inscribing and containing
ellipsoids have been used in the ellipsoid method, where the ellipsoids
are not constrained to be symmetric along coordinate axes. The geometric
interpretation also makes it clear that the optimal value $\kappa^{\ast}\geq1$
is achieved in the optimization problem. Also compare with the approach
in \cite{jambulapati2020fast}, which develop constant-factor optimal algorithms based on structured
mixed packing and covering semidefinite programs.

Note that the bisection algorithm finds an $\epsilon$-optimal solution
in $O(\log\frac{1}{\epsilon})$ iterations, where each iteration requires
solving an SDP feasibility problem. In practice, the bisection algorithm usually converges in less than 10 updates with $\epsilon = 0.01$ on most test cases of moderate size from the datasets considered in this paper (see Section \ref{sec:experiments}). 

\subsection{An Interior Point Algorithm for Optimal Diagonal Preconditioning}
\label{sec:potential-reduction}
Although the baseline algorithm introduced above is easy to implement, it suffers from sub-optimal complexity in theory and limited problem size in practice. In this section, we focus
on developing an interior point method that finds an $\epsilon$-optimal
solution in $O(\log\frac{1}{\epsilon})$ iterations, where each
iteration only consists of a Newton update step. This enjoys better
complexity than the baseline algorithm based on bisection, which requires solving an SDP feasibility problem at each iteration. Our algorithm draws inspirations from interior point
methods for linear programming and semidefinite programming 
\citep{mizuno1992new,ye1992potential,ye1995neumann,nesterov1997self},
particularly \cite{nesterov1997self}
on directions of Newton updates in interior point methods for SDPs and \cite{ye1995neumann}
on the ``Von Neumann economic growth problem'' \citep{von1937uber,neumann1945model}. 
%Add a remark on the connection to the Von Neumann problem of the right preconditioning problem.

Recall the reformulated two-sided optimal diagonal preconditioning problem in \eqref{eq:SDP-two-sided}. For ease of exposition, we present the algorithm and theory for the following right preconditioning problem by setting $D_1=I_m$ in \eqref{eq:SDP-two-sided}: %Extension to the two-sided problem can be found in the appendix.
\begin{align*}
\min_{\kappa\geq0}\kappa\\
A^{T}A\succeq D\\
\kappa D\succeq A^{T}A
\end{align*}
Let $\kappa^{\ast}\in[1,\infty)$ be optimal objective value of the above problem. Following \cite{ye1995neumann}, with $M=A^TA$, we define the \textbf{potential function} on $(\kappa^\ast,\infty)$
as
\begin{align*}
P(\kappa) & :=\sum_{i}\log\lambda_{i}(M-D^{\kappa})+\sum_{i}\log\lambda_{i}(\kappa D^{\kappa}-M)+\sum_{i}\log D_{ii}^{\kappa}
\end{align*}
where $D^{\kappa}$ is the \textbf{analytic center} of the feasible
region \textbf{
	\begin{align*}
	\Gamma(\kappa) & =\{D\succeq0:D\text{ diagonal};M\succeq D;\kappa D\succeq M\}
	\end{align*}
} which is simply the unique maximizer of the strictly concave problem
\begin{align*}
\max_{D\succeq0\text{ diagonal}} & \sum_{i}\log\lambda_{i}(M-D)+\sum_{i}\log\lambda_{i}(\kappa D-M)+\sum_{i}\log D_{ii}\\
& \Longleftrightarrow\\
\max_{D\succeq0\text{ diagonal}} & \log\det(M-D)+\log\det(\kappa D-M)+\log\det D
\end{align*}

See also \cite{mizuno1993adaptive,luo1998superlinear,sturm1999symmetric}
for the use of analytic centers in path-following and potential reduction
interior point algorithms for LP and SDP problems. 

The geometric interpretation of the problem makes it clear that if
the feasible region $\Gamma(\kappa^{0})$ has a non-empty interior
for some $\kappa^{0}<\infty$, then the feasible region $\Gamma(\kappa)$
has a non-empty interior for all $\kappa\geq\kappa^{0}$, so that
the analytic center is well defined. At the optimal objective value
$\kappa^{\ast}\geq1$, however, the solution set has no interior because
it must be the case that $\lambda_{n}(\kappa D-M)=0$ for any $D$
in the solution set, where $\lambda_{1}\geq\lambda_{2}\geq\cdots\geq\lambda_{n}$
are the eigenvalues of a matrix, and so perturbing $D$ in some direction
by any amount will violate the constraint $M\succeq D$. 
\begin{lemma}
	For $M\succ0,$ the feasible set of the feasibility problem 
	\begin{align*}
	\min_{D\succeq0}0\\
	M\succeq D\\
	\kappa D\succeq M
	\end{align*}
	has bounded non-empty interior for any $\kappa>\kappa^{\ast}$.
\end{lemma}
Next, we show that the potential function is monotonic in $\kappa$,
and that it is bounded away from $P(\kappa^{\ast})$, for any $\kappa$
large. This implies that $P(\kappa)$ is a reasonable measure of the progress of an algorithm:
to obtain an approximate optimal solution to the optimal preconditioning problem, it suffices to reduce the potential function by a constant
amount at every step and terminate when the potential function is
reduced below a certain threshold determined by accuracy $\epsilon$. This is summarized in the following two results. All proofs in this section can be found in the appendix.
\begin{proposition}\label{prop:monotonicity}
	If $\kappa_{0}>\kappa_{1}>\kappa^{\ast}$, then $P(\kappa_{0})>P(\kappa_{1})$. 
\end{proposition}
%
\begin{proposition}\label{prop:lower bound}
	Let $t$ satisfy $\kappa^{\ast}\leq2^{t}$, then for any $\overline{\kappa}>\kappa^{\ast}+2^{-t}$,
	we have
	\begin{align*}
	P(\overline{\kappa}) & >-Cnt
	\end{align*}
	for some universal constant that only depends on $M$. 
\end{proposition}
These two results imply that if $P(\kappa)<O(-nt)$, then we must
have $\kappa\leq\kappa^{\ast}+2^{-t}$. Therefore, if we can find a
$D$ whose associated potential is below the threshold of $O(n\log\epsilon)$,
we have found an approximate solution that yields a condition number
that is within $\epsilon$ of the optimal condition number. Our goal
is then to design an algorithm that achieves constant reduction of
the potential at every iteration, which would guarantee an iteration
complexity of $O(\log\frac{1}{\epsilon})$. 

In the next two subsections, we develop potential reduction algorithms based on this idea, using exact and approximate analytic centers, respetively. Before doing so, we show that the analytic center satisfies an equality condition that is useful in the analysis of the reduction of the potential function. It is essentially the first order condition of the convex optimziation problem. Since it also serves an important role in the Newton step, we state it in a particular form in the next lemma. 
\begin{lemma}
	The analytic center $D$ of the feasible region $\Gamma(\kappa)$
	satisfies 
	\begin{align*}
	Z+\kappa Y & =X
	\end{align*}
	where with $R:=M-D$, $S:=\kappa D-M$,  \begin{align*}
	X&=R^{-1},Y=S^{-1},Z=D^{-1}
	\end{align*}
\end{lemma}

\subsection{Analysis of Potential Reduction with Exact Analytic Centers}

Let $D^{0},D^{1}$ be the analytic centers of $\Gamma^{0}=\Gamma(\kappa^{0})$
and $\Gamma^{1}=\Gamma(\kappa^{1})$ for $\kappa^0,\kappa^1>\kappa^\ast$. With a suitable choice of $\Delta\kappa=\kappa^{0}-\kappa^{1}>0$,
we show that the analytic centers $D^{0}$ and $D^{1}$ are close,
and that 
\begin{align*}
P(\kappa^{1}) & \leq P(\kappa^{0})-\Omega(1)
\end{align*}
so that we can achieve constant reductions of the potential function
by updating from $D^{0}$ to $D^{1}$. To obtain $D^{1}$ from $D^{0}$,
we can use Newton iterations with a quadratic
convergence rate. The exact form of the Newton iteration is deferred
to the next subsection, where we propose a practical potential algorithm
using approximate analytic centers and only one Newton step.
%
\begin{theorem}
	\label{thm:exact center}Let $\overline{\kappa}$ be an upper bound of $\kappa^{\ast}$. Let $D^{0}$ and $D^{1}$ be the analytic centers of $\Gamma^{0}=\Gamma(\kappa^{0})$
	and $\Gamma^{1}=\Gamma(\kappa^{1})$ for $\kappa^{0},\kappa^{1}\in(\kappa^{\ast},\overline{\kappa})$.
	If $\Delta\kappa=\kappa^{0}-\kappa^{1}>0$ satisfies
	\begin{align*}
	\Delta\kappa & =\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}\\
	& =\frac{\beta}{e^{T}D^{0}\text{diag}((\kappa^{0}D^{0}-M)^{-1})e}
	\end{align*}
	for some sufficiently small $\beta\in(0,1)$ that only depends on
	$\overline{\kappa},M$, then 
	\begin{align*}
	\sqrt{Tr((D^{1})^{1/2}(D^{0})^{-1}(D^{1})^{1/2}-I)^{2}} & \leq c\cdot\beta\\
	\sqrt{Tr((D^{0})^{1/2}(D^{1})^{-1}(D^{0})^{1/2}-I)^{2}} & \leq c\cdot\beta
	\end{align*}
	for some constant $c$,
	and	$P(\kappa^{1}) \leq P(\kappa^{0})-\beta$.
	
\end{theorem}

%We have thus obtained a conceptual algorithm, which uses the exact
%analytic center, summarized in Algorithm \ref{alg:exact}.
\begin{algorithm}[Potential Reduction with Exact Analytic Center]
	\label{alg:exact}
\begin{enumerate}
	\normalfont 
	    \item Let $D^{0}$ be analytic center of $\Gamma(\kappa^{0})$ with some
	$\kappa^{0}>\kappa^{\ast}$. Set $k=0$. 
	
	\item  With a small fixed constant $0<\beta<1$, set 
	\begin{align*}
	\Delta\kappa^{k} & =\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})},
	\end{align*}
and let $\kappa^{k+1}=\kappa^{k}-\Delta\kappa^{k}$.
	Then use Newton's method with updates of the form in Proposition \ref{prop:Newton step} to generate
	the exact analytic center $D^{k+1}$ of $\Gamma(\kappa^{k+1})$. 
	
	\item If $P(\kappa^{k+1})>O(-nt)$, set $k\leftarrow k+1$ and return
	to Step 1.
	\end{enumerate}
\end{algorithm}

\subsection{Algorithm with Approximate Analytic Center}

Given step size $\Delta\kappa$, in order to apply the potential reduction
algorithm, we still need to find the new analytic center $D^{1}$
corresponding to $\kappa^{0}-\Delta\kappa$. This can be achieved
using Newton iterations. However, it is not necessary to use exact
analytic centers. Instead, we can use an approximate analytic center
obtained from only one Newton update step, and show that the potential function
still reduces by a constant amount. Moreover, if we start from an approximate
analytic center, one Newton step with an appropriate step size $\Delta\kappa$
yields an approximate center that still achieves this constant reduction
in potential. We develop these results in this subsection. 

By an approximate analytic center, we mean a set of variables $(R,S,D,X,Y,Z)$
that satisfy the optimality conditions 
\begin{align*}
R & =M-D\succeq0\\
S & =\kappa D-M\succeq0\\
D & \succeq0\\
Z+\kappa Y & =X,
\end{align*}
but instead of requiring $RX=SY=DZ=I$ as is true for the exact analytic
center, we allow the products to be close to the identity $I$, where we use the following measure of proximity:
\begin{align*}
\delta(A,B) & :=\sqrt{Tr(B^{1/2}AB^{1/2}-I)^{2}}\\
& =\|B^{1/2}AB^{1/2}-I\|_{F}=\|A^{1/2}BA^{1/2}-I\|_{F}
\end{align*}
The second equality above follows from the fact that the Frobenius norm
is a spectral property for symmetric matrices. We may also check that
\begin{align*}
\delta(A,B) & =\sqrt{Tr((AB-I)^{2})}=\sqrt{Tr((BA-I)^{2})}
\end{align*}
As we will see in the following results, this is the appropriate measure
of proximity. The first result we show is that starting from an exact analytic
center for $\Gamma(\kappa^{0})$, we can obtain a feasible point in
$\Gamma(\kappa^{1})$ that is an $O(\beta)$ approximate analytic center.
\begin{proposition}
	\label{prop:initial}
	Let $D^{0}$ be the exact analytic center of $\kappa^{0}$. Define
	$R_{0}=M-D_{0}$, $S_{0}=\kappa_{0}D_{0}-M$ and $X_{0}=R_{0}^{-1},Y_{0}=S_{0}^{-1},Z_{0}=D_{0}^{-1}$.	Further, let $\Delta\kappa=\kappa^{0}-\kappa^{1}$ with $\Delta\kappa=\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}$
	where $\beta\in(0,1)$ is a sufficiently small constant, and 
	\begin{align*}
	\overline{R}^{0} & =R^{0},\overline{S}^{0}=-\Delta\kappa D^{0}+S^{0},\overline{D}^{0}=D^{0}\\
	\overline{X}^{0} & =X^{0},\overline{Y}^{0}=Y^{0},\overline{Z}^{0}=\Delta\kappa Y^{0}+Z^{0}
	\end{align*}
	Then, the new variables satisfy 
	\begin{align*}
	\overline{R}^{0} & =M-\overline{D}^{0}\succeq0\\
	\overline{S}^{0} & =\kappa^{1}\overline{D}^{0}-M\succeq0\\
	\overline{D}^{0} & \succeq0
	\end{align*}
	and $\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0}=\overline{X}^{0}$.
	Moreover, $\delta(\overline{S}^{0},\overline{Y}^{0})\leq\beta,\delta(\overline{D}^{0},\overline{Z}^{0})\leq\beta,\delta(\overline{R}^{0},\overline{X}^{0})=0$.
\end{proposition}
Next we show that this set of variables $(\overline{R}^{0},\overline{S}^{0},\overline{D}^{0},\overline{X}^{0},\overline{Y}^{0},\overline{Z}^{0})$
can be used as an initial set to generate a new $ O(\beta^{2}) $ approximate center
for $\kappa^{1}$, using a Newton step. This also implies that starting from an approximate analytic center we can obtain an exact analytic center by applying the Newton iterations with quadratic convergence. Here to ensure the symmetry
of updates in the Newton step, we use the Nesterov-Todd direction
\citep{todd1998nesterov,nesterov1997self}. 

\begin{proposition}
   \label{prop:Newton step}
   Let $(\overline{R}^{0},\overline{S}^{0},\overline{D}^{0},\overline{X}^{0},\overline{Y}^{0},\overline{Z}^{0})$
	be any set that satisfy 
	\begin{align*}
	\overline{R}^{0} & =M-\overline{D}^{0}\succeq0\\
	\overline{S}^{0} & =\kappa^{1}\overline{D}^{0}-M\succeq0\\
	\overline{D}^{0} & \succeq0
	\end{align*}
	and $\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0}=\overline{X}^{0}$,
	with 
	\begin{align*}
	\delta(\overline{R}^{0},\overline{X}^{0})=\|(\overline{R}^{0})^{\frac{1}{2}}\overline{X}^{0}(\overline{R}^{0})^{\frac{1}{2}}-I\|_{F} & \leq\beta\\
	\delta(\overline{D}^{0},\overline{Z}^{0})=\|(\overline{D}^{0})^{\frac{1}{2}}\overline{Z}^{0}(\overline{D}^{0})^{\frac{1}{2}}-I\|_{F} & \leq\beta\\
	\delta(\overline{S}^{0},\overline{Y}^{0})=\|(\overline{S}^{0})^{\frac{1}{2}}\overline{Y}^{0}(\overline{S}^{0})^{\frac{1}{2}}-I\|_{F} & \leq\beta
	\end{align*}
	for some $\beta\in(0,1)$.	Let $X^{1},Y^{1},Z^{1},R^{1},S^{1},D^{1}$ be defined by 
	\begin{align*}
	X^{1} & =\overline{X}^{0}+\Delta X,Y^{1}=\overline{Y}^{0}+\Delta Y,Z^{1}=\overline{Z}^{0}+\Delta Z\\
	R^{1} & =\overline{R}^{0}+\Delta R,S^{1}=\overline{S}^{0}+\Delta S,D^{1}=\overline{D}^{0}+\Delta D
	\end{align*}
	where the increments $\Delta$s are given by the Newton step %
	\begin{comment}
	The Newton step is to ensure 
	\begin{align*}
	\overline{R}^{0} & =M-\overline{D}^{0}\succeq0\\
	\overline{S}^{0} & =\kappa^{1}\overline{D}^{0}-M\succeq0\\
	\overline{D}^{0} & \succeq0
	\end{align*}
	and 
	\begin{align*}
	\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0} & =\overline{X}^{0}
	\end{align*}
	still holds. 
	
	Regular Newton step is
	
	\begin{align*}
	\overline{D}^{0}\cdot\Delta Z+\overline{Z}^{0}\cdot\Delta D & =I-\overline{D}^{0}\cdot\overline{Z}^{0}\\
	\overline{R}^{0}\cdot\Delta X+\overline{X}^{0}\cdot\Delta R & =I-\overline{R}^{0}\cdot\overline{X}^{0}\\
	\overline{S}^{0}\cdot\Delta Y+\overline{Y}^{0}\cdot\Delta S & =I-\overline{S}^{0}\cdot\overline{Y}^{0}
	\end{align*}
	but here we need to use the Nesterov-Todd direction to ensure symmetry
	of updates. 
	\end{comment}
	\begin{align*}
	\Delta Z+W^{-1}\Delta DW^{-1} & =(\overline{D}^{0})^{-1}-\overline{Z}^{0}\\
	\Delta X+U^{-1}\Delta RU^{-1} & =(\overline{R}^{0})^{-1}-\overline{X}^{0}\\
	\Delta Y+V^{-1}\Delta S & V^{-1}=(\overline{S}^{0})^{-1}-\overline{Y}^{0}
	\end{align*}
	{} and 
	$\Delta R  =-\Delta D,\Delta S=\kappa^{1}\Delta D,\Delta X=\Delta Z+\kappa^{1}\Delta Y$,
	where $U,V,W$ are the geometric means 
	\begin{align*}
	U & =(\overline{R}^{0})^{1/2}((\overline{R}^{0})^{1/2}\overline{X}^{0}(\overline{R}^{0})^{1/2})^{-1/2}(\overline{R}^{0})^{1/2}\\
	V & =(\overline{S}^{0})^{1/2}((\overline{S}^{0})^{1/2}\overline{Y}^{0}(\overline{S}^{0})^{1/2})^{-1/2}(\overline{S}^{0})^{1/2}\\
	W & =(\overline{D}^{0})^{1/2}((\overline{D}^{0})^{1/2}\overline{Z}^{0}(\overline{D}^{0})^{1/2})^{-1/2}(\overline{D}^{0})^{1/2}
	\end{align*}
	to ensure that updates are symmetric. Then we have 
	\begin{align*}
	\delta(R^{1},X^{1})=\|(R^{1})^{\frac{1}{2}}X^{1}(R^{1})^{\frac{1}{2}}-I\|_{F} & \leq\frac{1}{2}\frac{\beta^{2}}{1-\beta}\\
	\delta(S^{1},Y^{1})=\|(S^{1})^{\frac{1}{2}}Y^{1}(S^{1})^{\frac{1}{2}}-I\|_{F} & \leq\frac{1}{2}\frac{\beta^{2}}{1-\beta}\\
	\delta(D^{1},Z^{1})=\|(D^{1})^{\frac{1}{2}}Z^{1}(D^{1})^{\frac{1}{2}}-I\|_{F} & \leq\frac{1}{2}\frac{\beta^{2}}{1-\beta}
	\end{align*}
	and 
	\begin{align*}
	\|(\overline{D}^{0})^{-\frac{1}{2}}D^{1}(\overline{D}^{0})^{-\frac{1}{2}}-I\|_{F} & \le\frac{\beta}{1-\beta}.
	\end{align*}
\end{proposition}
%
Our next result shows that starting from an $O(\delta)$ approximate
center $(R^{0},S^{0},D^{0},X^{0},Y^{0},Z^{0})$ instead of an exact
center for $\kappa^{0}$, by following the procedures described in
Proposition \ref{prop:initial} to form the initial set $(\overline{R}^{0},\overline{S}^{0},\overline{D}^{0},\overline{X}^{0},\overline{Y}^{0},\overline{Z}^{0})$
for $\kappa^{1}$, this intial set also satisfies the closeness conditions
\begin{align*}
\delta(\overline{R}^{0},\overline{X}^{0}) & \leq\delta',\delta(\overline{D}^{0},\overline{Z}^{0})\leq\delta',\delta(\overline{S}^{0},\overline{Y}^{0})\leq\delta'
\end{align*}
for $\delta'=\beta+\delta$, i.e. it is an $O(\beta+\delta)$ approximate
analytic center for $\kappa^{1}$, for $\delta$ sufficiently small.
This $O(\beta+\delta)$ approximate center can then be used in the
Newton step in Proposition \ref{prop:Newton step} to obtain
an $O((\beta+\delta)^{2})=O(\delta)$ approximate center for $\kappa^{1}$,
thus ensuring that we can go from an $O(\delta)$ approximate center
for $\kappa^{0}$ to an $O(\delta)$ approximate center for $\kappa^{1}$
with a single Newton step. 
\begin{proposition}\label{prop:approximate}
	Suppose that $(R^{0},S^{0},D^{0},X^{0},Y^{0},Z^{0})$ satisfy 
	\begin{align*}
	R^{0} & =M-D^{0}\succeq0\\
	S^{0} & =\kappa^{0}S^{0}-M\succeq0\\
	D^{0} & \succeq0\\
	Z^{0}+\kappa^{0}Y^{0} & =X^{0}
	\end{align*}
	with $\delta(R^{0},X^{0})\leq\delta,\delta(D^{0},Z^{0})\leq\delta,\delta(S^{0},Y^{0})\leq\delta$
	for some $\delta\in(0,1)$. Further, let $\Delta\kappa=\kappa^{0}-\kappa^{1}$
	with 
	\begin{align*}
	\Delta\kappa & =\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}
	\end{align*}
	where $\beta\in(0,1)$ is a sufficiently small constant, then with
	\begin{align*}
	\overline{R}^{0} & =R^{0},\overline{S}^{0}=-\Delta\kappa D^{0}+S^{0},\overline{D}^{0}=D^{0}\\
	\overline{X}^{0} & =X^{0},\overline{Y}^{0}=Y^{0},\overline{Z}^{0}=\Delta\kappa Y^{0}+Z^{0}
	\end{align*}
	we have 
	$\overline{R}^{0} =M-\overline{D}^{0}\succeq0$, $\overline{S}^{0} =\kappa^{1}\overline{D}^{0}-M\succeq 0$, $\overline{D}^{0} \succeq0$, $\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0} =\overline{X}^{0}$,
	and $\delta(\overline{R}^{0},\overline{X}^{0})  \leq\beta$, $\delta(\overline{S}^{0},\overline{Y}^{0})\leq\delta+\beta$, $\delta(\overline{D}^{0},\overline{Z}^{0})\leq\delta+\beta$.

\end{proposition}
%
The above three results guarantee that if we start from an $O(\delta)$
approximate center for $\kappa^{0}$, by taking a small but constant
step $\Delta\kappa$, a Newton update step yields an $O(\delta)$
approximate center for $\kappa^{1}=\kappa^{0}-\Delta\kappa$, and
we may iteratively generate approximate centers in this fashion. In
the next result, we show that approximate centers, as the name suggests,
yields a potential that is close to that of the exact center, and
we have thus obtained an algorithm with approximate centers, such that the reduction
in potential at every step is constant, and the termination criterion
is the same as before, when the potential drops below
some threshold. 
\begin{theorem}
	\label{thm:approximate center}Let $\overline{D}^{0}$ and $\overline{D}^{1}$
	be approximate centers for $\kappa^{0}$ and $\kappa^{1}=\kappa^{0}-\frac{\beta}{Tr(\overline{D}^{0}\cdot(\kappa^{0}\overline{D}^{0}-M)^{-1})}$
	respectively, obtained using the procedures in Proposition \ref{prop:initial}
	to generate a feasible point and the Newton update with Nesterov-Todd
	directions for $\beta$ sufficiently small. If 
	\begin{align*}
	\delta(\overline{R}^{0},\overline{X}^{0}) & \leq\delta,\delta(\overline{D}^{0},\overline{Z}^{0})\leq\delta,\delta(\overline{S}^{0},\overline{Y}^{0})\leq\delta
	\end{align*}
	for $\delta$ a small universal constant, then 
	\begin{align*}
	\delta(\overline{R}^{1},\overline{X}^{1}) & \leq\delta,\delta(\overline{D}^{1},\overline{Z}^{1})\leq\delta,\delta(\overline{S}^{1},\overline{Y}^{1})\leq\delta
	\end{align*}
	and $P(\overline{D}^{1},\kappa^{1})\leq P(\overline{D}^{0},\kappa^{0})-c\beta$
	for $c\in(0,1)$ a universal constant. 
\end{theorem}
%The above result thus guarantees that if we start from an approximate center that is accurate enough, we can always ensure that the updated approximate center obtained from a Newton step with Nesterov-Todd direction remain as accurate, given small but constant step size.
\begin{algorithm}[Potential Reduction with Approximate Analytic Center]
	\label{alg:approximate}
	\begin{enumerate}
	\normalfont
	    \item  Let $\overline{D}^{0}$ be an $O(\beta)$ approximate analytic
	center of $\Gamma(\kappa^{0})$ with $\kappa^{0}>\kappa^{\ast}$.
	Set $k=0$. 
	
	\item Let $\Delta\kappa^{k}=\frac{\beta}{Tr(\overline{D}^{0}\cdot(\kappa^{0}\overline{D}^{0}-M)^{-1})}$
	for fixed constant $0<\beta<1$ and let $\kappa^{k+1}=\kappa^{k}-\Delta\kappa^{k}$.
	Update 
	\begin{align*}
	\overline{S}^{0}\leftarrow & -\Delta\kappa\overline{D}^{0}+\overline{S}^{0}\\
	\overline{Z}^{0}\leftarrow & \Delta\kappa Y^{0}+\overline{Z}^{0}
	\end{align*}
	to obtain feasible point for $\kappa^{k+1}$. 
	
	\item Use Newton's update to generate approximate analytic center
	$\overline{D}^{k+1}$ of $\Gamma(\kappa^{k+1})$. 
	
	\item If $P(\kappa^{k+1})>O(-nt)$, set $k\leftarrow k+1$ and return
	to Step 1. 
	\end{enumerate}
\end{algorithm}
%
Our results in this section provided us with algorithms that generate two-sided
optimal diagonal preconditioners  given any fixed matrix $A$. In practice, we observe that running
the bisection algorithm for a few itereations already
generates a pair of preconditioners $(D_1,D_2)$ with high quality. In numerical experiments in Section \ref{sec:experiments}, we will implement the bisection algorithm to solve \eqref{eq:two-sided-problem} when
comparing with other preconditioning techniques, including the one-sided optimal diagonal preconditioners via SDPs introduced next in Section \ref{sec:DSDP}.

==> major revision/theory-old.tex <==
\section{Optimal Diagonal Preconditioning via Potential Reduction}
\label{sec:optimal}



We have shown that when the population correlation matrix is diagonally
dominant, diagonal preconditioning of design matrix by sample standard
deviations yields a reduction in condition number on the order of
$\sqrt{\kappa(D)}$ with high probability. However, many population
correlation matrices are not diagonally dominant, or we may not be
able to easily verify this condition. In such cases, we need an efficient
method to obtain a diagonal conditioner that does reduce the condition
number of any fixed design matrix $X$. We turn to this problem in
this section. 

Given a fixed design matrix $X\in\mathbb{R}^{n\times p}$, we are
interested in the optimal diagonal preconditioning matrix $D$, that
gives the minimal condition number of 
\begin{align*}
\min_{D\text{ diagonal, }D\succeq0}XD^{-\frac{1}{2}}
\end{align*}
among all diagonal preconditioners. We first reformulate the problem
to a quasi-convex SDP problem that can be solved with bisection, and
then provide a faster potential reduction algorithm with guarantee
on convergence. The purpose of studying the optimal diagonal preconditioning
procedure is the following:
\begin{enumerate}
	\item In settings where diagonal preconditioning helps to reduce condition
	number, we would like to compare the performances of diagonal preconditioning
	using column standard deviation/norm studied in the previous section
	with that of the optimal diagonal preconditioning, to see how much
	gap there is between the two. 
	\item In situations where diagonal preconditioning with sample standard
	deviation/norm does not actually reduce the condition number, we may
	instead use the optimal diagonal preconditioning procedure.
	\item We are also interested in how the result of adaptive diagonal preconditioning
	procedures, such as batch normalization, compares with the optimal
	diagonal preconditioning. This may help us understand the nature of
	such adaptive preconditioning procedures. 
\end{enumerate}

\subsection{Optimal Diagonal Preconditioning}

\textbf{}%
\begin{comment}
\textbf{(discussion with Boyd)}
\end{comment}

Writing $M=X^{T}X\in\mathbb{R}^{p\times p}$ and rewriting $D^{-\frac{1}{2}}$
as $D$, the optimal diagonal preconditioning problem is 
\begin{align*}
\min_{D\text{ diagonal}}\kappa(DMD)
\end{align*}
We can rewrite it as 
\begin{align*}
\min_{D,\kappa}\kappa\\
I\preceq DMD\preceq\kappa I
\end{align*}
The inequality constraints can be further simplified to $D^{-2}\preceq M\preceq\kappa D^{-2}$. The problem can thus be reformulated as 
\begin{align*}
\min_{\kappa,D}\kappa\\
s.t.M\succeq D\\
\kappa D\succeq M
\end{align*}
where $D$ is a diagonal matrix with strictly positive entries.

\begin{comment}
{[}FOC analysis:{]}Let $X$ and $Y$ be the multipliers of the first
and second constraints, with Lagrangian $\kappa-Tr(X(M-E))-Tr(Y(\kappa E-M))$.
The KKT condition is given by 
\begin{align*}
1 & =Tr(YE)\\
X & =\kappa Y
\end{align*}
But complementary slackness does not hold (strong duality does not
hold), otherwise they would imply $\kappa=1$. 
\end{comment}

We may solve this problem using bisection as follows. First find a large fixed $\kappa_{0}$ such that the convex
feasiblity SDP problem
\begin{align*}
\min_{D\succeq0}0\\
s.t.M\succeq D\\
\kappa_{0}D\succeq M
\end{align*}
has a solution. In practice, we can start with $\kappa_{0}=\kappa(M)$,
or if we have some prior information that there exists some $D_{0}$
that satisfies 
\begin{align*}
\kappa(D_{0}MD_{0}) & <\kappa(M)
\end{align*}
we can set $\kappa_{0}=\kappa(D_{0}MD_{0})$ as a warm start. Often
the choice $D_{0}\equiv\left(\text{diag}(M)\right)^{-1/2}$ or $D_{0}\equiv\left(\text{diag}(\text{std}(M))\right)^{-1/2}$
yields a smaller upper bound. 

Then, solve the feasibility problem
\begin{align*}
\min_{D\succeq0}0\\
s.t.M\succeq D\\
\frac{\kappa_{0}}{2}D\succeq M
\end{align*}

If it is feasible, then we know the optimal objective value is in
$[1,\frac{\kappa_{0}}{2}]$, otherwise it is in $[\frac{\kappa_{0}}{2},\kappa_{0}]$.
We can find an $\epsilon$-optimal solution in $O(\log\frac{1}{\epsilon})$
iterations. 

There is also a geometric interpretation of the feasibility problem
with parameter $\kappa$: it looks for an ellipsoid $E$ with axes
of symmetry the coordinate axes, such that it is inscribed in the
ellipsoid defined by $M$, and such that a multiple $\kappa$ of $E$
includes the ellipsoid defined by $M$. Such inscribing and containing
ellipsoids have been used the ellipsoid method, where the ellipsoids
are not constrained to be symmetric along coordinate axes. The geometric
interpretation also makes it clear that the optimal value $\kappa^{\ast}\geq1$
is achieved. 

\begin{algorithm}
	\label{alg:bisection}
	
	Step 0. Start with $\kappa^{0}>\kappa^{\ast}$ such that 
	\begin{align*}
	\min_{D\succeq0}0\\
	s.t.M\succeq D\\
	\kappa_{0}D\succeq M
	\end{align*}
	is feasible. Set $\kappa_{min}=1$, $\kappa_{\max}=\kappa_{0}$. 
	
	Step 1. Solve the feasibility problem 
	\begin{align*}
	\min_{D\succeq0}0\\
	s.t.M\succeq D\\
	\frac{\kappa_{\max}+\kappa_{\min}}{2}D\succeq M
	\end{align*}
	If it is feasible, then set $\kappa_{max}\leftarrow\frac{\kappa_{\max}+\kappa_{\min}}{2}$.
	Otherwise, set $\kappa_{\min}\leftarrow\frac{\kappa_{\max}+\kappa_{\min}}{2}$. 
	
	Step 2. If $\kappa_{max}-\kappa_{min}>\epsilon$, return to Step 1. 
\end{algorithm}

We next develop an interior point method that finds an $\epsilon$-optimal
diagonal scaling in $O(\log\frac{1}{\epsilon})$ iterations, where
each iteration consists of a Newton update step. This is in contrast
to the bisection algorithm, which also has $O(\log\frac{1}{\epsilon})$
iterations, but each iteration consists of solving a SDP feasibility
problem. The formulation and proof borrows ideas from interior point
methods for linear programming and semidefinite programming, in particular
\cite{mizuno1992new,ye1992potential,ye1995neumann,nesterov1997self},
most notable of which are \cite{nesterov1997self}
on Newton updates in SDP and \cite{ye1995neumann}
on the ``von Neumann economic growth problem''. 

\subsection{Interior Point Algorithms with Potential Reduction}

Recall the reformulated optimal diagonal preconditioning problem
\begin{align*}
\min_{D\succeq0}\kappa\\
s.t.M\succeq D\\
\kappa D\succeq M
\end{align*}

Following \cite{ye1995neumann}, we define the potential function
as
\begin{align*}
P(\kappa) & =\sum_{i}\log\lambda_{i}(M-D^{\kappa})+\sum_{i}\log\lambda_{i}(\kappa D^{\kappa}-M)+\sum_{i}\log D_{ii}^{\kappa}
\end{align*}
where $D^{\kappa}$ is the \emph{analytic center} of the feasible
region \textbf{
	\begin{align*}
	\Gamma(\kappa) & =\{D\succeq0:D\text{ diagonal};M\succeq D;\kappa D\succeq M\}
	\end{align*}
} which is simply the unique maximizer of the strictly concave problem
\begin{align*}
\max_{D\succeq0\text{ diagonal}} & \sum_{i}\log\lambda_{i}(M-D)+\sum_{i}\log\lambda_{i}(\kappa D-M)+\sum_{i}\log D_{ii}\\
& \Longleftrightarrow\\
\max_{D\succeq0\text{ diagonal}} & \log\det(M-D)+\log\det(\kappa D-M)+\log\det D
\end{align*}

See also \cite{mizuno1993adaptive,luo1998superlinear,sturm1999symmetric}
for the use of analytic centers in path-following and potential reduction
interior point algorithms for LP and SDP problems. 

The geometric interpretation of the problem makes it clear that if
the feasible region $\Gamma(\kappa^{0})$ has a non-empty interior
for some $\kappa^{0}<\infty$, then the feasible region $\Gamma(\kappa)$
has a non-empty interior for all $\kappa\geq\kappa^{0}$, so that
the analytic center is well defined. At the optimal objective value
$\kappa^{\ast}\geq1$, however, the solution set has no interior because
it must be the case that $\lambda_{p}(\kappa D-M)=0$ for any $D$
in the solution set, where $\lambda_{1}\geq\lambda_{2}\geq\cdots\geq\lambda_{p}$
are the eigenvalues of a matrix, and so perturbing $D$ in some direction
by any amount will violate the constraint $M\succeq D$. 
\begin{lemma}
	For $M\succ0,$ the feasible set of the feasibility problem 
	\begin{align*}
	\min_{D\succeq0}0\\
	s.t.M\succeq D\\
	\kappa D\succeq M
	\end{align*}
	has bounded non-empty interior for all $\kappa>\kappa^{\ast}$.
\end{lemma}
Next we show that the potential function is monotonic in $\kappa$,
and that it is bounded away from $P(\kappa^{\ast})$, for any $\kappa$
large, so that it is a reasonable measure of the progress of the problem:
we just need to be able to reduce the potential function by a constant
amount at every step and terminate when the potential function is
reduced below a certain threshold determined by accuracy $\epsilon$. 
\begin{proposition}\label{prop:monotonicity}
	If $\kappa_{0}>\kappa_{1}>\kappa^{\ast}$, then $P(\kappa_{0})>P(\kappa_{1})$. 
\end{proposition}
\proof{Proof}
See the appendix.
	\hfill \halmos
\endproof
%
\begin{proposition}\label{prop:lower bound}
	Let $t$ satisfy $\kappa^{\ast}\leq2^{t}$, then for any $\overline{\kappa}>\kappa^{\ast}+2^{-t}$,
	we have
	\begin{align*}
	P(\overline{\kappa}) & >-Cpt
	\end{align*}
	for some universal constant that only depends on $M$. 
\end{proposition}
\proof{Proof}
See the appendix.\hfill \halmos 
\endproof
These two results imply that if $P(\kappa)<O(-pt)$, then we must
have $\kappa\leq\kappa^{\ast}+2^{-t}$. Therefore if we can find a
$D$ whose associated potential is below the threshold of $O(p\log\epsilon)$,
we have found an approximate solution that yields a condition number
that is within $\epsilon$ of the optimal condition number. Our goal
is then to design an algorithm that achieves constant reduction of
the potential at every iteration, which would guarantee an iteration
complexity of $O(\log\frac{1}{\epsilon})$. 

In the next two subsections, we develop potential reduction algorithms based on this idea, using exact and and approximate analytic centers, respetively. Before doing so, we show that the analytic center satisfies an equality condition that is useful in the proof of the reduction of potential function. This is essentially the first order condition of the convex optimziation problem, but because it also serves an important role in the Newton reduction step, we state it is a particular form in the next lemma. 
\begin{lemma}
	The analytic center $D$ of the feasible region $\Gamma(\kappa)$
	satisfies 
	\begin{align*}
	Z+\kappa Y & =X
	\end{align*}
	where \begin{align*}
	X&=R^{-1},Y=S^{-1},Z=D^{-1},R=M-D,S=\kappa D-M
	\end{align*}
\end{lemma}
\proof{Proof}
	Since $D$ solves the convex problem
	\begin{align*}
	& \max_{D}\log\det(M-D)+\log\det(\kappa D-M)+\log\det D
	\end{align*}
	The first order condition implies 
	\begin{align*}
	-(M-D)^{-1}+\kappa(\kappa D-M)^{-1}+D^{-1} & =0
	\end{align*}
	so if we define $R=M-D$ and $S=\kappa D-M$, and 
	\begin{align*}
	X	=R^{-1},Y=S^{-1},Z=D^{-1}
	\end{align*}
	then we have $	Z+\kappa Y  =X$ and moreover $R+S=(\kappa-1)D$. 
	\hfill \halmos
\endproof

\subsection{Analysis of Potential Reduction with Exact Analytic Center}

Let $D^{0},D^{1}$ be the analytic centers of $\Gamma^{0}=\Gamma(\kappa^{0})$
and $\Gamma^{1}=\Gamma(\kappa^{1})$. With a suitable choice of $\Delta\kappa=\kappa^{0}-\kappa^{1}>0$,
we show that the analytic centers $D^{0}$ and $D^{1}$ are close,
and that 
\begin{align*}
P(\kappa^{1}) & \leq P(\kappa^{0})-\Omega(1)
\end{align*}
so that we can achieve constant reduction of the potential function
by going from $D^{0}$ to $D^{1}$. To obtain $D^{1}$ from $D^{0}$,
we can use symmetrized versions of Newton iterations with a quadratic
convergence rate. The exact form of the Newton iteration is deferred
to the next subsection, where we propose a practical potential algorithm
using approximate analytic centers and only one Newton step.
%
\begin{theorem}
	\label{thm:exact center}Let $\kappa^{\ast}\in[1,\infty)$ be the
	solution of 
	\begin{align*}
	\min_{D\succeq0}\kappa\\
	s.t.M\succeq D\\
	\kappa D\succeq M
	\end{align*}
	and let $\overline{\kappa}$ be a known upper bound of $\kappa^{\ast}$,
	i.e. 
	\begin{align*}
	\min_{D\succeq0}0\\
	s.t.M\succeq D\\
	\overline{\kappa}D\succeq M
	\end{align*}
	is feasible. 
	
	Let $D^{0}$ and $D^{1}$ be the analytic centers of $\Gamma^{0}=\Gamma(\kappa^{0})$
	and $\Gamma^{1}=\Gamma(\kappa^{1})$ for $\kappa^{0},\kappa^{1}\in(\kappa^{\ast},\overline{\kappa})$.
	If $\Delta\kappa=\kappa^{0}-\kappa^{1}>0$ satisfies
	\begin{align*}
	\Delta\kappa & =\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}\\
	& =\frac{\beta}{e^{T}D^{0}\text{diag}((\kappa^{0}D^{0}-M)^{-1})e}
	\end{align*}
	for some sufficiently small $\beta\in(0,1)$ that only depends on
	$\overline{\kappa},M$, then 
	\begin{align*}
	\sqrt{Tr((D^{1})^{1/2}(D^{0})^{-1}(D^{1})^{1/2}-I)^{2}} & \leq c\cdot\beta\\
	\sqrt{Tr((D^{0})^{1/2}(D^{1})^{-1}(D^{0})^{1/2}-I)^{2}} & \leq c\cdot\beta
	\end{align*}
	{} for some constant $c$
	and\textbf{
		\begin{align*}
		P(\kappa^{1}) & \leq P(\kappa^{0})-\beta
		\end{align*}
	}
\end{theorem}
\proof{Proof}
	See the appendix.
	\hfill \halmos
\endproof

We have thus obtained a conceptual algorithm, which uses the exact
analytic center, summarized in Algorithm \ref{alg:exact}.
\begin{algorithm}
	\label{alg:exact}
	
	Step 0. Let $D^{0}$ be analytic center of $\Gamma(\kappa^{0})$ with
	$\kappa^{0}>\kappa^{\ast}$. Set $k=0$. 
	
	Step 1. Let 
	\begin{align*}
	\Delta\kappa^{k} & =\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}
	\end{align*}
	for some small constant $0<\beta<1$ and let $\kappa^{k+1}=\kappa^{k}-\Delta\kappa^{k}$.
	Then use Newton's method described in the next section to generate
	the axact analytic center $D^{k+1}$ of $\Gamma(\kappa^{k+1})$. 
	
	Step 2. If $P(\kappa^{k+1})>O(-pt)$, set $k\leftarrow k+1$ and return
	to Step 1. 
\end{algorithm}

\subsection{Algorithm with Approximate Analytic Center}

Given step size $\Delta\kappa$, in order to apply the potential reduction
algorithm, we still need to find the new analytic center $D^{1}$
corresponding to $\kappa^{0}-\Delta\kappa$. This can be achieved
using Newton iterations. However, it is not necessary to use exact
analytic centers. Instead, we can use an approximate analytic center
obtained from only one Newton update step, and show that the max-potential
still reduces by a constant amount. Moreover, if we start from an approximate
analytic center, one Newton step with the appropriate step size $\Delta\kappa$
yields an approximate center that still achieves this constant reduction
in potential. We develop these results in this subsection. 

By an approximate analytic center, we mean a set of variables $(R,S,D,X,Y,Z)$
that satisfy the optimality conditions 
\begin{align*}
R & =M-D\succeq0,\\
S & =\kappa D-M\succeq0\\
D & \succeq0\\
Z+\kappa Y & =X
\end{align*}
but instead of requiring $RX=SY=DZ=I$ as is true for the exact analytic
center, we allow the products to be close to the identity $I$.

We define a measure of proximity of the products as follows 
\begin{align*}
\delta(A,B) & :=\sqrt{Tr(B^{1/2}AB^{1/2}-I)^{2}}\\
& =\|B^{1/2}AB^{1/2}-I\|_{F}=\|A^{1/2}BA^{1/2}-I\|_{F}
\end{align*}
where the equality follows from the fact that the Frobenius norm
is a spectral property for symmetric matrices. We may also check that
\begin{align*}
\delta(A,B) & =\sqrt{Tr((AB-I)^{2})}=\sqrt{Tr((BA-I)^{2})}
\end{align*}
As we will see in the following results, this is the appropriate measure
of proximity. The first result we show is that starting from an analytic
center for $\Gamma(\kappa^{0})$, we can obtain a feasible point in
$\Gamma(\kappa^{1})$ that is an $O(\beta)$ approximate analytic center.
\begin{proposition}
	\label{prop:initial}
	Let $D^{0}$ be the exact analytic center of $\kappa^{0}$. Define
	$R_{0}=M-D_{0}$, $S_{0}=\kappa_{0}D_{0}-M$ and $X_{0}=R_{0}^{-1},Y_{0}=S_{0}^{-1},Z_{0}=D_{0}^{-1}$.
	
	Further, let $\Delta\kappa=\kappa^{0}-\kappa^{1}$ with $\Delta\kappa=\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}$
	where $\beta\in(0,1)$ is a sufficiently small constant, and 
	\begin{align*}
	\overline{R}^{0} & =R^{0},\overline{S}^{0}=-\Delta\kappa D^{0}+S^{0},\overline{D}^{0}=D^{0}\\
	\overline{X}^{0} & =X^{0},\overline{Y}^{0}=Y^{0},\overline{Z}^{0}=\Delta\kappa Y^{0}+Z^{0}
	\end{align*}
	Then, the new variables satisfy 
	\begin{align*}
	\overline{R}^{0} & =M-\overline{D}^{0}\succeq0\\
	\overline{S}^{0} & =\kappa^{1}\overline{D}^{0}-M\succeq0\\
	\overline{D}^{0} & \succeq0
	\end{align*}
	and $\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0}=\overline{X}^{0}$.
	Moreover, $\delta(\overline{S}^{0},\overline{Y}^{0})\leq\beta,\delta(\overline{D}^{0},\overline{Z}^{0})\leq\beta,\delta(\overline{R}^{0},\overline{X}^{0})=0$.
\end{proposition}
\proof{Proof}
	We can readily verify that the new variables satisfy the desired equalities.
	When $\Delta\kappa$ is appropriately chosen as in the previous theorem,
	we can guarantee that $\overline{S}^{0}\succeq0$. Now 
	\begin{align*}
	\delta(\overline{S}^{0},\overline{Y}^{0})^{2}=Tr((\overline{S}^{0}\overline{Y}^{0}-I)^{2}) & =Tr((-\Delta\kappa D^{0}+S^{0})Y^{0}-I)^{2}\\
	& =Tr(-\Delta\kappa D^{0}Y^{0})^{2}\\
	& =Tr(-\Delta\kappa D^{0}(\kappa_{0}D_{0}-M)^{-1})^{2}\\
	& \leq(Tr(-\Delta\kappa D^{0}(\kappa_{0}D_{0}-M)^{-1}))^{2}=\beta^{2}
	\end{align*}
	where we have used $Tr(A^{2})=(TrA)^{2}-2\sigma_{2}(A)$ where $\sigma_{2}(A)=\sum_{i<j}\lambda_{i}\lambda_{j}$
	and $\lambda_{i}$ are the eigenvalues of $A$. Therefore, $\delta(\overline{S}^{0},\overline{Y}^{0})\leq\beta$.
	Similarly, $\delta(\overline{D}^{0},\overline{Z}^{0})\leq\beta$ and
	since $\overline{R}^{0}=R^{0},\overline{X}^{0}=X^{0}$, we have $\delta(\overline{D}^{0},\overline{Z}^{0})=0$
	\hfill \halmos
\endproof
Next we show that this set of variables $(\overline{R}^{0},\overline{S}^{0},\overline{D}^{0},\overline{X}^{0},\overline{Y}^{0},\overline{Z}^{0})$
can be used as an initial set to generate a new $ O(\beta^{2}) $ approximate center
for $\kappa^{1}$, using a Newton step. This also implies that starting from an approximate analytic center we can obtain an exact analytic center by applying the Newton iterations with quadratic convergence. Here to ensure the symmetry
of updates in the Newton step, we use the Nesterov-Todd direction
\cite{todd1998nesterov,nesterov1997self}. 

\begin{proposition}
	\label{prop:Newton step}Let \label{prop:Newton step}Let $(\overline{R}^{0},\overline{S}^{0},\overline{D}^{0},\overline{X}^{0},\overline{Y}^{0},\overline{Z}^{0})$
	be any set that satisfy 
	\begin{align*}
	\overline{R}^{0} & =M-\overline{D}^{0}\succeq0\\
	\overline{S}^{0} & =\kappa^{1}\overline{D}^{0}-M\succeq0\\
	\overline{D}^{0} & \succeq0
	\end{align*}
	and $\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0}=\overline{X}^{0}$,
	with 
	\begin{align*}
	\delta(\overline{R}^{0},\overline{X}^{0})=\|(\overline{R}^{0})^{\frac{1}{2}}\overline{X}^{0}(\overline{R}^{0})^{\frac{1}{2}}-I\|_{F} & \leq\beta\\
	\delta(\overline{D}^{0},\overline{Z}^{0})=\|(\overline{D}^{0})^{\frac{1}{2}}\overline{Z}^{0}(\overline{D}^{0})^{\frac{1}{2}}-I\|_{F} & \leq\beta\\
	\delta(\overline{S}^{0},\overline{Y}^{0})=\|(\overline{S}^{0})^{\frac{1}{2}}\overline{Y}^{0}(\overline{S}^{0})^{\frac{1}{2}}-I\|_{F} & \leq\beta
	\end{align*}
	for some $\beta\in(0,1)$. 
	
	Let $X^{1},Y^{1},Z^{1},R^{1},S^{1},D^{1}$ be defined by 
	\begin{align*}
	X^{1} & =\overline{X}^{0}+\Delta X,Y^{1}=\overline{Y}^{0}+\Delta Y,Z^{1}=\overline{Z}^{0}+\Delta Z\\
	R^{1} & =\overline{R}^{0}+\Delta R,S^{1}=\overline{S}^{0}+\Delta S,D^{1}=\overline{D}^{0}+\Delta D
	\end{align*}
	where the increments $\Delta$s are given by the Newton step %
	\begin{comment}
	The Newton step is to ensure 
	\begin{align*}
	\overline{R}^{0} & =M-\overline{D}^{0}\succeq0\\
	\overline{S}^{0} & =\kappa^{1}\overline{D}^{0}-M\succeq0\\
	\overline{D}^{0} & \succeq0
	\end{align*}
	and 
	\begin{align*}
	\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0} & =\overline{X}^{0}
	\end{align*}
	still holds. 
	
	Regular Newton step is
	
	\begin{align*}
	\overline{D}^{0}\cdot\Delta Z+\overline{Z}^{0}\cdot\Delta D & =I-\overline{D}^{0}\cdot\overline{Z}^{0}\\
	\overline{R}^{0}\cdot\Delta X+\overline{X}^{0}\cdot\Delta R & =I-\overline{R}^{0}\cdot\overline{X}^{0}\\
	\overline{S}^{0}\cdot\Delta Y+\overline{Y}^{0}\cdot\Delta S & =I-\overline{S}^{0}\cdot\overline{Y}^{0}
	\end{align*}
	but here we need to use the Nesterov-Todd direction to ensure symmetry
	of updates. 
	\end{comment}
	\begin{align*}
	\Delta Z+W^{-1}\Delta DW^{-1} & =(\overline{D}^{0})^{-1}-\overline{Z}^{0}\\
	\Delta X+U^{-1}\Delta RU^{-1} & =(\overline{R}^{0})^{-1}-\overline{X}^{0}\\
	\Delta Y+V^{-1}\Delta S & V^{-1}=(\overline{S}^{0})^{-1}-\overline{Y}^{0}
	\end{align*}
	{} and 
	\begin{align*}
	\Delta R & =-\Delta D,\Delta S=\kappa^{1}\Delta D,\Delta X=\Delta Z+\kappa^{1}\Delta Y
	\end{align*}
	where $U,V,W$ are the geometric means 
	\begin{align*}
	U & =(\overline{R}^{0})^{1/2}((\overline{R}^{0})^{1/2}\overline{X}^{0}(\overline{R}^{0})^{1/2})^{-1/2}(\overline{R}^{0})^{1/2}\\
	V & =(\overline{S}^{0})^{1/2}((\overline{S}^{0})^{1/2}\overline{Y}^{0}(\overline{S}^{0})^{1/2})^{-1/2}(\overline{S}^{0})^{1/2}\\
	W & =(\overline{D}^{0})^{1/2}((\overline{D}^{0})^{1/2}\overline{Z}^{0}(\overline{D}^{0})^{1/2})^{-1/2}(\overline{D}^{0})^{1/2}
	\end{align*}
	to ensure that updates are symmetric.
	
	Then we have 
	\begin{align*}
	\delta(R^{1},X^{1})=\|(R^{1})^{\frac{1}{2}}X^{1}(R^{1})^{\frac{1}{2}}-I\|_{F} & \leq\frac{1}{2}\frac{\beta^{2}}{1-\beta}\\
	\delta(S^{1},Y^{1})=\|(S^{1})^{\frac{1}{2}}Y^{1}(S^{1})^{\frac{1}{2}}-I\|_{F} & \leq\frac{1}{2}\frac{\beta^{2}}{1-\beta}\\
	\delta(D^{1},Z^{1})=\|(D^{1})^{\frac{1}{2}}Z^{1}(D^{1})^{\frac{1}{2}}-I\|_{F} & \leq\frac{1}{2}\frac{\beta^{2}}{1-\beta}
	\end{align*}
	and 
	\begin{align*}
	\|(\overline{D}^{0})^{-\frac{1}{2}}D^{1}(\overline{D}^{0})^{-\frac{1}{2}}-I\|_{F} & \le\frac{\beta}{1-\beta}
	\end{align*}
\end{proposition}
\proof{Proof}
	See the appendix.
	\hfill \halmos
\endproof
%
Our next result shows that starting from an $O(\delta)$ approximate
center $(R^{0},S^{0},D^{0},X^{0},Y^{0},Z^{0})$ instead of an exact
center for $\kappa^{0}$, by following the procedures described in
Proposition \ref{prop:initial} to form the initial set $(\overline{R}^{0},\overline{S}^{0},\overline{D}^{0},\overline{X}^{0},\overline{Y}^{0},\overline{Z}^{0})$
for $\kappa^{1}$, this intial set also satisfies the closeness conditions
\begin{align*}
\delta(\overline{R}^{0},\overline{X}^{0}) & \leq\delta',\delta(\overline{D}^{0},\overline{Z}^{0})\leq\delta',\delta(\overline{S}^{0},\overline{Y}^{0})\leq\delta'
\end{align*}
for $\delta'=\beta+\delta$, i.e. it is an $O(\beta+\delta)$ approximate
analytic center for $\kappa^{1}$, for $\delta$ sufficiently small.
This $O(\beta+\delta)$ approximate center can then be used in the
Newton iteration in Proposition \ref{prop:Newton step} to obtain
an $O((\beta+\delta)^{2})=O(\delta)$ approximate center for $\kappa^{1}$,
thus ensuring that we can go from an $O(\delta)$ approximate center
for $\kappa^{0}$ to an $O(\delta)$ approximate center for $\kappa^{1}$
with a Newton step. 
\begin{proposition}\label{prop:approximate}
	Suppose that $(R^{0},S^{0},D^{0},X^{0},Y^{0},Z^{0})$ satisfy 
	
	\begin{align*}
	R^{0} & =M-D^{0}\succeq0\\
	S^{0} & =\kappa^{0}S^{0}-M\succeq0\\
	D^{0} & \succeq0\\
	Z^{0}+\kappa^{0}Y^{0} & =X^{0}
	\end{align*}
	with $\delta(R^{0},X^{0})\leq\delta,\delta(D^{0},Z^{0})\leq\delta,\delta(S^{0},Y^{0})\leq\delta$
	for some $\delta\in(0,1)$. Further, let $\Delta\kappa=\kappa^{0}-\kappa^{1}$
	with 
	\begin{align*}
	\Delta\kappa & =\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}
	\end{align*}
	where $\beta\in(0,1)$ is a sufficiently small constant, then with
	\begin{align*}
	\overline{R}^{0} & =R^{0},\overline{S}^{0}=-\Delta\kappa D^{0}+S^{0},\overline{D}^{0}=D^{0}\\
	\overline{X}^{0} & =X^{0},\overline{Y}^{0}=Y^{0},\overline{Z}^{0}=\Delta\kappa Y^{0}+Z^{0}
	\end{align*}
	we have 
	$\overline{R}^{0} =M-\overline{D}^{0}\succeq0$, $\overline{S}^{0} =\kappa^{1}\overline{D}^{0}-M\succeq 0$, $\overline{D}^{0} \succeq0$, $\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0} =\overline{X}^{0}$,
	and $\delta(\overline{R}^{0},\overline{X}^{0})  \leq\beta$, $\delta(\overline{S}^{0},\overline{Y}^{0})\leq\delta+\beta$, $\delta(\overline{D}^{0},\overline{Z}^{0})\leq\delta+\beta$.

\end{proposition}
\proof{Proof}
    See the appendix.
	\hfill \halmos
\endproof
\textbf{}
%
The above three results guarantee that if we start from an $O(\delta)$
approximate center for $\kappa^{0}$, by taking a small but constant
step $\Delta\kappa$, a Newton update step yields an $O(\delta)$
approximate center for $\kappa^{1}=\kappa^{0}-\Delta\kappa$, and
we may iteratively generate approximate centers in this fashion. In
the next result, we show that approximate centers, as the name suggests,
yields a potential that is close to that of the exact center, and
so we have an algorithm with approximate centers, such that the reduction
in potential at every step is constant, and the termination criterion
is when the potential evaluated at the approximate center drops below
some threshold. 
\begin{theorem}
	\label{thm:approximate center}Let $\overline{D}^{0}$ and $\overline{D}^{1}$
	be approximate centers for $\kappa^{0}$ and $\kappa^{1}=\kappa^{0}-\frac{\beta}{Tr(\overline{D}^{0}\cdot(\kappa^{0}\overline{D}^{0}-M)^{-1})}$
	respectively, obtained using the procedures in Proposition \ref{prop:initial}
	to generate feasible point and the Newton update with Nesterov-Todd
	direction for $\beta$ sufficiently small. If 
	\begin{align*}
	\delta(\overline{R}^{0},\overline{X}^{0}) & \leq\delta,\delta(\overline{D}^{0},\overline{Z}^{0})\leq\delta,\delta(\overline{S}^{0},\overline{Y}^{0})\leq\delta
	\end{align*}
	for $\delta$ a small universal constant, then 
	\begin{align*}
	\delta(\overline{R}^{1},\overline{X}^{1}) & \leq\delta,\delta(\overline{D}^{1},\overline{Z}^{1})\leq\delta,\delta(\overline{S}^{1},\overline{Y}^{1})\leq\delta
	\end{align*}
	and $P(\overline{D}^{1},\kappa^{1})\leq P(\overline{D}^{0},\kappa^{0})-c\beta$
	for $c\in(0,1)$ a universal constant. 
\end{theorem}
\proof{Proof}
	See the appendix.
	\hfill \halmos
\endproof

\begin{algorithm}
	\label{alg:approximate}
	
	Step 0. Let $\overline{D}^{0}$ be an $O(\beta)$ approximate analytic
	center of $\Gamma(\kappa^{0})$ with $\kappa^{0}>\kappa^{\ast}$.
	Set $k=0$. 
	
	Step 1. Let $\Delta\kappa^{k}=\frac{\beta}{Tr(\overline{D}^{0}\cdot(\kappa^{0}\overline{D}^{0}-M)^{-1})}$
	for some small constant $0<\beta<1$ and let $\kappa^{k+1}=\kappa^{k}-\Delta\kappa^{k}$.
	Update 
	\begin{align*}
	\overline{S}^{0}\leftarrow & -\Delta\kappa\overline{D}^{0}+\overline{S}^{0}\\
	\overline{Z}^{0}\leftarrow & \Delta\kappa Y^{0}+\overline{Z}^{0}
	\end{align*}
	to obtain feasible point for $\kappa^{k+1}$. 
	
	Step 2. Use Newton's update to generate approximate analytic center
	$\overline{D}^{k+1}$ of $\Gamma(\kappa^{k+1})$. 
	
	Step 3. If $P(\kappa^{k+1})>O(-pt)$, set $k\leftarrow k+1$ and return
	to Step 1. 
\end{algorithm}
%
The above result thus guarantees that if we start from an approximate
center that is accurate enough, we can always ensure that the updated
approximate center obtained from a Newton step with Nesterov-Todd
direction remain as accurate, given small but constant step size.
Our results in this section provided us with two algorithms that generate
optimal diagonal preconditioners that guarantee reduction in condition
number, given any fixed matrix. In practice, we observe that running
the bisection algorithm or Newton update for a few itereations already
generates a good preconditioner, and that is what we implement when
comparing with other preconditioning methods. 

==> major revision/theory.tex <==
\section{Problem Setup and Algorithms}
\label{sec:optimal}

In this section, we turn to the two-sided optimal diagonal preconditioning
problem. For a matrix $A\in\mathbb{R}^{m\times n}$ with full rank, we want to find positive \emph{diagonal} matrices $D_1,D_2$ that solve the following minimization problem (the particular choice of exponents for $D_1,D_2$ will become clear shortly):
\begin{align}
\label{eq:two-sided-problem}
\min_{D_{1},D_{2}\succ0}\kappa(D_{1}^{1/2}AD_{2}^{-1/2})
\end{align}
There are two related \emph{one-sided} optimal diagonal preconditioning problems that seek diagonal matrices $D_1$ and $D_2$ which solve the following two distinct problems, respectively:
\begin{align}
\label{eq:left-sided-problem}
\min_{D_{1}\succ0}&\kappa(D_{1}^{1/2}A)\\
\label{eq:right-sided-problem}
\min_{D_{2}\succ0}&\kappa(AD_{2}^{-1/2})
\end{align}
 Note first that without loss of generality, we can always assume $m\geq n$, so that $A$ is a \emph{tall} matrix, since otherwise we may take the transpose of $A$ without changing the optimal solution pairs to the two-sided problem \eqref{eq:two-sided-problem}. For the one-sided problems \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem}, taking the transpose of $A$ essentially transforms one problem to the other. Moreover, for square matrices,
i.e., $m=n$, the three optimal preconditioning problems share the
solutions, since similar square matrices
have the same eigenvalues hence the same condition numbers. Finally, note that solutions are scale-invariant, since for any optimal
pair $(D_{1},D_{2})$ of diagonal preconditioners that achieves the
minimum objective value of \eqref{eq:two-sided-problem}, $(c_1D_{1},c_2D_{2})$ for any $c_1,c_2>0$ is also
a pair of optimal diagonal preconditioners, and similarly for \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem}. %For the purpose of reducing condition numbers, any optimal solution is sufficient.

%For now, we will primarily focus on developing algorithms for the two-sided problem \eqref{eq:two-sided-problem}. 
\textbf{Overview.} We will develop a baseline algorithm based on bisection that solves an equivalent reformulation of the two-sided problem \eqref{eq:two-sided-problem} in Section \ref{sec:bisection}, and then develop a polynomial time interior point algorithm in Section \ref{sec:potential-reduction}. This potential reduction procedure based on Newton updates with Nesterov-Todd directions can be adapted to other quasi-convex problems.  %The corresponding algorithms and theory for the one-sided problems \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem} can be obtained with straightforward reductions. 
In Section \ref{sec:DSDP}, we show that \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem} admit reformulations as standard dual SDP problems,
to which customized solvers can be applied to obtain solutions efficiently for large matrices. We then develop specialized algorithms for the one-sided problems based on this reformulation.
%In contrast, the two-sided problem \eqref{eq:two-sided-problem} does not admit an SDP reformulation. 
In Section \ref{sec:experiments}, we study the empirical performance
of these optimal preconditioning procedures. In general, one-sided optimal diagonal preconditioners are sufficient to achieve significant reductions in condition numbers, although there are instances where two-sided preconditioners are much better. In practice, we can handle problems of size up to $m \leq 200,000$ using our customized solver with random sampling. %In particular, we will investigate
%when and how two-sided optimal preconditioning improves upon the
%two one-sided preconditioners significantly in
%terms of condition number reduction, as well as when the two one-sided
%methods differ from each other.

\subsection{Problem Reformulation}
 We start by rewriting the two-sided optimal diagonal preconditioning problem \eqref{eq:two-sided-problem} in a more accessible form. First, note that for any matrix $A \in \mathbb{R}^{m\times n}$ with full rank and $m\geq n$, $\kappa(A)=\sqrt{\kappa(A^{T}A)}$, so we can instead minimize the condition
number of $(D_{1}^{1/2}AD_{2}^{-1/2})^{T}(D_{1}^{1/2}AD_{2}^{-1/2})=D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2}$.
As the condition number is scale-invariant, we can introduce a new
positive \emph{variable} $\kappa$ (to be distinguished from the condition
number $\kappa(M)$ of a matrix) and rewrite the resulting problem
as
\begin{align*}
\min_{\kappa,D_{1},D_{2}\succ0}\kappa\\
I_n\preceq D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2}\preceq\kappa I_n
\end{align*}
The objective above achieves its optimal value $\kappa^\ast:=(\min_{D_{1},D_{2}\succ0}\kappa(D_{1}^{1/2}AD_{2}^{-1/2}))^{2}$, and at any optimal solution $(D_1,D_2)$, $\lambda_{\min}(D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2})=1$ and $\lambda_{\max}(D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2})=\kappa^\ast$.

Next, the constraint $I_n\preceq D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2}\preceq\kappa I_n$
is equivalent to $D_{2}\preceq A^{T}D_{1}A\preceq\kappa D_{2}$, and, with diagonal matrices $D_1,D_2$, we can rewrite the problem in its final reformulation as
\begin{align}
\label{eq:SDP-two-sided}
\begin{split}
    \min_{\kappa\geq0} \kappa \\
A^{T}D_{1}A\succeq D_{2}\\
\kappa D_{2}\succeq A^{T}D_{1}A \\
D_1 \succeq I_m 
\end{split}
\end{align}
where we have replaced the strict inequalities $D_1,D_2\succ0$ by equivalently requiring $\kappa \geq 0$ and $D_1 \succeq I_m$. Since $A^TD_1A\succeq A^TA\succ 0$, $D_2$ and $\kappa$ in fact need to be both strictly positive. Note that the alternative constraint $D_2 \succeq I_n$ instead of $D_1 \succeq I_m$ does not work, however, since $m\geq n$ and $D_1$ could still have zero diagonal entries even if $D_2 \succ 0$.
The problem \eqref{eq:SDP-two-sided} is also scale-invariant, and we may further impose normalization constraints to make the solution unique. This is not necessary for the purpose of the baseline algorithm we develop in this section. For the interior point algorithm we develop in Section \ref{sec:potential-reduction}, we will impose an upper bound on $D_1$ to facilitate the definition of a potential function which we will aim to reduce. 
%However, as we will see, the interior point algorithm we develop based on potential reduction will find the unique solution with $\lambda_{\min}(D_1)=1$, so we do not need to explicitly impose the normalization constraint. 

Note also that the problem in \eqref{eq:SDP-two-sided} is a quasi-convex problem. To see this, let $d_1\in\mathbb{R}^m,d_2\in\mathbb{R}^n$ be the vector representations of the diagonal matrices $D_1,D_2$, and $d_3 \in \mathbb{R}^n$. With $d_{1i}$ denoting the $i$-th element of $d_1$, and $d_{2j},d_{3j}$ the $j$-th elements of $d_2,d_3$, \eqref{eq:SDP-two-sided} is equivalent to the following problem:
\begin{align}
\label{eq:quasi-convex}
\begin{split}
\min_{d_1,d_2,d_3\geq0} \max_j d_{3j}/d_{2j}\\
\sum_{i=1}^{m} d_{1i} a_i a_i^T - \sum_{j=1}^n d_{2j} e_j e_j^T   \succeq 0\\
\sum_{j=1}^n d_{3j} e_j e_j^T -\sum_{i=1}^{m} d_{1i} a_i a_i^T\succeq 0\\
d_1 - \mathbf{1}_m \geq 0
\end{split}
\end{align}
where vector $a_i$ is the $i$-th row of $A$ and $e_j \in \mathbb{R}^n$ is the vector whose $j$-th entry is 1 and zero otherwise. This problem is reminiscent of the Von Neumann economic growth problem \citep{neumann1945model}. %However, \eqref{eq:SDP-two-sided} is not equivalent to a standard SDP, because of the product term $\kappa D_2$.

\subsection{A Bisection Algorithm for Optimal Two-sided Diagonal Preconditioning}
\label{sec:bisection}
We start with a simple baseline algorithm for the two-sided optimal preconditioning problem \eqref{eq:SDP-two-sided} using bisection. This algorithm is easy to implement in practice, although it may be slow for larger problems. In Section \ref{sec:potential-reduction}, we will introduce an interior point algorithm with polynomial complexity, and comparison with the baseline algorithm will facilitate in understanding its improvements.

Our bisection algorithm consists of the following three steps:
\begin{enumerate}
\item Start with some large $\kappa_{0}\geq1$ such that the SDP feasibility
problem 
\begin{align*}
\min_{D_1,D_2} 0\\
A^{T}D_{1}A\succeq D_{2}\\
\kappa_{0}D_{2}\succeq A^{T}D_{1}A\\
D_1 \succeq I_m
\end{align*}
 has a solution. A choice that always works is $\kappa_{0}=\kappa(A^{T}A)$.
If we have prior information that there exists some $D_{1},D_{2}$
such that one of $\kappa(A^{T}D_{1}A)$, $\kappa(D_{2}^{-1/2}A^{T}AD_{2}^{-1/2})$,
or $\kappa(D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2})$ is smaller than
$\kappa(A^{T}A)$, we can set $\kappa_{0}$ to that number as a warm
start. Popular candidates for such $D_{1},D_{2}$ could be based on
the diagonals or row/column standard deviations of $A$, or other
matrix scaling techniques such as matrix equilibriation \citep{takapoui2016preconditioning} and Ruiz scalings \citep{ruiz2001scaling}.
Set the upper bound $\overline{\kappa}=\kappa_{0}$ and lower bound
$\underline{\kappa}=1$.
\item Solve the SDP feasibility problem 
\begin{align*}
\min_{D_{1},D_{2}}0\\
A^{T}D_{1}A\succeq D_{2}\\
\frac{\overline{\kappa}+\underline{\kappa}}{2}D_{2}\succeq A^{T}D_{1}A\\
D_1 \succeq I_m
\end{align*}
If the problem is feasible, set $\frac{\overline{\kappa}+\underline{\kappa}}{2}$
to be the new \emph{upper} bound $\overline{\kappa}$. If the problem
is infeasible, set $\frac{\overline{\kappa}+\underline{\kappa}}{2}$
to be new \emph{lower} bound $\underline{\kappa}$.
\item Solve the SDP feasibility problems iteratively while updating the
upper and lower bounds, until $\overline{\kappa}-\underline{\kappa}<\epsilon$
for some tolerance parameter $\epsilon$. The final set of feasible
solutions $D_{1},D_{2}$ will provide an $\epsilon$-optimal two-sided
preconditioning.
\end{enumerate}

The algorithm can be improved via intelligent choices of the updates to lower and upper bounds by exploiting the quasi-convexity structure.
There is also a geometric interpretation of each feasibility problem
with a fixed parameter $\kappa$: it looks for $D_{1},D_{2}$ such
that the ellipsoid defined by $D_{2}$, with axes of symmetry the
coordinate axes, is inscribed in the ellipsoid defined by $A^{T}D_{1}A$,
and such that expanding $D_{2}$ by a factor of $\kappa$ will encapsulate
the ellipsoid defined by $A^{T}D_{1}A$. Such inscribing and containing
ellipsoids are used in the ellipsoid method, where the ellipsoids
are not constrained to be symmetric along coordinate axes. The geometric
interpretation also makes it clear that the optimal value $\kappa^{\ast}\geq1$
is achieved in the optimization problem. Also compare with the approach
in \cite{jambulapati2020fast}, which develops constant-factor optimal algorithms for one-sided problems based on structured
mixed packing and covering semidefinite programs. 

Note that the bisection algorithm finds an $\epsilon$-optimal solution
in $O(\log\frac{1}{\epsilon})$ iterations, where each iteration requires
solving an SDP feasibility problem. In practice, the bisection algorithm usually converges in less than 10 updates with $\epsilon = 0.01$ on most test cases of moderate size from the datasets considered in this paper (see Section \ref{sec:experiments}). 

\subsection{An Interior Point Algorithm for Optimal Diagonal Preconditioning}
\label{sec:potential-reduction}
Although the baseline algorithm introduced in the previous section is easy to implement, it suffers from sub-optimal complexity in theory and limited problem size in practice. In this section, we focus
on developing an interior point method that finds an $\epsilon$-optimal
solution in $O(\log\frac{1}{\epsilon})$ iterations, where each
iteration only consists of a Newton update step. This enjoys better
complexity than the baseline algorithm based on bisection, which requires solving an SDP feasibility problem at each iteration. Our algorithm draws inspirations from interior point
methods for linear programming and semidefinite programming
\citep{mizuno1992new,ye1992potential,ye1995neumann,nesterov1997self},
particularly \cite{nesterov1997self}
on directions of Newton updates in interior point methods for SDPs and \cite{ye1995neumann}
on the ``Von Neumann economic growth problem'' \citep{von1937uber,neumann1945model}. Our general potential reduction procedure using the Nesterov-Todd
direction is potentially applicable to other settings with quasi-convex problems, and is therefore also of independent interest.
%Add a remark on the connection to the Von Neumann problem of the right preconditioning problem.

Recall the reformulated two-sided optimal diagonal preconditioning problem in \eqref{eq:SDP-two-sided}. Due to the scale invariance nature of the problem, we impose an additional constraint on $D_1$ and develop an interior point algorithm for the following equivalent problem:
\begin{align}
\label{eq:SDP-two-sided-upper-bound}
\begin{split}
    \min_{\kappa\geq0} \kappa \\
A^{T}D_{1}A\succeq D_{2}\\
\kappa D_{2}\succeq A^{T}D_{1}A \\
\hat \kappa I_m \succeq D_1 \succeq I_m 
\end{split}
\end{align}
where $\hat{\kappa}$ is some fixed large constant. One obvious choice is $\hat{\kappa}=\kappa(A^TA)$. Following \cite{ye1995neumann}, for each fixed $\kappa\geq \kappa^\ast$, we
denote the \textbf{feasible region} of the associated SDP feasibility
problem by \textbf{
\begin{align*}
\Gamma(\kappa): & =\{D_{1},D_{2}\text{ diagonal:}\text{ }A^{T}D_{1}A\succeq D_{2};\text{ }\kappa D_{2}\succeq A^{T}D_{1}A;\text{ }\hat \kappa I_m \succeq D_{1}\succeq I_{m}\}
\end{align*}
}and define the \textbf{analytic center} of $\Gamma(\kappa)$, denoted
by $(D_{1}(\kappa),D_{2}(\kappa))$, as the \emph{unique} maximizer
of 
\begin{align*}
\max_{D_{1},D_{2}\in \Gamma(\kappa)} & \log\det(A^{T}D_{1}A-D_{2})+\log\det(\kappa D_{2}-A^{T}D_{1}A)+\log\det(D_{1}-I_{m})+\log\det(\hat \kappa I_{m}-D_1)
\end{align*}
where the objective is strictly concave because of the strict concavity
of the log determinant function. Finally, we define the \textbf{potential
function} $P(\kappa)$ as the maximum objective value above, achieved at the analytic
centers $(D_{1}(\kappa),D_{2}(\kappa))$.

As we will demonstrate, the potential function is well-defined and a suitable measure of progress towards optimality, and the iterative algorithm we design will aim to reduce the potential function by a constant amount at each step. The analytic centers will
form the central path which converges to the optimal solution as $\kappa$
is reduced together with $P(\kappa)$. See also \cite{mizuno1993adaptive,luo1998superlinear,sturm1999symmetric,burer2002solving}
for the use of potential functions and analytic centers in path-following
and potential reduction interior point algorithms for LP, SDP and
nonlinear programming problems. To facilitate presentation, we summarize our result in the following general statement and leave the detailed treatment to Appendix \ref{sec:appendix_optimal}.

\begin{theorem}
\label{thm:general-statement}
    There exists an iterative algorithm which requires a single Newton update to  $(D_1,D_2)$ at each iteration that is guaranteed to decrease the potential function $P(\kappa)$ by a constant amount. The potential is guaranteed to decrease to $O(m\log\epsilon)$ after $O(\log \frac{1}{\epsilon})$ iterations, at which point $(D_1,D_2)$ satisfies $\kappa(D_{1}^{1/2}AD_{2}^{-1/2})-\kappa^\ast = O(\epsilon)$.
\end{theorem}
%
Our results in this section provide us with algorithms that generate two-sided
optimal diagonal preconditioners given any fixed matrix $A$ with full rank. They can be easily adapted to the one-sided optimal preconditioning problems \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem} as well. To our knowledge, our potential reduction algorithm is the first interior point algorithm for both the two-sided and one-sided optimal diagonal preconditioning problems. A potential concern is that the Newton updates may result in significant computation costs. In Appendix \ref{sec:first-order-methods}, we suggest some first order methods, including a first order version of the potential reduction algorithm, as alternatives to the algorithms in the main text. In practice, thanks to the sparse and low rank structure of the problems with large real datasets, our approach to find one-sided optimal diagonal preconditioners via solving dual SDPs with customized solvers, introduced in Section \ref{sec:DSDP}, is most efficient, and we may also use the procedure described in Section \ref{subsec:dual-SDP} based on these one-sided problems to obtain two-sided preconditioners. Nevertheless, the general potential reduction procedure introduced in this section can be adapted to solve other quasi-convex problems with PSD matrix variables, as is the case for problem \eqref{eq:quasi-convex}, with high accuracy when computation time is not the main constraint and bisection methods fail for large problems. %The applicability of the interior point algorithm introduced in this section is thus more general beyond the current particular problem.

%Thus, even though it may not be practically as efficient as the dual SDP approach for our particular problem, the audience of OR can potentially adapt it to solve their large quasi-convex problems with high accuracy, where the time to solve Newton updates is not a constraint factor. 

%In practice, we observe that running the bisection algorithm for a few iterations usually generates preconditioners $(D_1,D_2)$ with high quality for problems with moderate sizes. In numerical experiments in Section \ref{sec:experiments}, we will implement the bisection algorithm to solve \eqref{eq:two-sided-problem} when comparing with other preconditioning techniques, including the one-sided optimal diagonal preconditioners via SDPs introduced next in Section \ref{sec:DSDP}. 

==> optimization.tex <==
\section{Diagonal Preconditioning and Stochastic Convex Optimization}
\label{sec:optimization}

So far we have focused on diagonal preconditioning of design matrices.
We studied how preconditioning affects the condition number of the
design matrices, and also developed algorithms to compute optimal
diagonal preconditioners. These results have direct implications on
the convergence rates of iterative solvers of linear systems and first
order methods applied to quadratic objectives, since convergence rates
depend explicitly on the condition number of the (constant) Hessian
matrix $X^{T}X$. 

For general convex objective functions, convergence rates of first
order methods depend on the smoothness and convexity constants of
the function. It is therefore more challenging to study the impact
of preconditioning on the design matrix on the convergence of first
order methods on general convex objective functions, as we need to
investigate how the reduction in condition number of the design matrix
translates to improvements in the smoothness and convexity constants
of the objective function. In this section, we first give such a result
for a class of objective functions $f$ that correspond to the (regularized)
loss of an empirical risk minimization problem (\cite{shalev2013stochastic}),
and show that when $f$ is smooth and strongly convex, reductions
in the condition number of the objective is on the order of $\frac{\kappa(X)}{\kappa(X_{0})}$
where $X$ is the design matrix and $X_{0}$ is any preconditioned
design matrix with smaller condition number. For other more general
classes of convex objectives, we leave to future work to quantify
theoretically the impact of condition number on convergence rates.
However, we make the case that the optimal diagonal preconditioning
algorithms developed in the previous section is not limited to being
applied to fixed design matrices. We establish the connection of batch
normalization, a popular technique in machine learning, to adaptive
preconditioning, and develop an adaptive version of the optimal diagonal
preconditioning algorithm. We then conduct numerical experiments that
demonstrate the effectiveness of the optimal diagonal preconditioning
algorithm at speeding up first order methods in regression and classification
problems in the next section. 

\subsection{Convergence Rates for General Convex Problems}

The relationship between the complexity of first order methods and
the smoothness and convexity properties of the objective function
has been well established in the optimization literature. Here the
complexity is usually expressed in terms of the number of iterations
required to obtain an $\epsilon$-optimal solution. We summarize the
corresponding iteration complexities of solving 
\begin{align*}
\min_{\theta}f(\theta,X)
\end{align*}
in Table \ref{tab:Optimal-iteration-complexity}, taken from \cite{zhang2013linear}. 

\begin{table}
	\begin{centering}
		\begin{tabular}{|c|c|c|c|}
			\hline 
			& Lipschitz continuous & Smooth & Smooth\&Strongly Convex\tabularnewline
			\hline 
			\hline 
			Full Gradient & $O(\frac{1}{\epsilon^{2}})$ & $O(\frac{L}{\sqrt{\epsilon}})$ & $O(\sqrt{\kappa}\log\frac{1}{\epsilon})$\tabularnewline
			\hline 
			Stochastic Gradient & $O(\frac{1}{\epsilon^{2}})$ & $O(\frac{1}{\epsilon^{2}})$ & $O(\frac{1}{\lambda\epsilon})$\tabularnewline
			\hline 
		\end{tabular}
		\par\end{centering}
	\caption{\label{tab:Optimal-iteration-complexity}Optimal iteration complexity
		of convex optimization. $L$ and $\lambda$ are the moduli of smoothness
		and convexity, i.e. $\lambda\protect\leq\|\nabla_{\theta}^{2}f\|\protect\leq L$,
		and $\kappa=L/\lambda$ is the condition number. }
	
\end{table}

The iteration complexity in stochastic optimization is generally polynomial
in $\frac{1}{\epsilon}$. However, when $f$ is of the form 
\begin{align*}
f & =\frac{1}{n}\sum_{i=1}^{n}f_{i}+g_{\lambda}
\end{align*}
where $f_{i}$ are convex and $L$-smooth, while $g_{\lambda}$ is
$L$-smooth and $\lambda$-strongly convex, the complexity can be
improved to be logarithmic in $\frac{1}{\epsilon}$. For example,
the stochastic average gradient (SAG) method has iteration complexity
$O(n\log\frac{1}{\epsilon})$ provided $n\geq8\kappa$, the stochastic
dual coordinate ascent (SDCA) method (\cite{shalev2013stochastic})
has iteration complexity $O((n+\kappa)\log\frac{1}{\epsilon})$, and
the epoch mixed gradient descent (EMGD) method (\cite{zhang2013linear})
has the complexity $O((n+\kappa^{2})\log\frac{1}{\epsilon})$. Of
the three, EMGD can be applied to general strongly convex and smooth
functions, in which case it requires $O(\log\frac{1}{\epsilon})$
full gradient queries and $O(\kappa^{2}\log\frac{1}{\epsilon})$ stochastic
gradient queries. Table \ref{tab:complexity_stochastic} compares
these stochastic gradient algorithms with the accelerated gradient
descent of Nesterov applied to stochastic gradient descent. 

\begin{table}
	\begin{centering}
		\begin{tabular}{|c|c|c|c|}
			\hline 
			Nesterov & EMGD & SAG $(n\geq8\kappa)$ & SDCA\tabularnewline
			\hline 
			\hline 
			$O(\sqrt{\kappa}n\log\frac{1}{\epsilon})$ & $O((n+\kappa^{2})\log\frac{1}{\epsilon})$ & $O(n\log\frac{1}{\epsilon})$ & $O((n+\kappa)\log\frac{1}{\epsilon})$\tabularnewline
			\hline 
		\end{tabular}
		\par\end{centering}
	\caption{\label{tab:complexity_stochastic}Computational complexity of stochastic
		first order methods for minimizing $f=\frac{1}{n}\sum_{i=1}^{n}f_{i}+g_{\lambda}$. }
\end{table}

We note the distinction between the condition number of a function
and a matrix. For a function $f(\theta,X)$, where $X$ denotes data
and $\theta$ denotes parameter, the condition number is given by
$L/\lambda$ where 
\begin{align*}
\lambda\leq\|\nabla_{\theta}^{2}f(\theta,X)\| & \leq L
\end{align*}
for all $\theta\in\Theta$ the parameter space. When $f(\theta,X,Y)=\frac{1}{n}\|X\theta-Y\|_{2}^{2}$,
the Hessian is a fixed quantity, namely the Wishart matrix $X^{T}X$.
In general, the Hessian is parameterized by $\theta$ and $\lambda$
and $L$ are the upper and lower bounds of the largest and smallest
eigenvalues of the Hesisan, respectively. 

In this section, we are interested in how diagonal preconditioning
procedures on the design matrix affect the iteration complexity through
reducing the condition number of the objective function. 

\begin{comment}
In this section, we focus on how preconditioning procedures speed
up the convergence of first order methods in optimization. Note however
that preconditioning is important for second order methods as well,
but we defer the analysis to future work. By the data matrix, we mean
the input $x$ required to evaluate the full or stochastic gradients
of $f(x;w)$, where $w$ is the variable we are trying to minimize
$f$ over. 
\end{comment}


\subsection{Accelerating Optimization through Preconditioning}

To motivate the discussion, we first examine the least squares problem
\begin{align*}
\min_{\theta}\frac{1}{n}\|X\theta-Y\|_{2}^{2}
\end{align*}
where $X\in\mathbb{R}^{n\times p}$ which has smoothness and strong
convexity moduli of $\lambda_{1}(X^{T}X)$ and $\lambda_{n}(X^{T}X)$,
respectively. Here we assume that $n>p$, so that $X^{T}X$ is invertible
and hence the objective function is both smooth and strongly convex.
For the least squares problem, an analytic solution is available,
but we consider first order methods mainly because the quadratic form
makes the effect of preconditioning procedures obvious. We may also
imagine a setting where potentially $n,p$ are large so that direct
computation of $(X^{T}X)^{-1}$ is costly, so that we can only resort
to (stochastic) first order methods. In any case, given the least
squares problem, we are interested in how diagonal preconditioning
procedures speed up the convergence of first order methods. 

There are potentially two levels of stochasticity. The data matrix
is assumed to have i.i.d. rows from some distribution. Our earlier
results show that the condition number $\kappa(X^{T}X)$ of sub-Gaussian
data matrices concentrate around that of the population covariance
matrix $\Sigma$, and that for a class of population covariance matrices,
preconditioning with column standard deviation reduces the condition
number of the data matrix by a factor on the order of $\sqrt{\kappa(\text{diag}(\Sigma))}$
with high probability. So for full gradient methods, a reduction in
computational complexity is achieved through the reduction of the
condition number on the order of $\sqrt{\kappa(\text{diag}(\Sigma))}$
with high probability if we assume sub-Gaussian data distribution
with well-behaved covariance matrix $\Sigma$, or $\sqrt{\frac{\kappa(X^{T}X)}{\kappa(D^{-1}X^{T}XD^{-1})}}$
using optimal diagonal preconditioning methods developed in the previous
section, for the least squares problem. 

For general smooth and strongly convex objectives $f(\theta,X)$ the
condition number $\kappa(\nabla_{\theta}^{2}f(\theta,X))$ of the
Hessian of the objective function is not constant, but depends on
the current estimate $\theta^{k}$ of the parameter.\textbf{ }Here
there are two types of preconditioning that can be performed. The
first type is that done on the data matrix $X$, using a variety of
conditioning algorithms including the usual data normalization procedure,
batch normalization, or the optimal diagonal preconditioning algorithm
developed in this paper. It can be done on the entire $X$ once before
the optimization procedure, or for stochastic systems, on the sub
design matrix formed by the minibatch of samples. If we are using
first order methods, only the above preconditioning on the (sub)design
matrix is possible. If we can efficiently calculate or approximate
the inverse Hessian, then a second preconditioning option is to precondition
directly on the (approximate) Hessian or inverse Hessian, evaluated
at the current estimate $\theta^{k}$. As discussed earlier, Quasi-Newton
methods and other accelerated gradient methods such as Anderson mixing
(\cite{zhang2018globally}) and Adagrad (\cite{duchi2011adaptive}) rely
crucially on some form of approximate inverse Hessian or Jacobian.
When the approximate inverse Hessian is ill-conditioned, the methods
are known to slow down or diverge both in theory and in practice (\cite{shanno1970optimal}).
Preconditioning the approximate inverse Hessian has been considered
in as early as (\cite{shanno1970conditioning}). Here we simply note
that our optimal diagonal algorithm can also be applied to the quasi-Newton
update formulae to improve the condition number of the approximate
inverse Hessian. 

We focus on the case of preconditioning on the data/design matrix
$X$, and study how the reduction in $\kappa(X^{T}X)$ translates
into that of $\kappa_{f}$, where 
\begin{align*}
\kappa_{f} & =\frac{L_{f}}{\lambda_{f}}\\
L_{f} & =\sup_{\theta}\|\nabla_{\theta}^{2}f(X,\theta)\|\\
\lambda_{f} & =\inf_{\theta}\|\nabla_{\theta}^{2}f(X,\theta)\|
\end{align*}

In order to analyze how preconditioning of the data\textbf{ }matrix
affects the condition number of the Hessian at $\theta^{k}$, we need
to make assumptions about the structure of the objective function
$f$. For example, if $f$ is of the form $f_{0}(X\theta)$ for some
$f_{0}$ with condition number $\kappa_{0}$, then the Hessian of
the objective function satisfies 
\begin{align*}
\kappa(\nabla_{\theta}^{2}f) & =\kappa(X^{T}\cdot\nabla^{2}f_{0}(X\theta)\cdot X)
\end{align*}
and we should expect improvements on the condition number of $X^{T}X$
to improve the condition number of the Hessian as well. In the following
result, we focus on the case when $f$ corresponds to the (regularized)
loss of an empirical risk minimization problem (\cite{shalev2013stochastic}).
In this case, the reduction in $\kappa_{f}$ is on the order of $\sqrt{\kappa(X^{T}X)/\kappa(DX^{T}XD)}$
for smooth and strongly convex objectives. This reduction then implies
the corresponding improvements in iteration complexities of first
order methods, thorugh their dependences on $\kappa_{f}$. 

\begin{theorem}
\label{thm:cond_number_general}If $f(X,w)=\frac{1}{n}\sum_{i}f_{i}(w^{T}x_{i})$
for scalar $\lambda$-strongly convex and $L$-smooth functions $f_{i}$.
Then replacing $x_{i}$ with $Dx_{i}$, where $D$ is a diagonal matrix
such that $\kappa(DX^{T}XD)\leq\kappa(X^{T}X)$, we have

(i) For general $f_{i}(z)$,

\begin{align*}
\kappa(\nabla_{w}^{2}f(XD,w)) & \leq\frac{\kappa(\nabla_{w}^{2}f(X,w))}{\kappa(X^{T}X)/\kappa(DX^{T}XD)}\kappa_{0}^{2}
\end{align*}
where $\kappa_{0}=\frac{L}{\lambda}$, i.e. when $f_{i}$ are well-conditioned
so $\kappa_{0}$ is small, the reduction in condition number of the
objective function with preconditioning is on the order of $\kappa(X^{T}X)/\kappa(DX^{T}XD)$.

(ii) When $f_{i}(z)=z^{2}$, the result reduces to the special case
of linear regression, where the reduction in condition number is lower
bounded by exactly $\kappa(X^{T}X)/\kappa(DX^{T}XD)$.
\end{theorem}
\proof{Proof}
	We have 
	\begin{align*}
	\nabla_{w}^{2}f(X,w) & =\frac{1}{n}\sum_{i}\nabla^{2}f_{i}(w^{T}x_{i})x_{i}x_{i}^{T}
	\end{align*}
	Moreover,
	\begin{align*}
	\frac{1}{n}LX^{T}X\succeq\frac{1}{n}\sum_{i}\nabla^{2}f_{i}(w^{T}x_{i})x_{i}x_{i}^{T} & \succeq\frac{1}{n}\lambda X^{T}X
	\end{align*}
	so that 
	\begin{align*}
	\kappa(\nabla_{w}^{2}f(XD,w)) & \leq\kappa(DX^{T}XD)\cdot\kappa_{0}\\
	& =\frac{\kappa(DX^{T}XD)}{\kappa(X^{T}X)}\cdot\kappa(X^{T}X)\cdot\kappa_{0}\\
	& \leq\kappa_{0}^{2}\cdot\kappa(\nabla_{w}^{2}f(X,w))\cdot\frac{\kappa(DX^{T}XD)}{\kappa(X^{T}X)}
	\end{align*}
	\hfill \halmos
\endproof
The above result separates out the effect of the design matrix on
the condition number of the objective function. If the objective function
itself is smooth and strongly convex, then diagonal preconditioning
on a badly-conditioned design matrix results in a reduction of the
condition number of the objective function on the order of $\sqrt{\kappa(X^{T}X)/\kappa(DX^{T}XD)}$,
which then implies improvements on the complexities of first order
methods through their dependences on the condition number. 

\subsection{Adaptive Diagonal Preconditioning}

So far, we have focused on preconditioning with a fixed preconditioner
$D$ when we have acces to all the data at once in the form of the
design matrix, where $D$ is obtained from data matrix $X$, e.g.
column-wise standard deviation of $X$ or optimal diagonal preconditioning
obtained using methods discussed in the previous section. However,
in practice such a preconditioner may not be available. For example,
in stochastic gradient descent or online learning, we may not have
prior access to the full data matrix $X$, instead only drawing random
subsets of all samples. In such settings, it is still possible to
speed up the convergence with adaptive preconditioning procedures
applied to first order methods. In fact, many first order methods
can be understood to involve some form of adaptive preconditioning.
For example, BFGS method (\cite{broyden1970convergence,goldfarb1970family})
and AdaGrad (\cite{duchi2011adaptive}) pre-multiply the gradient with
some approximate (diagonal) inverse Hessian. Other adaptive gradient
methods that perform local optimization with an adaptive metric constructed
from observed iterates have become increasingly popular in deep learning
with benefits to the convergence speed as well as statistical properties
of the iterative optimization procedures. For example, \cite{levy2019necessary} show that when the ``scale'' of the gradients
varies across dimensions, adaptive gradient methods such as AdaGrad
(\cite{duchi2011adaptive}) achieves lower regret compared to vanilla
stochastic gradient methods. 

A popular normalization technique used in deep learning, called batch
normalization (\cite{ioffe2015batch}), can also be understood as a
form of adaptive (diagonal) conditioning. 

For general neural networks, let $x^{(m,k)}\in\mathbb{R}^{n\times p_{m}}$
denote the output of the $m$-th layer, consisting of $n$ $p_{m}$-dimensional
vectors, at the $k$th iteration of stochastic gradient descent. Batch
normalization involves applying a centering operation and a scaling
operation to $x^{(m,k)}$, followed by reverse operations with parameters
$\gamma\in\mathbb{R}_{++}^{p_{m}},\beta\in\mathbb{R}^{p_{m}}$, to
obtain 
\begin{align*}
\tilde{x}_{i}^{(m,k)} & =\frac{(x_{i}^{(m,k)}-\mu_{i})}{\sigma_{i}}\cdot\gamma_{i}+\beta_{i}
\end{align*}
for the $i$th column of $x^{(m,k)}$, where $\mu_{i}$ is the mean
of the $i$th column, and $\sigma_{i}$ is the standard deviation.
The parameters $\gamma,\beta$ are updated through SGD together with
the original parameters of the neural network. The point is that population
statistics for intermediate layers are not known a priori, so $\gamma$
and $\beta$ serve as adaptive parameters that are updated at each
step of the training. 

Specialized to the least squares problem, it effectively solves the
problem $\min_{\theta,D}\frac{1}{n}\|XD\theta-y\|_{2}^{2}$ by alternating
between $\theta$ and $D$ during each iteration, i.e. at the $k$th
iteration, given $D^{(k)}$, one solves the problem $\min_{\theta}\frac{1}{n}\|XD^{(k)}\theta-y\|_{2}^{2}$
and then find $D_{1}^{(k+1)}$ by solving $\min_{D}\frac{1}{n}\|XD\theta^{(k+1)}-y\|_{2}^{2}$.

This alternating optimization procedure is present in many other convex
optimization problems with special structures, for example the ADMM
method for minimizing the sum of convex functions with block variables
(\cite{lin2015global,wen2010alternating}). It is also used in non-convex
formulations of convex problems, most notably low-rank matrix and
tensor factorization \cite{chi2019nonconvex,aswani2016low,zhao2015nonconvex},
where alternating minimization of the objective is employed to solve
a non-convex formulation of the problem. Besides convergence issues,
another recent focus of the latter literature is on the ``implicit
regularization'' (\cite{wu2019implicit}) of the alternating minimization
algorithm associated with the non-convex formulation. 

It is similarly possible to extend our optimal diagonal preconditioning
procedure to the stochastic setting. Suppose each iteration we observe
subsets of rows of a design matrix $X$. At each iteration we update
our estimate of $X^{T}X$ based on samples drawn from $X$ so far.
Then we can compute the optimal diagonal preconditioner $D$ based
on the current estimate of $X^{T}X$. As the number of iterations
increases, our estimate of $X^{T}X$ becomes more accurate, and $D$
should approach the appropriate optimal diagonal preconditioner given
$X^{T}X$. This gives the following algorithm. 

\begin{comment}
More generally, at each iteration, $D$ can be calculated based on
other heuristics depending on $X$ and current parameter estimates.
The popular batch normalization procedure can be understood as an
instance of this adaptive preconditioning. Other adaptive gradient
methods that perform local optimization with an adaptive metric constructed
from observed iterates have become increasingly popular in deep learning.
\cite{levy2019necessary} show that when the ``scale''
of the gradients varies across dimensions, adaptive gradient methods
such as AdaGrad \cite{duchi2011adaptive} achieves lower regret compared
to vanilla stochastic gradient methods. 
\end{comment}

\begin{algorithm}
	(Adaptive optimal diagonal preconditioning) Let $\overline{X}^{(0)}=[]$
	and at the $k$th iteration, form the cumulative design matrix $\overline{X}^{(k)}$
	by concatenating the $k$-th batch $X^{(k)}$ with $\overline{X}^{(k-1)}$
	and retaining unique rows. If $\overline{X}^{(k)}$ is full rank,
	then find $D_{1}^{(k)}$ that minimizes $\kappa(D(\overline{X}^{(k)T}\overline{X}^{(k)}D)$
	and perform the preconditioning$X^{(k)}D_{1}^{(k)}$. Alternatively,
	we can perform the optimal diagonal scaling every $m$ iterations,
	where $m$ is chosen to balance the tradeoff between computational
	cost and convergence speed. 
\end{algorithm}

A natural next step is to compare the performance of the optimal diagonal
preconditioning with that of batch normalization on regression and
classification problems. We take up this in the next section. We also
note that although batch normalization speeds up the convergence of
first order methods and can be viewed as a form of adaptive diagonal
preconditioning, it is not the case that the effective condition numbers
of Hessian matrices under batch normalization are reduced, since the
diagonal conditioner is selected so as to minimze the objective loss
rather than the condition number of the preconditioned matrix. This
is in contrast to our adaptive optimal preconditioning algorithm,
which speeds up convergence by reducing the effective condition number
of the design matrix. Thus it remains to further investigate the mechanism
through which batch normalization speeds up the convergence of first
order methods. 

We also mention that other adaptive methods, such adaptive regularization
of objective (\cite{jiang2017unified}) and adaptive step size \cite{gao2019quasi},
are also effective in speeding up the convergence of first order methods.
These methods are often applied to quasi-Newton methods and the step
size is determined based on information on the local curvature of
the objective function, e.g. the damped Newton method \cite{nesterov2013introductory}
of Nesterov, who derived convergence results for self-concordant functions
\cite{nesterov1994interior}. As a possible extension of the optimal
preconditioning framework, it may be interesting to consider using
an approximate optimal preconditioner of the approximate inverse Hessian,
and to explore potential connections with adaptive step size approaches
for self-concordant functions. 

==> theory-old-2.tex <==
\section{Problem Setup and Algorithms}
\label{sec:optimal}

In this section, we turn to the two-sided optimal diagonal preconditioning
problem. For a matrix $A\in\mathbb{R}^{m\times n}$ with full rank, we want to find positive \emph{diagonal} matrices $D_1,D_2$ that solve the following minimization problem (the particular choice of exponents for $D_1,D_2$ will become clear shortly):
\begin{align}
\label{eq:two-sided-problem}
\min_{D_{1},D_{2}\succ0}\kappa(D_{1}^{1/2}AD_{2}^{-1/2})
\end{align}
There are two related \emph{one-sided} optimal diagonal preconditioning problems that seek diagonal matrices $D_1$ and $D_2$ which solve the following two distinct problems, respectively:
\begin{align}
\label{eq:left-sided-problem}
\min_{D_{1}\succ0}&\kappa(D_{1}^{1/2}A)\\
\label{eq:right-sided-problem}
\min_{D_{2}\succ0}&\kappa(AD_{2}^{-1/2})
\end{align}
 Note first that without loss of generality, we can always assume $m\geq n$, so that $A$ is a \emph{tall} matrix, since otherwise we may take the transpose of $A$ without changing the optimal solution pairs to the two-sided problem \eqref{eq:two-sided-problem}. For the one-sided problems \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem}, taking the transpose of $A$ essentially transforms one problem to the other. Moreover, for square matrices,
i.e., $m=n$, the three optimal preconditioning procedures essentially
yield the same optimal diagonal preconditioners, since similar square matrices
have the same eigenvalues hence the same condition numbers. Finally, note that solutions are scale-invariant, since for any optimal
pair $(D_{1},D_{2})$ of diagonal preconditioners that achieves the
minimum objective value of \eqref{eq:two-sided-problem}, $(c_1D_{1},c_2D_{2})$ for any $c_1,c_2>0$ is also
a pair of optimal diagonal preconditioners, and similarly for \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem}. For the purpose of reducing condition numbers, any optimal solution is sufficient.

%For now, we will primarily focus on developing algorithms for the two-sided problem \eqref{eq:two-sided-problem}. 
\textbf{Overview.} We will develop a baseline algorithm based on bisection that solves the two-sided problem \eqref{eq:two-sided-problem} in this section, and then develop a polynomial time interior point algorithm in Section \ref{sec:potential-reduction}. %The corresponding algorithms and theory for the one-sided problems \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem} can be obtained with straightforward reductions. 
In Section \ref{sec:DSDP}, we show that \eqref{eq:left-sided-problem} and \eqref{eq:right-sided-problem} admit reformulations as standard dual SDP problems,
to which customized solvers can be applied to obtain solutions efficiently for large matrices. We will then develop specialized algorithms for the one-sided problems based on this reformulation.
%In contrast, the two-sided problem \eqref{eq:two-sided-problem} does not admit an SDP reformulation. 
In Section \ref{sec:experiments}, we will compare the empirical performance
of these optimal preconditioning procedures. In general, one-sided optimal diagonal preconditioners are sufficient to achieve significant reductions in condition numbers, although there are instances where two-sided preconditioners are essential. In practice, we can handle large one-sided problems ($m \approx 5000$) thanks to the customized solver. %In particular, we will investigate
%when and how two-sided optimal preconditioning improves upon the
%two one-sided preconditioners significantly in
%terms of condition number reduction, as well as when the two one-sided
%methods differ from each other.

\subsection{Problem Reformulation}
 We start by rewriting the two-sided optimal diagonal preconditioning problem \eqref{eq:two-sided-problem} in a more accessible form. First, note that for any matrix $A \in \mathbb{R}^{m\times n}$ with full rank and $m\geq n$, $\kappa(A)=\sqrt{\kappa(A^{T}A)}$, so we can instead minimize the condition
number of $(D_{1}^{1/2}AD_{2}^{-1/2})^{T}(D_{1}^{1/2}AD_{2}^{-1/2})=D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2}$.
As the condition number is scale-invariant, we can introduce a new
positive \emph{variable} $\kappa$ (to be distinguished from the condition
number $\kappa(M)$ of a matrix) and rewrite the resulting problem
as
\begin{align*}
\min_{\kappa,D_{1},D_{2}\succ0}\kappa\\
I_n\preceq D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2}\preceq\kappa I_n
\end{align*}
The objective above achieves its minimum value $\kappa^\ast=(\min_{D_{1},D_{2}\succ0}\kappa(D_{1}^{1/2}AD_{2}^{-1/2}))^{2}$, and at any optimal solution $(D_1,D_2)$, $\lambda_{\min}(D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2})=1$ and $\lambda_{\max}(D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2})=\kappa^\ast$.

Next, the constraint $I_n\preceq D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2}\preceq\kappa I_n$
is equivalent to $D_{2}\preceq A^{T}D_{1}A\preceq\kappa D_{2}$, and, with diagonal matrices $D_1,D_2$, we can rewrite the problem in its final reformulation as
\begin{align}
\label{eq:SDP-two-sided}
\begin{split}
    \min_{\kappa\geq0} \kappa \\
A^{T}D_{1}A\succeq D_{2}\\
\kappa D_{2}\succeq A^{T}D_{1}A \\
D_1 \succeq I_m 
\end{split}
\end{align}
where we have replaced the strict inequalities $D_1,D_2\succ0$ by equivalently requiring $\kappa \geq 0$ and $D_1 \succeq I_m$. Since $A^TD_1A\succeq A^TA\succ 0$, $D_2$ and $\kappa$ in fact need to be both strictly positive. Note that the alternative constraint $D_2 \succeq I_n$ instead of $D_1 \succeq I_m$ does not work, however, since $m\geq n$ and $D_1$ could still have zero diagonal entries even if $D_2 \succ 0$.
The problem \eqref{eq:SDP-two-sided} is also scale-invariant, and we may further impose normalization constraints to make the solution unique. This is not necessary for the purpose of the baseline algorithm we develop in this section. For the interior point algorithm we develop in Section \ref{sec:potential-reduction}, we will impose an upper bound on $D_1$ to facilitate the definition of a potential function which we will aim to reduce. 
%However, as we will see, the interior point algorithm we develop based on potential reduction will find the unique solution with $\lambda_{\min}(D_1)=1$, so we do not need to explicitly impose the normalization constraint. 

Note that the problem in \eqref{eq:SDP-two-sided} is a quasi-convex problem. To see this more clearly, let $d_1\in\mathbb{R}^m,d_2\in\mathbb{R}^n$ be the vector representations of the diagonal matrices $D_1,D_2$, and moreover $d_3=\kappa d_2$. With $d_{1i}$ denoting the $i$-th element of $d_1$, and $d_{2j}$ the $j$-th element of $d_2$, the problem can be written as
\begin{align*}
\min_{\kappa,d_1,d_2,d_3\geq0} \sum_{j=1}^n d_{3j}/d_{2j}\\
\sum_{i=1}^{m} d_{1i} a_i a_i^T - \sum_{j=1}^n d_{2j} e_j e_j^T   \succeq 0\\
\sum_{j=1}^n d_{3j} e_j e_j^T -\sum_{i=1}^{m} d_{1i} a_i a_i^T\succeq 0\\
d_1 - \mathbf{1}_m \geq 0
\end{align*}
where vector $a_i$ is the $i$-th row of $A$ and $e_j \in \mathbb{R}^n$ is the vector whose $j$-th entry is 1 and zero otherwise. However, \eqref{eq:SDP-two-sided} is not equivalent to a standard SDP, because of the product term $\kappa D_2$.

\subsection{A Bisection Algorithm for Optimal Diagonal Preconditioning}
We start with a simple baseline algorithm for the two-sided optimal preconditioning problem \eqref{eq:SDP-two-sided} using bisection. This algorithm is easy to implement in practice, although it may be slow for larger problems. In Section \ref{sec:potential-reduction}, we will introduce an interior point algorithm with polynomial complexity, and comparison with the baseline algorithm will facilitate in understanding its improvements.

Our bisection algorithm consists of the following three steps:
\begin{enumerate}
\item Start with some large $\kappa_{0}\geq1$ such that the SDP feasibility
problem 
\begin{align*}
\min_{D_1,D_2} 0\\
A^{T}D_{1}A\succeq D_{2}\\
\kappa_{0}D_{2}\succeq A^{T}D_{1}A\\
D_1 \succeq I_m
\end{align*}
 has a solution. A choice that always works is $\kappa_{0}=\kappa(A^{T}A)$.
If we have prior information that there exists some $D_{1},D_{2}$
such that one of $\kappa(A^{T}D_{1}A)$, $\kappa(D_{2}^{-1/2}A^{T}AD_{2}^{-1/2})$,
or $\kappa(D_{2}^{-1/2}A^{T}D_{1}AD_{2}^{-1/2})$ is smaller than
$\kappa(A^{T}A)$, we can set $\kappa_{0}$ to that number as a warm
start. Popular candidates for such $D_{1},D_{2}$ could be based on
the diagonals or row/column standard deviations of $A$, or other
matrix scaling techniques such as matrix equilibriation \citep{takapoui2016preconditioning} and Ruiz scalings \citep{ruiz2001scaling}.
Set the upper bound $\overline{\kappa}=\kappa_{0}$ and lower bound
$\underline{\kappa}=1$.
\item Solve the SDP feasibility problem 
\begin{align*}
\min_{D_{1},D_{2}}0\\
A^{T}D_{1}A\succeq D_{2}\\
\frac{\overline{\kappa}+\underline{\kappa}}{2}D_{2}\succeq A^{T}D_{1}A\\
D_1 \succeq I_m
\end{align*}
If the problem is feasible, set $\frac{\overline{\kappa}+\underline{\kappa}}{2}$
to be the new \emph{upper} bound $\overline{\kappa}$. If the problem
is infeasible, set $\frac{\overline{\kappa}+\underline{\kappa}}{2}$
to be new \emph{lower} bound $\underline{\kappa}$.
\item Solve the SDP feasibility problems iteratively while updating the
upper and lower bounds, until $\overline{\kappa}-\underline{\kappa}<\epsilon$
for some tolerance parameter $\epsilon$. The final set of feasible
solutions $D_{1},D_{2}$ will provide an $\epsilon$-optimal two-sided
preconditioning.
\end{enumerate}

The algorithm can be improved via intelligent choices of the updates to lower and upper bounds by exploiting the quasi-convexity structure.
There is also a geometric interpretation of each feasibility problem
with a fixed parameter $\kappa$: it looks for $D_{1},D_{2}$ such
that the ellipsoid defined by $D_{2}$, with axes of symmetry the
coordinate axes, is inscribed in the ellipsoid defined by $A^{T}D_{1}A$,
and such that expanding $D_{2}$ by a factor of $\kappa$ will encapsulate
the ellipsoid defined by $A^{T}D_{1}A$. Such inscribing and containing
ellipsoids have been used in the ellipsoid method, where the ellipsoids
are not constrained to be symmetric along coordinate axes. The geometric
interpretation also makes it clear that the optimal value $\kappa^{\ast}\geq1$
is achieved in the optimization problem. Also compare with the approach
in \cite{jambulapati2020fast}, which develop constant-factor optimal algorithms based on structured
mixed packing and covering semidefinite programs.

Note that the bisection algorithm finds an $\epsilon$-optimal solution
in $O(\log\frac{1}{\epsilon})$ iterations, where each iteration requires
solving an SDP feasibility problem. In practice, the bisection algorithm usually converges in less than 10 updates with $\epsilon = 0.01$ on most test cases of moderate size from the datasets considered in this paper (see Section \ref{sec:experiments}). 

\subsection{An Interior Point Algorithm for Optimal Diagonal Preconditioning}
\label{sec:potential-reduction}
Although the baseline algorithm introduced above is easy to implement, it suffers from sub-optimal complexity in theory and limited problem size in practice. In this section, we focus
on developing an interior point method that finds an $\epsilon$-optimal
solution in $O(\log\frac{1}{\epsilon})$ iterations, where each
iteration only consists of a Newton update step. This enjoys better
complexity than the baseline algorithm based on bisection, which requires solving an SDP feasibility problem at each iteration. Our algorithm draws inspirations from interior point
methods for linear programming and semidefinite programming 
\citep{mizuno1992new,ye1992potential,ye1995neumann,nesterov1997self},
particularly \cite{nesterov1997self}
on directions of Newton updates in interior point methods for SDPs and \cite{ye1995neumann}
on the ``Von Neumann economic growth problem'' \citep{von1937uber,neumann1945model}. 
%Add a remark on the connection to the Von Neumann problem of the right preconditioning problem.

Recall the reformulated two-sided optimal diagonal preconditioning problem in \eqref{eq:SDP-two-sided}. For ease of exposition, we present the algorithm and theory for the following right preconditioning problem by setting $D_1=I_m$ in \eqref{eq:SDP-two-sided}: %Extension to the two-sided problem can be found in the appendix.
\begin{align*}
\min_{\kappa\geq0}\kappa\\
A^{T}A\succeq D\\
\kappa D\succeq A^{T}A
\end{align*}
Let $\kappa^{\ast}\in[1,\infty)$ be optimal objective value of the above problem. Following \cite{ye1995neumann}, with $M=A^TA$, we define the \textbf{potential function} on $(\kappa^\ast,\infty)$
as
\begin{align*}
P(\kappa) & :=\sum_{i}\log\lambda_{i}(M-D^{\kappa})+\sum_{i}\log\lambda_{i}(\kappa D^{\kappa}-M)+\sum_{i}\log D_{ii}^{\kappa}
\end{align*}
where $D^{\kappa}$ is the \textbf{analytic center} of the feasible
region \textbf{
	\begin{align*}
	\Gamma(\kappa) & =\{D\succeq0:D\text{ diagonal};M\succeq D;\kappa D\succeq M\}
	\end{align*}
} which is simply the unique maximizer of the strictly concave problem
\begin{align*}
\max_{D\succeq0\text{ diagonal}} & \sum_{i}\log\lambda_{i}(M-D)+\sum_{i}\log\lambda_{i}(\kappa D-M)+\sum_{i}\log D_{ii}\\
& \Longleftrightarrow\\
\max_{D\succeq0\text{ diagonal}} & \log\det(M-D)+\log\det(\kappa D-M)+\log\det D
\end{align*}

See also \cite{mizuno1993adaptive,luo1998superlinear,sturm1999symmetric}
for the use of analytic centers in path-following and potential reduction
interior point algorithms for LP and SDP problems. 

The geometric interpretation of the problem makes it clear that if
the feasible region $\Gamma(\kappa^{0})$ has a non-empty interior
for some $\kappa^{0}<\infty$, then the feasible region $\Gamma(\kappa)$
has a non-empty interior for all $\kappa\geq\kappa^{0}$, so that
the analytic center is well defined. At the optimal objective value
$\kappa^{\ast}\geq1$, however, the solution set has no interior because
it must be the case that $\lambda_{n}(\kappa D-M)=0$ for any $D$
in the solution set, where $\lambda_{1}\geq\lambda_{2}\geq\cdots\geq\lambda_{n}$
are the eigenvalues of a matrix, and so perturbing $D$ in some direction
by any amount will violate the constraint $M\succeq D$. 
\begin{lemma}
	For $M\succ0,$ the feasible set of the feasibility problem 
	\begin{align*}
	\min_{D\succeq0}0\\
	M\succeq D\\
	\kappa D\succeq M
	\end{align*}
	has bounded non-empty interior for any $\kappa>\kappa^{\ast}$.
\end{lemma}
Next, we show that the potential function is monotonic in $\kappa$,
and that it is bounded away from $P(\kappa^{\ast})$, for any $\kappa$
large. This implies that $P(\kappa)$ is a reasonable measure of the progress of an algorithm:
to obtain an approximate optimal solution to the optimal preconditioning problem, it suffices to reduce the potential function by a constant
amount at every step and terminate when the potential function is
reduced below a certain threshold determined by accuracy $\epsilon$. This is summarized in the following two results. All proofs in this section can be found in the appendix.
\begin{proposition}\label{prop:monotonicity}
	If $\kappa_{0}>\kappa_{1}>\kappa^{\ast}$, then $P(\kappa_{0})>P(\kappa_{1})$. 
\end{proposition}
%
\begin{proposition}\label{prop:lower bound}
	Let $t$ satisfy $\kappa^{\ast}\leq2^{t}$, then for any $\overline{\kappa}>\kappa^{\ast}+2^{-t}$,
	we have
	\begin{align*}
	P(\overline{\kappa}) & >-Cnt
	\end{align*}
	for some universal constant that only depends on $M$. 
\end{proposition}
These two results imply that if $P(\kappa)<O(-nt)$, then we must
have $\kappa\leq\kappa^{\ast}+2^{-t}$. Therefore, if we can find a
$D$ whose associated potential is below the threshold of $O(n\log\epsilon)$,
we have found an approximate solution that yields a condition number
that is within $\epsilon$ of the optimal condition number. Our goal
is then to design an algorithm that achieves constant reduction of
the potential at every iteration, which would guarantee an iteration
complexity of $O(\log\frac{1}{\epsilon})$. 

In the next two subsections, we develop potential reduction algorithms based on this idea, using exact and approximate analytic centers, respetively. Before doing so, we show that the analytic center satisfies an equality condition that is useful in the analysis of the reduction of the potential function. It is essentially the first order condition of the convex optimziation problem. Since it also serves an important role in the Newton step, we state it in a particular form in the next lemma. 
\begin{lemma}
	The analytic center $D$ of the feasible region $\Gamma(\kappa)$
	satisfies 
	\begin{align*}
	Z+\kappa Y & =X
	\end{align*}
	where with $R:=M-D$, $S:=\kappa D-M$,  \begin{align*}
	X&=R^{-1},Y=S^{-1},Z=D^{-1}
	\end{align*}
\end{lemma}

\subsection{Analysis of Potential Reduction with Exact Analytic Centers}

Let $D^{0},D^{1}$ be the analytic centers of $\Gamma^{0}=\Gamma(\kappa^{0})$
and $\Gamma^{1}=\Gamma(\kappa^{1})$ for $\kappa^0,\kappa^1>\kappa^\ast$. With a suitable choice of $\Delta\kappa=\kappa^{0}-\kappa^{1}>0$,
we show that the analytic centers $D^{0}$ and $D^{1}$ are close,
and that 
\begin{align*}
P(\kappa^{1}) & \leq P(\kappa^{0})-\Omega(1)
\end{align*}
so that we can achieve constant reductions of the potential function
by updating from $D^{0}$ to $D^{1}$. To obtain $D^{1}$ from $D^{0}$,
we can use Newton iterations with a quadratic
convergence rate. The exact form of the Newton iteration is deferred
to the next subsection, where we propose a practical potential algorithm
using approximate analytic centers and only one Newton step.
%
\begin{theorem}
	\label{thm:exact center}Let $\overline{\kappa}$ be an upper bound of $\kappa^{\ast}$. Let $D^{0}$ and $D^{1}$ be the analytic centers of $\Gamma^{0}=\Gamma(\kappa^{0})$
	and $\Gamma^{1}=\Gamma(\kappa^{1})$ for $\kappa^{0},\kappa^{1}\in(\kappa^{\ast},\overline{\kappa})$.
	If $\Delta\kappa=\kappa^{0}-\kappa^{1}>0$ satisfies
	\begin{align*}
	\Delta\kappa & =\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}\\
	& =\frac{\beta}{e^{T}D^{0}\text{diag}((\kappa^{0}D^{0}-M)^{-1})e}
	\end{align*}
	for some sufficiently small $\beta\in(0,1)$ that only depends on
	$\overline{\kappa},M$, then 
	\begin{align*}
	\sqrt{Tr((D^{1})^{1/2}(D^{0})^{-1}(D^{1})^{1/2}-I)^{2}} & \leq c\cdot\beta\\
	\sqrt{Tr((D^{0})^{1/2}(D^{1})^{-1}(D^{0})^{1/2}-I)^{2}} & \leq c\cdot\beta
	\end{align*}
	for some constant $c$,
	and	$P(\kappa^{1}) \leq P(\kappa^{0})-\beta$.
	
\end{theorem}

%We have thus obtained a conceptual algorithm, which uses the exact
%analytic center, summarized in Algorithm \ref{alg:exact}.
\begin{algorithm}[Potential Reduction with Exact Analytic Center]
	\label{alg:exact}
\begin{enumerate}
	\normalfont 
	    \item Let $D^{0}$ be analytic center of $\Gamma(\kappa^{0})$ with some
	$\kappa^{0}>\kappa^{\ast}$. Set $k=0$. 
	
	\item  With a small fixed constant $0<\beta<1$, set 
	\begin{align*}
	\Delta\kappa^{k} & =\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})},
	\end{align*}
and let $\kappa^{k+1}=\kappa^{k}-\Delta\kappa^{k}$.
	Then use Newton's method with updates of the form in Proposition \ref{prop:Newton step} to generate
	the exact analytic center $D^{k+1}$ of $\Gamma(\kappa^{k+1})$. 
	
	\item If $P(\kappa^{k+1})>O(-nt)$, set $k\leftarrow k+1$ and return
	to Step 1.
	\end{enumerate}
\end{algorithm}

\subsection{Algorithm with Approximate Analytic Center}

Given step size $\Delta\kappa$, in order to apply the potential reduction
algorithm, we still need to find the new analytic center $D^{1}$
corresponding to $\kappa^{0}-\Delta\kappa$. This can be achieved
using Newton iterations. However, it is not necessary to use exact
analytic centers. Instead, we can use an approximate analytic center
obtained from only one Newton update step, and show that the potential function
still reduces by a constant amount. Moreover, if we start from an approximate
analytic center, one Newton step with an appropriate step size $\Delta\kappa$
yields an approximate center that still achieves this constant reduction
in potential. We develop these results in this subsection. 

By an approximate analytic center, we mean a set of variables $(R,S,D,X,Y,Z)$
that satisfy the optimality conditions 
\begin{align*}
R & =M-D\succeq0\\
S & =\kappa D-M\succeq0\\
D & \succeq0\\
Z+\kappa Y & =X,
\end{align*}
but instead of requiring $RX=SY=DZ=I$ as is true for the exact analytic
center, we allow the products to be close to the identity $I$, where we use the following measure of proximity:
\begin{align*}
\delta(A,B) & :=\sqrt{Tr(B^{1/2}AB^{1/2}-I)^{2}}\\
& =\|B^{1/2}AB^{1/2}-I\|_{F}=\|A^{1/2}BA^{1/2}-I\|_{F}
\end{align*}
The second equality above follows from the fact that the Frobenius norm
is a spectral property for symmetric matrices. We may also check that
\begin{align*}
\delta(A,B) & =\sqrt{Tr((AB-I)^{2})}=\sqrt{Tr((BA-I)^{2})}
\end{align*}
As we will see in the following results, this is the appropriate measure
of proximity. The first result we show is that starting from an exact analytic
center for $\Gamma(\kappa^{0})$, we can obtain a feasible point in
$\Gamma(\kappa^{1})$ that is an $O(\beta)$ approximate analytic center.
\begin{proposition}
	\label{prop:initial}
	Let $D^{0}$ be the exact analytic center of $\kappa^{0}$. Define
	$R_{0}=M-D_{0}$, $S_{0}=\kappa_{0}D_{0}-M$ and $X_{0}=R_{0}^{-1},Y_{0}=S_{0}^{-1},Z_{0}=D_{0}^{-1}$.	Further, let $\Delta\kappa=\kappa^{0}-\kappa^{1}$ with $\Delta\kappa=\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}$
	where $\beta\in(0,1)$ is a sufficiently small constant, and 
	\begin{align*}
	\overline{R}^{0} & =R^{0},\overline{S}^{0}=-\Delta\kappa D^{0}+S^{0},\overline{D}^{0}=D^{0}\\
	\overline{X}^{0} & =X^{0},\overline{Y}^{0}=Y^{0},\overline{Z}^{0}=\Delta\kappa Y^{0}+Z^{0}
	\end{align*}
	Then, the new variables satisfy 
	\begin{align*}
	\overline{R}^{0} & =M-\overline{D}^{0}\succeq0\\
	\overline{S}^{0} & =\kappa^{1}\overline{D}^{0}-M\succeq0\\
	\overline{D}^{0} & \succeq0
	\end{align*}
	and $\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0}=\overline{X}^{0}$.
	Moreover, $\delta(\overline{S}^{0},\overline{Y}^{0})\leq\beta,\delta(\overline{D}^{0},\overline{Z}^{0})\leq\beta,\delta(\overline{R}^{0},\overline{X}^{0})=0$.
\end{proposition}
Next we show that this set of variables $(\overline{R}^{0},\overline{S}^{0},\overline{D}^{0},\overline{X}^{0},\overline{Y}^{0},\overline{Z}^{0})$
can be used as an initial set to generate a new $ O(\beta^{2}) $ approximate center
for $\kappa^{1}$, using a Newton step. This also implies that starting from an approximate analytic center we can obtain an exact analytic center by applying the Newton iterations with quadratic convergence. Here to ensure the symmetry
of updates in the Newton step, we use the Nesterov-Todd direction
\citep{todd1998nesterov,nesterov1997self}. 

\begin{proposition}
   \label{prop:Newton step}
   Let $(\overline{R}^{0},\overline{S}^{0},\overline{D}^{0},\overline{X}^{0},\overline{Y}^{0},\overline{Z}^{0})$
	be any set that satisfy 
	\begin{align*}
	\overline{R}^{0} & =M-\overline{D}^{0}\succeq0\\
	\overline{S}^{0} & =\kappa^{1}\overline{D}^{0}-M\succeq0\\
	\overline{D}^{0} & \succeq0
	\end{align*}
	and $\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0}=\overline{X}^{0}$,
	with 
	\begin{align*}
	\delta(\overline{R}^{0},\overline{X}^{0})=\|(\overline{R}^{0})^{\frac{1}{2}}\overline{X}^{0}(\overline{R}^{0})^{\frac{1}{2}}-I\|_{F} & \leq\beta\\
	\delta(\overline{D}^{0},\overline{Z}^{0})=\|(\overline{D}^{0})^{\frac{1}{2}}\overline{Z}^{0}(\overline{D}^{0})^{\frac{1}{2}}-I\|_{F} & \leq\beta\\
	\delta(\overline{S}^{0},\overline{Y}^{0})=\|(\overline{S}^{0})^{\frac{1}{2}}\overline{Y}^{0}(\overline{S}^{0})^{\frac{1}{2}}-I\|_{F} & \leq\beta
	\end{align*}
	for some $\beta\in(0,1)$.	Let $X^{1},Y^{1},Z^{1},R^{1},S^{1},D^{1}$ be defined by 
	\begin{align*}
	X^{1} & =\overline{X}^{0}+\Delta X,Y^{1}=\overline{Y}^{0}+\Delta Y,Z^{1}=\overline{Z}^{0}+\Delta Z\\
	R^{1} & =\overline{R}^{0}+\Delta R,S^{1}=\overline{S}^{0}+\Delta S,D^{1}=\overline{D}^{0}+\Delta D
	\end{align*}
	where the increments $\Delta$s are given by the Newton step %
	\begin{comment}
	The Newton step is to ensure 
	\begin{align*}
	\overline{R}^{0} & =M-\overline{D}^{0}\succeq0\\
	\overline{S}^{0} & =\kappa^{1}\overline{D}^{0}-M\succeq0\\
	\overline{D}^{0} & \succeq0
	\end{align*}
	and 
	\begin{align*}
	\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0} & =\overline{X}^{0}
	\end{align*}
	still holds. 
	
	Regular Newton step is
	
	\begin{align*}
	\overline{D}^{0}\cdot\Delta Z+\overline{Z}^{0}\cdot\Delta D & =I-\overline{D}^{0}\cdot\overline{Z}^{0}\\
	\overline{R}^{0}\cdot\Delta X+\overline{X}^{0}\cdot\Delta R & =I-\overline{R}^{0}\cdot\overline{X}^{0}\\
	\overline{S}^{0}\cdot\Delta Y+\overline{Y}^{0}\cdot\Delta S & =I-\overline{S}^{0}\cdot\overline{Y}^{0}
	\end{align*}
	but here we need to use the Nesterov-Todd direction to ensure symmetry
	of updates. 
	\end{comment}
	\begin{align*}
	\Delta Z+W^{-1}\Delta DW^{-1} & =(\overline{D}^{0})^{-1}-\overline{Z}^{0}\\
	\Delta X+U^{-1}\Delta RU^{-1} & =(\overline{R}^{0})^{-1}-\overline{X}^{0}\\
	\Delta Y+V^{-1}\Delta S & V^{-1}=(\overline{S}^{0})^{-1}-\overline{Y}^{0}
	\end{align*}
	{} and 
	$\Delta R  =-\Delta D,\Delta S=\kappa^{1}\Delta D,\Delta X=\Delta Z+\kappa^{1}\Delta Y$,
	where $U,V,W$ are the geometric means 
	\begin{align*}
	U & =(\overline{R}^{0})^{1/2}((\overline{R}^{0})^{1/2}\overline{X}^{0}(\overline{R}^{0})^{1/2})^{-1/2}(\overline{R}^{0})^{1/2}\\
	V & =(\overline{S}^{0})^{1/2}((\overline{S}^{0})^{1/2}\overline{Y}^{0}(\overline{S}^{0})^{1/2})^{-1/2}(\overline{S}^{0})^{1/2}\\
	W & =(\overline{D}^{0})^{1/2}((\overline{D}^{0})^{1/2}\overline{Z}^{0}(\overline{D}^{0})^{1/2})^{-1/2}(\overline{D}^{0})^{1/2}
	\end{align*}
	to ensure that updates are symmetric. Then we have 
	\begin{align*}
	\delta(R^{1},X^{1})=\|(R^{1})^{\frac{1}{2}}X^{1}(R^{1})^{\frac{1}{2}}-I\|_{F} & \leq\frac{1}{2}\frac{\beta^{2}}{1-\beta}\\
	\delta(S^{1},Y^{1})=\|(S^{1})^{\frac{1}{2}}Y^{1}(S^{1})^{\frac{1}{2}}-I\|_{F} & \leq\frac{1}{2}\frac{\beta^{2}}{1-\beta}\\
	\delta(D^{1},Z^{1})=\|(D^{1})^{\frac{1}{2}}Z^{1}(D^{1})^{\frac{1}{2}}-I\|_{F} & \leq\frac{1}{2}\frac{\beta^{2}}{1-\beta}
	\end{align*}
	and 
	\begin{align*}
	\|(\overline{D}^{0})^{-\frac{1}{2}}D^{1}(\overline{D}^{0})^{-\frac{1}{2}}-I\|_{F} & \le\frac{\beta}{1-\beta}.
	\end{align*}
\end{proposition}
%
Our next result shows that starting from an $O(\delta)$ approximate
center $(R^{0},S^{0},D^{0},X^{0},Y^{0},Z^{0})$ instead of an exact
center for $\kappa^{0}$, by following the procedures described in
Proposition \ref{prop:initial} to form the initial set $(\overline{R}^{0},\overline{S}^{0},\overline{D}^{0},\overline{X}^{0},\overline{Y}^{0},\overline{Z}^{0})$
for $\kappa^{1}$, this intial set also satisfies the closeness conditions
\begin{align*}
\delta(\overline{R}^{0},\overline{X}^{0}) & \leq\delta',\delta(\overline{D}^{0},\overline{Z}^{0})\leq\delta',\delta(\overline{S}^{0},\overline{Y}^{0})\leq\delta'
\end{align*}
for $\delta'=\beta+\delta$, i.e. it is an $O(\beta+\delta)$ approximate
analytic center for $\kappa^{1}$, for $\delta$ sufficiently small.
This $O(\beta+\delta)$ approximate center can then be used in the
Newton step in Proposition \ref{prop:Newton step} to obtain
an $O((\beta+\delta)^{2})=O(\delta)$ approximate center for $\kappa^{1}$,
thus ensuring that we can go from an $O(\delta)$ approximate center
for $\kappa^{0}$ to an $O(\delta)$ approximate center for $\kappa^{1}$
with a single Newton step. 
\begin{proposition}\label{prop:approximate}
	Suppose that $(R^{0},S^{0},D^{0},X^{0},Y^{0},Z^{0})$ satisfy 
	\begin{align*}
	R^{0} & =M-D^{0}\succeq0\\
	S^{0} & =\kappa^{0}S^{0}-M\succeq0\\
	D^{0} & \succeq0\\
	Z^{0}+\kappa^{0}Y^{0} & =X^{0}
	\end{align*}
	with $\delta(R^{0},X^{0})\leq\delta,\delta(D^{0},Z^{0})\leq\delta,\delta(S^{0},Y^{0})\leq\delta$
	for some $\delta\in(0,1)$. Further, let $\Delta\kappa=\kappa^{0}-\kappa^{1}$
	with 
	\begin{align*}
	\Delta\kappa & =\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}
	\end{align*}
	where $\beta\in(0,1)$ is a sufficiently small constant, then with
	\begin{align*}
	\overline{R}^{0} & =R^{0},\overline{S}^{0}=-\Delta\kappa D^{0}+S^{0},\overline{D}^{0}=D^{0}\\
	\overline{X}^{0} & =X^{0},\overline{Y}^{0}=Y^{0},\overline{Z}^{0}=\Delta\kappa Y^{0}+Z^{0}
	\end{align*}
	we have 
	$\overline{R}^{0} =M-\overline{D}^{0}\succeq0$, $\overline{S}^{0} =\kappa^{1}\overline{D}^{0}-M\succeq 0$, $\overline{D}^{0} \succeq0$, $\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0} =\overline{X}^{0}$,
	and $\delta(\overline{R}^{0},\overline{X}^{0})  \leq\beta$, $\delta(\overline{S}^{0},\overline{Y}^{0})\leq\delta+\beta$, $\delta(\overline{D}^{0},\overline{Z}^{0})\leq\delta+\beta$.

\end{proposition}
%
The above three results guarantee that if we start from an $O(\delta)$
approximate center for $\kappa^{0}$, by taking a small but constant
step $\Delta\kappa$, a Newton update step yields an $O(\delta)$
approximate center for $\kappa^{1}=\kappa^{0}-\Delta\kappa$, and
we may iteratively generate approximate centers in this fashion. In
the next result, we show that approximate centers, as the name suggests,
yields a potential that is close to that of the exact center, and
we have thus obtained an algorithm with approximate centers, such that the reduction
in potential at every step is constant, and the termination criterion
is the same as before, when the potential drops below
some threshold. 
\begin{theorem}
	\label{thm:approximate center}Let $\overline{D}^{0}$ and $\overline{D}^{1}$
	be approximate centers for $\kappa^{0}$ and $\kappa^{1}=\kappa^{0}-\frac{\beta}{Tr(\overline{D}^{0}\cdot(\kappa^{0}\overline{D}^{0}-M)^{-1})}$
	respectively, obtained using the procedures in Proposition \ref{prop:initial}
	to generate a feasible point and the Newton update with Nesterov-Todd
	directions for $\beta$ sufficiently small. If 
	\begin{align*}
	\delta(\overline{R}^{0},\overline{X}^{0}) & \leq\delta,\delta(\overline{D}^{0},\overline{Z}^{0})\leq\delta,\delta(\overline{S}^{0},\overline{Y}^{0})\leq\delta
	\end{align*}
	for $\delta$ a small universal constant, then 
	\begin{align*}
	\delta(\overline{R}^{1},\overline{X}^{1}) & \leq\delta,\delta(\overline{D}^{1},\overline{Z}^{1})\leq\delta,\delta(\overline{S}^{1},\overline{Y}^{1})\leq\delta
	\end{align*}
	and $P(\overline{D}^{1},\kappa^{1})\leq P(\overline{D}^{0},\kappa^{0})-c\beta$
	for $c\in(0,1)$ a universal constant. 
\end{theorem}
%The above result thus guarantees that if we start from an approximate center that is accurate enough, we can always ensure that the updated approximate center obtained from a Newton step with Nesterov-Todd direction remain as accurate, given small but constant step size.
\begin{algorithm}[Potential Reduction with Approximate Analytic Center]
	\label{alg:approximate}
	\begin{enumerate}
	\normalfont
	    \item  Let $\overline{D}^{0}$ be an $O(\beta)$ approximate analytic
	center of $\Gamma(\kappa^{0})$ with $\kappa^{0}>\kappa^{\ast}$.
	Set $k=0$. 
	
	\item Let $\Delta\kappa^{k}=\frac{\beta}{Tr(\overline{D}^{0}\cdot(\kappa^{0}\overline{D}^{0}-M)^{-1})}$
	for fixed constant $0<\beta<1$ and let $\kappa^{k+1}=\kappa^{k}-\Delta\kappa^{k}$.
	Update 
	\begin{align*}
	\overline{S}^{0}\leftarrow & -\Delta\kappa\overline{D}^{0}+\overline{S}^{0}\\
	\overline{Z}^{0}\leftarrow & \Delta\kappa Y^{0}+\overline{Z}^{0}
	\end{align*}
	to obtain feasible point for $\kappa^{k+1}$. 
	
	\item Use Newton's update to generate approximate analytic center
	$\overline{D}^{k+1}$ of $\Gamma(\kappa^{k+1})$. 
	
	\item If $P(\kappa^{k+1})>O(-nt)$, set $k\leftarrow k+1$ and return
	to Step 1. 
	\end{enumerate}
\end{algorithm}
%
Our results in this section provided us with algorithms that generate two-sided
optimal diagonal preconditioners  given any fixed matrix $A$. In practice, we observe that running
the bisection algorithm for a few itereations already
generates a pair of preconditioners $(D_1,D_2)$ with high quality. In numerical experiments in Section \ref{sec:experiments}, we will implement the bisection algorithm to solve \eqref{eq:two-sided-problem} when
comparing with other preconditioning techniques, including the one-sided optimal diagonal preconditioners via SDPs introduced next in Section \ref{sec:DSDP}.

==> theory-old.tex <==
\section{Optimal Diagonal Preconditioning via Potential Reduction}
\label{sec:optimal}



We have shown that when the population correlation matrix is diagonally
dominant, diagonal preconditioning of design matrix by sample standard
deviations yields a reduction in condition number on the order of
$\sqrt{\kappa(D)}$ with high probability. However, many population
correlation matrices are not diagonally dominant, or we may not be
able to easily verify this condition. In such cases, we need an efficient
method to obtain a diagonal conditioner that does reduce the condition
number of any fixed design matrix $X$. We turn to this problem in
this section. 

Given a fixed design matrix $X\in\mathbb{R}^{n\times p}$, we are
interested in the optimal diagonal preconditioning matrix $D$, that
gives the minimal condition number of 
\begin{align*}
\min_{D\text{ diagonal, }D\succeq0}XD^{-\frac{1}{2}}
\end{align*}
among all diagonal preconditioners. We first reformulate the problem
to a quasi-convex SDP problem that can be solved with bisection, and
then provide a faster potential reduction algorithm with guarantee
on convergence. The purpose of studying the optimal diagonal preconditioning
procedure is the following:
\begin{enumerate}
	\item In settings where diagonal preconditioning helps to reduce condition
	number, we would like to compare the performances of diagonal preconditioning
	using column standard deviation/norm studied in the previous section
	with that of the optimal diagonal preconditioning, to see how much
	gap there is between the two. 
	\item In situations where diagonal preconditioning with sample standard
	deviation/norm does not actually reduce the condition number, we may
	instead use the optimal diagonal preconditioning procedure.
	\item We are also interested in how the result of adaptive diagonal preconditioning
	procedures, such as batch normalization, compares with the optimal
	diagonal preconditioning. This may help us understand the nature of
	such adaptive preconditioning procedures. 
\end{enumerate}

\subsection{Optimal Diagonal Preconditioning}

\textbf{}%
\begin{comment}
\textbf{(discussion with Boyd)}
\end{comment}

Writing $M=X^{T}X\in\mathbb{R}^{p\times p}$ and rewriting $D^{-\frac{1}{2}}$
as $D$, the optimal diagonal preconditioning problem is 
\begin{align*}
\min_{D\text{ diagonal}}\kappa(DMD)
\end{align*}
We can rewrite it as 
\begin{align*}
\min_{D,\kappa}\kappa\\
I\preceq DMD\preceq\kappa I
\end{align*}
The inequality constraints can be further simplified to $D^{-2}\preceq M\preceq\kappa D^{-2}$. The problem can thus be reformulated as 
\begin{align*}
\min_{\kappa,D}\kappa\\
s.t.M\succeq D\\
\kappa D\succeq M
\end{align*}
where $D$ is a diagonal matrix with strictly positive entries.

\begin{comment}
{[}FOC analysis:{]}Let $X$ and $Y$ be the multipliers of the first
and second constraints, with Lagrangian $\kappa-Tr(X(M-E))-Tr(Y(\kappa E-M))$.
The KKT condition is given by 
\begin{align*}
1 & =Tr(YE)\\
X & =\kappa Y
\end{align*}
But complementary slackness does not hold (strong duality does not
hold), otherwise they would imply $\kappa=1$. 
\end{comment}

We may solve this problem using bisection as follows. First find a large fixed $\kappa_{0}$ such that the convex
feasiblity SDP problem
\begin{align*}
\min_{D\succeq0}0\\
s.t.M\succeq D\\
\kappa_{0}D\succeq M
\end{align*}
has a solution. In practice, we can start with $\kappa_{0}=\kappa(M)$,
or if we have some prior information that there exists some $D_{0}$
that satisfies 
\begin{align*}
\kappa(D_{0}MD_{0}) & <\kappa(M)
\end{align*}
we can set $\kappa_{0}=\kappa(D_{0}MD_{0})$ as a warm start. Often
the choice $D_{0}\equiv\left(\text{diag}(M)\right)^{-1/2}$ or $D_{0}\equiv\left(\text{diag}(\text{std}(M))\right)^{-1/2}$
yields a smaller upper bound. 

Then, solve the feasibility problem
\begin{align*}
\min_{D\succeq0}0\\
s.t.M\succeq D\\
\frac{\kappa_{0}}{2}D\succeq M
\end{align*}

If it is feasible, then we know the optimal objective value is in
$[1,\frac{\kappa_{0}}{2}]$, otherwise it is in $[\frac{\kappa_{0}}{2},\kappa_{0}]$.
We can find an $\epsilon$-optimal solution in $O(\log\frac{1}{\epsilon})$
iterations. 

There is also a geometric interpretation of the feasibility problem
with parameter $\kappa$: it looks for an ellipsoid $E$ with axes
of symmetry the coordinate axes, such that it is inscribed in the
ellipsoid defined by $M$, and such that a multiple $\kappa$ of $E$
includes the ellipsoid defined by $M$. Such inscribing and containing
ellipsoids have been used the ellipsoid method, where the ellipsoids
are not constrained to be symmetric along coordinate axes. The geometric
interpretation also makes it clear that the optimal value $\kappa^{\ast}\geq1$
is achieved. 

\begin{algorithm}
	\label{alg:bisection}
	
	Step 0. Start with $\kappa^{0}>\kappa^{\ast}$ such that 
	\begin{align*}
	\min_{D\succeq0}0\\
	s.t.M\succeq D\\
	\kappa_{0}D\succeq M
	\end{align*}
	is feasible. Set $\kappa_{min}=1$, $\kappa_{\max}=\kappa_{0}$. 
	
	Step 1. Solve the feasibility problem 
	\begin{align*}
	\min_{D\succeq0}0\\
	s.t.M\succeq D\\
	\frac{\kappa_{\max}+\kappa_{\min}}{2}D\succeq M
	\end{align*}
	If it is feasible, then set $\kappa_{max}\leftarrow\frac{\kappa_{\max}+\kappa_{\min}}{2}$.
	Otherwise, set $\kappa_{\min}\leftarrow\frac{\kappa_{\max}+\kappa_{\min}}{2}$. 
	
	Step 2. If $\kappa_{max}-\kappa_{min}>\epsilon$, return to Step 1. 
\end{algorithm}

We next develop an interior point method that finds an $\epsilon$-optimal
diagonal scaling in $O(\log\frac{1}{\epsilon})$ iterations, where
each iteration consists of a Newton update step. This is in contrast
to the bisection algorithm, which also has $O(\log\frac{1}{\epsilon})$
iterations, but each iteration consists of solving a SDP feasibility
problem. The formulation and proof borrows ideas from interior point
methods for linear programming and semidefinite programming, in particular
\cite{mizuno1992new,ye1992potential,ye1995neumann,nesterov1997self},
most notable of which are \cite{nesterov1997self}
on Newton updates in SDP and \cite{ye1995neumann}
on the ``von Neumann economic growth problem''. 

\subsection{Interior Point Algorithms with Potential Reduction}

Recall the reformulated optimal diagonal preconditioning problem
\begin{align*}
\min_{D\succeq0}\kappa\\
s.t.M\succeq D\\
\kappa D\succeq M
\end{align*}

Following \cite{ye1995neumann}, we define the potential function
as
\begin{align*}
P(\kappa) & =\sum_{i}\log\lambda_{i}(M-D^{\kappa})+\sum_{i}\log\lambda_{i}(\kappa D^{\kappa}-M)+\sum_{i}\log D_{ii}^{\kappa}
\end{align*}
where $D^{\kappa}$ is the \emph{analytic center} of the feasible
region \textbf{
	\begin{align*}
	\Gamma(\kappa) & =\{D\succeq0:D\text{ diagonal};M\succeq D;\kappa D\succeq M\}
	\end{align*}
} which is simply the unique maximizer of the strictly concave problem
\begin{align*}
\max_{D\succeq0\text{ diagonal}} & \sum_{i}\log\lambda_{i}(M-D)+\sum_{i}\log\lambda_{i}(\kappa D-M)+\sum_{i}\log D_{ii}\\
& \Longleftrightarrow\\
\max_{D\succeq0\text{ diagonal}} & \log\det(M-D)+\log\det(\kappa D-M)+\log\det D
\end{align*}

See also \cite{mizuno1993adaptive,luo1998superlinear,sturm1999symmetric}
for the use of analytic centers in path-following and potential reduction
interior point algorithms for LP and SDP problems. 

The geometric interpretation of the problem makes it clear that if
the feasible region $\Gamma(\kappa^{0})$ has a non-empty interior
for some $\kappa^{0}<\infty$, then the feasible region $\Gamma(\kappa)$
has a non-empty interior for all $\kappa\geq\kappa^{0}$, so that
the analytic center is well defined. At the optimal objective value
$\kappa^{\ast}\geq1$, however, the solution set has no interior because
it must be the case that $\lambda_{p}(\kappa D-M)=0$ for any $D$
in the solution set, where $\lambda_{1}\geq\lambda_{2}\geq\cdots\geq\lambda_{p}$
are the eigenvalues of a matrix, and so perturbing $D$ in some direction
by any amount will violate the constraint $M\succeq D$. 
\begin{lemma}
	For $M\succ0,$ the feasible set of the feasibility problem 
	\begin{align*}
	\min_{D\succeq0}0\\
	s.t.M\succeq D\\
	\kappa D\succeq M
	\end{align*}
	has bounded non-empty interior for all $\kappa>\kappa^{\ast}$.
\end{lemma}
Next we show that the potential function is monotonic in $\kappa$,
and that it is bounded away from $P(\kappa^{\ast})$, for any $\kappa$
large, so that it is a reasonable measure of the progress of the problem:
we just need to be able to reduce the potential function by a constant
amount at every step and terminate when the potential function is
reduced below a certain threshold determined by accuracy $\epsilon$. 
\begin{proposition}\label{prop:monotonicity}
	If $\kappa_{0}>\kappa_{1}>\kappa^{\ast}$, then $P(\kappa_{0})>P(\kappa_{1})$. 
\end{proposition}
\proof{Proof}
See the appendix.
	\hfill \halmos
\endproof
%
\begin{proposition}\label{prop:lower bound}
	Let $t$ satisfy $\kappa^{\ast}\leq2^{t}$, then for any $\overline{\kappa}>\kappa^{\ast}+2^{-t}$,
	we have
	\begin{align*}
	P(\overline{\kappa}) & >-Cpt
	\end{align*}
	for some universal constant that only depends on $M$. 
\end{proposition}
\proof{Proof}
See the appendix.\hfill \halmos 
\endproof
These two results imply that if $P(\kappa)<O(-pt)$, then we must
have $\kappa\leq\kappa^{\ast}+2^{-t}$. Therefore if we can find a
$D$ whose associated potential is below the threshold of $O(p\log\epsilon)$,
we have found an approximate solution that yields a condition number
that is within $\epsilon$ of the optimal condition number. Our goal
is then to design an algorithm that achieves constant reduction of
the potential at every iteration, which would guarantee an iteration
complexity of $O(\log\frac{1}{\epsilon})$. 

In the next two subsections, we develop potential reduction algorithms based on this idea, using exact and and approximate analytic centers, respetively. Before doing so, we show that the analytic center satisfies an equality condition that is useful in the proof of the reduction of potential function. This is essentially the first order condition of the convex optimziation problem, but because it also serves an important role in the Newton reduction step, we state it is a particular form in the next lemma. 
\begin{lemma}
	The analytic center $D$ of the feasible region $\Gamma(\kappa)$
	satisfies 
	\begin{align*}
	Z+\kappa Y & =X
	\end{align*}
	where \begin{align*}
	X&=R^{-1},Y=S^{-1},Z=D^{-1},R=M-D,S=\kappa D-M
	\end{align*}
\end{lemma}
\proof{Proof}
	Since $D$ solves the convex problem
	\begin{align*}
	& \max_{D}\log\det(M-D)+\log\det(\kappa D-M)+\log\det D
	\end{align*}
	The first order condition implies 
	\begin{align*}
	-(M-D)^{-1}+\kappa(\kappa D-M)^{-1}+D^{-1} & =0
	\end{align*}
	so if we define $R=M-D$ and $S=\kappa D-M$, and 
	\begin{align*}
	X	=R^{-1},Y=S^{-1},Z=D^{-1}
	\end{align*}
	then we have $	Z+\kappa Y  =X$ and moreover $R+S=(\kappa-1)D$. 
	\hfill \halmos
\endproof

\subsection{Analysis of Potential Reduction with Exact Analytic Center}

Let $D^{0},D^{1}$ be the analytic centers of $\Gamma^{0}=\Gamma(\kappa^{0})$
and $\Gamma^{1}=\Gamma(\kappa^{1})$. With a suitable choice of $\Delta\kappa=\kappa^{0}-\kappa^{1}>0$,
we show that the analytic centers $D^{0}$ and $D^{1}$ are close,
and that 
\begin{align*}
P(\kappa^{1}) & \leq P(\kappa^{0})-\Omega(1)
\end{align*}
so that we can achieve constant reduction of the potential function
by going from $D^{0}$ to $D^{1}$. To obtain $D^{1}$ from $D^{0}$,
we can use symmetrized versions of Newton iterations with a quadratic
convergence rate. The exact form of the Newton iteration is deferred
to the next subsection, where we propose a practical potential algorithm
using approximate analytic centers and only one Newton step.
%
\begin{theorem}
	\label{thm:exact center}Let $\kappa^{\ast}\in[1,\infty)$ be the
	solution of 
	\begin{align*}
	\min_{D\succeq0}\kappa\\
	s.t.M\succeq D\\
	\kappa D\succeq M
	\end{align*}
	and let $\overline{\kappa}$ be a known upper bound of $\kappa^{\ast}$,
	i.e. 
	\begin{align*}
	\min_{D\succeq0}0\\
	s.t.M\succeq D\\
	\overline{\kappa}D\succeq M
	\end{align*}
	is feasible. 
	
	Let $D^{0}$ and $D^{1}$ be the analytic centers of $\Gamma^{0}=\Gamma(\kappa^{0})$
	and $\Gamma^{1}=\Gamma(\kappa^{1})$ for $\kappa^{0},\kappa^{1}\in(\kappa^{\ast},\overline{\kappa})$.
	If $\Delta\kappa=\kappa^{0}-\kappa^{1}>0$ satisfies
	\begin{align*}
	\Delta\kappa & =\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}\\
	& =\frac{\beta}{e^{T}D^{0}\text{diag}((\kappa^{0}D^{0}-M)^{-1})e}
	\end{align*}
	for some sufficiently small $\beta\in(0,1)$ that only depends on
	$\overline{\kappa},M$, then 
	\begin{align*}
	\sqrt{Tr((D^{1})^{1/2}(D^{0})^{-1}(D^{1})^{1/2}-I)^{2}} & \leq c\cdot\beta\\
	\sqrt{Tr((D^{0})^{1/2}(D^{1})^{-1}(D^{0})^{1/2}-I)^{2}} & \leq c\cdot\beta
	\end{align*}
	{} for some constant $c$
	and\textbf{
		\begin{align*}
		P(\kappa^{1}) & \leq P(\kappa^{0})-\beta
		\end{align*}
	}
\end{theorem}
\proof{Proof}
	See the appendix.
	\hfill \halmos
\endproof

We have thus obtained a conceptual algorithm, which uses the exact
analytic center, summarized in Algorithm \ref{alg:exact}.
\begin{algorithm}
	\label{alg:exact}
	
	Step 0. Let $D^{0}$ be analytic center of $\Gamma(\kappa^{0})$ with
	$\kappa^{0}>\kappa^{\ast}$. Set $k=0$. 
	
	Step 1. Let 
	\begin{align*}
	\Delta\kappa^{k} & =\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}
	\end{align*}
	for some small constant $0<\beta<1$ and let $\kappa^{k+1}=\kappa^{k}-\Delta\kappa^{k}$.
	Then use Newton's method described in the next section to generate
	the axact analytic center $D^{k+1}$ of $\Gamma(\kappa^{k+1})$. 
	
	Step 2. If $P(\kappa^{k+1})>O(-pt)$, set $k\leftarrow k+1$ and return
	to Step 1. 
\end{algorithm}

\subsection{Algorithm with Approximate Analytic Center}

Given step size $\Delta\kappa$, in order to apply the potential reduction
algorithm, we still need to find the new analytic center $D^{1}$
corresponding to $\kappa^{0}-\Delta\kappa$. This can be achieved
using Newton iterations. However, it is not necessary to use exact
analytic centers. Instead, we can use an approximate analytic center
obtained from only one Newton update step, and show that the max-potential
still reduces by a constant amount. Moreover, if we start from an approximate
analytic center, one Newton step with the appropriate step size $\Delta\kappa$
yields an approximate center that still achieves this constant reduction
in potential. We develop these results in this subsection. 

By an approximate analytic center, we mean a set of variables $(R,S,D,X,Y,Z)$
that satisfy the optimality conditions 
\begin{align*}
R & =M-D\succeq0,\\
S & =\kappa D-M\succeq0\\
D & \succeq0\\
Z+\kappa Y & =X
\end{align*}
but instead of requiring $RX=SY=DZ=I$ as is true for the exact analytic
center, we allow the products to be close to the identity $I$.

We define a measure of proximity of the products as follows 
\begin{align*}
\delta(A,B) & :=\sqrt{Tr(B^{1/2}AB^{1/2}-I)^{2}}\\
& =\|B^{1/2}AB^{1/2}-I\|_{F}=\|A^{1/2}BA^{1/2}-I\|_{F}
\end{align*}
where the equality follows from the fact that the Frobenius norm
is a spectral property for symmetric matrices. We may also check that
\begin{align*}
\delta(A,B) & =\sqrt{Tr((AB-I)^{2})}=\sqrt{Tr((BA-I)^{2})}
\end{align*}
As we will see in the following results, this is the appropriate measure
of proximity. The first result we show is that starting from an analytic
center for $\Gamma(\kappa^{0})$, we can obtain a feasible point in
$\Gamma(\kappa^{1})$ that is an $O(\beta)$ approximate analytic center.
\begin{proposition}
	\label{prop:initial}
	Let $D^{0}$ be the exact analytic center of $\kappa^{0}$. Define
	$R_{0}=M-D_{0}$, $S_{0}=\kappa_{0}D_{0}-M$ and $X_{0}=R_{0}^{-1},Y_{0}=S_{0}^{-1},Z_{0}=D_{0}^{-1}$.
	
	Further, let $\Delta\kappa=\kappa^{0}-\kappa^{1}$ with $\Delta\kappa=\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}$
	where $\beta\in(0,1)$ is a sufficiently small constant, and 
	\begin{align*}
	\overline{R}^{0} & =R^{0},\overline{S}^{0}=-\Delta\kappa D^{0}+S^{0},\overline{D}^{0}=D^{0}\\
	\overline{X}^{0} & =X^{0},\overline{Y}^{0}=Y^{0},\overline{Z}^{0}=\Delta\kappa Y^{0}+Z^{0}
	\end{align*}
	Then, the new variables satisfy 
	\begin{align*}
	\overline{R}^{0} & =M-\overline{D}^{0}\succeq0\\
	\overline{S}^{0} & =\kappa^{1}\overline{D}^{0}-M\succeq0\\
	\overline{D}^{0} & \succeq0
	\end{align*}
	and $\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0}=\overline{X}^{0}$.
	Moreover, $\delta(\overline{S}^{0},\overline{Y}^{0})\leq\beta,\delta(\overline{D}^{0},\overline{Z}^{0})\leq\beta,\delta(\overline{R}^{0},\overline{X}^{0})=0$.
\end{proposition}
\proof{Proof}
	We can readily verify that the new variables satisfy the desired equalities.
	When $\Delta\kappa$ is appropriately chosen as in the previous theorem,
	we can guarantee that $\overline{S}^{0}\succeq0$. Now 
	\begin{align*}
	\delta(\overline{S}^{0},\overline{Y}^{0})^{2}=Tr((\overline{S}^{0}\overline{Y}^{0}-I)^{2}) & =Tr((-\Delta\kappa D^{0}+S^{0})Y^{0}-I)^{2}\\
	& =Tr(-\Delta\kappa D^{0}Y^{0})^{2}\\
	& =Tr(-\Delta\kappa D^{0}(\kappa_{0}D_{0}-M)^{-1})^{2}\\
	& \leq(Tr(-\Delta\kappa D^{0}(\kappa_{0}D_{0}-M)^{-1}))^{2}=\beta^{2}
	\end{align*}
	where we have used $Tr(A^{2})=(TrA)^{2}-2\sigma_{2}(A)$ where $\sigma_{2}(A)=\sum_{i<j}\lambda_{i}\lambda_{j}$
	and $\lambda_{i}$ are the eigenvalues of $A$. Therefore, $\delta(\overline{S}^{0},\overline{Y}^{0})\leq\beta$.
	Similarly, $\delta(\overline{D}^{0},\overline{Z}^{0})\leq\beta$ and
	since $\overline{R}^{0}=R^{0},\overline{X}^{0}=X^{0}$, we have $\delta(\overline{D}^{0},\overline{Z}^{0})=0$
	\hfill \halmos
\endproof
Next we show that this set of variables $(\overline{R}^{0},\overline{S}^{0},\overline{D}^{0},\overline{X}^{0},\overline{Y}^{0},\overline{Z}^{0})$
can be used as an initial set to generate a new $ O(\beta^{2}) $ approximate center
for $\kappa^{1}$, using a Newton step. This also implies that starting from an approximate analytic center we can obtain an exact analytic center by applying the Newton iterations with quadratic convergence. Here to ensure the symmetry
of updates in the Newton step, we use the Nesterov-Todd direction
\cite{todd1998nesterov,nesterov1997self}. 

\begin{proposition}
	\label{prop:Newton step}Let \label{prop:Newton step}Let $(\overline{R}^{0},\overline{S}^{0},\overline{D}^{0},\overline{X}^{0},\overline{Y}^{0},\overline{Z}^{0})$
	be any set that satisfy 
	\begin{align*}
	\overline{R}^{0} & =M-\overline{D}^{0}\succeq0\\
	\overline{S}^{0} & =\kappa^{1}\overline{D}^{0}-M\succeq0\\
	\overline{D}^{0} & \succeq0
	\end{align*}
	and $\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0}=\overline{X}^{0}$,
	with 
	\begin{align*}
	\delta(\overline{R}^{0},\overline{X}^{0})=\|(\overline{R}^{0})^{\frac{1}{2}}\overline{X}^{0}(\overline{R}^{0})^{\frac{1}{2}}-I\|_{F} & \leq\beta\\
	\delta(\overline{D}^{0},\overline{Z}^{0})=\|(\overline{D}^{0})^{\frac{1}{2}}\overline{Z}^{0}(\overline{D}^{0})^{\frac{1}{2}}-I\|_{F} & \leq\beta\\
	\delta(\overline{S}^{0},\overline{Y}^{0})=\|(\overline{S}^{0})^{\frac{1}{2}}\overline{Y}^{0}(\overline{S}^{0})^{\frac{1}{2}}-I\|_{F} & \leq\beta
	\end{align*}
	for some $\beta\in(0,1)$. 
	
	Let $X^{1},Y^{1},Z^{1},R^{1},S^{1},D^{1}$ be defined by 
	\begin{align*}
	X^{1} & =\overline{X}^{0}+\Delta X,Y^{1}=\overline{Y}^{0}+\Delta Y,Z^{1}=\overline{Z}^{0}+\Delta Z\\
	R^{1} & =\overline{R}^{0}+\Delta R,S^{1}=\overline{S}^{0}+\Delta S,D^{1}=\overline{D}^{0}+\Delta D
	\end{align*}
	where the increments $\Delta$s are given by the Newton step %
	\begin{comment}
	The Newton step is to ensure 
	\begin{align*}
	\overline{R}^{0} & =M-\overline{D}^{0}\succeq0\\
	\overline{S}^{0} & =\kappa^{1}\overline{D}^{0}-M\succeq0\\
	\overline{D}^{0} & \succeq0
	\end{align*}
	and 
	\begin{align*}
	\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0} & =\overline{X}^{0}
	\end{align*}
	still holds. 
	
	Regular Newton step is
	
	\begin{align*}
	\overline{D}^{0}\cdot\Delta Z+\overline{Z}^{0}\cdot\Delta D & =I-\overline{D}^{0}\cdot\overline{Z}^{0}\\
	\overline{R}^{0}\cdot\Delta X+\overline{X}^{0}\cdot\Delta R & =I-\overline{R}^{0}\cdot\overline{X}^{0}\\
	\overline{S}^{0}\cdot\Delta Y+\overline{Y}^{0}\cdot\Delta S & =I-\overline{S}^{0}\cdot\overline{Y}^{0}
	\end{align*}
	but here we need to use the Nesterov-Todd direction to ensure symmetry
	of updates. 
	\end{comment}
	\begin{align*}
	\Delta Z+W^{-1}\Delta DW^{-1} & =(\overline{D}^{0})^{-1}-\overline{Z}^{0}\\
	\Delta X+U^{-1}\Delta RU^{-1} & =(\overline{R}^{0})^{-1}-\overline{X}^{0}\\
	\Delta Y+V^{-1}\Delta S & V^{-1}=(\overline{S}^{0})^{-1}-\overline{Y}^{0}
	\end{align*}
	{} and 
	\begin{align*}
	\Delta R & =-\Delta D,\Delta S=\kappa^{1}\Delta D,\Delta X=\Delta Z+\kappa^{1}\Delta Y
	\end{align*}
	where $U,V,W$ are the geometric means 
	\begin{align*}
	U & =(\overline{R}^{0})^{1/2}((\overline{R}^{0})^{1/2}\overline{X}^{0}(\overline{R}^{0})^{1/2})^{-1/2}(\overline{R}^{0})^{1/2}\\
	V & =(\overline{S}^{0})^{1/2}((\overline{S}^{0})^{1/2}\overline{Y}^{0}(\overline{S}^{0})^{1/2})^{-1/2}(\overline{S}^{0})^{1/2}\\
	W & =(\overline{D}^{0})^{1/2}((\overline{D}^{0})^{1/2}\overline{Z}^{0}(\overline{D}^{0})^{1/2})^{-1/2}(\overline{D}^{0})^{1/2}
	\end{align*}
	to ensure that updates are symmetric.
	
	Then we have 
	\begin{align*}
	\delta(R^{1},X^{1})=\|(R^{1})^{\frac{1}{2}}X^{1}(R^{1})^{\frac{1}{2}}-I\|_{F} & \leq\frac{1}{2}\frac{\beta^{2}}{1-\beta}\\
	\delta(S^{1},Y^{1})=\|(S^{1})^{\frac{1}{2}}Y^{1}(S^{1})^{\frac{1}{2}}-I\|_{F} & \leq\frac{1}{2}\frac{\beta^{2}}{1-\beta}\\
	\delta(D^{1},Z^{1})=\|(D^{1})^{\frac{1}{2}}Z^{1}(D^{1})^{\frac{1}{2}}-I\|_{F} & \leq\frac{1}{2}\frac{\beta^{2}}{1-\beta}
	\end{align*}
	and 
	\begin{align*}
	\|(\overline{D}^{0})^{-\frac{1}{2}}D^{1}(\overline{D}^{0})^{-\frac{1}{2}}-I\|_{F} & \le\frac{\beta}{1-\beta}
	\end{align*}
\end{proposition}
\proof{Proof}
	See the appendix.
	\hfill \halmos
\endproof
%
Our next result shows that starting from an $O(\delta)$ approximate
center $(R^{0},S^{0},D^{0},X^{0},Y^{0},Z^{0})$ instead of an exact
center for $\kappa^{0}$, by following the procedures described in
Proposition \ref{prop:initial} to form the initial set $(\overline{R}^{0},\overline{S}^{0},\overline{D}^{0},\overline{X}^{0},\overline{Y}^{0},\overline{Z}^{0})$
for $\kappa^{1}$, this intial set also satisfies the closeness conditions
\begin{align*}
\delta(\overline{R}^{0},\overline{X}^{0}) & \leq\delta',\delta(\overline{D}^{0},\overline{Z}^{0})\leq\delta',\delta(\overline{S}^{0},\overline{Y}^{0})\leq\delta'
\end{align*}
for $\delta'=\beta+\delta$, i.e. it is an $O(\beta+\delta)$ approximate
analytic center for $\kappa^{1}$, for $\delta$ sufficiently small.
This $O(\beta+\delta)$ approximate center can then be used in the
Newton iteration in Proposition \ref{prop:Newton step} to obtain
an $O((\beta+\delta)^{2})=O(\delta)$ approximate center for $\kappa^{1}$,
thus ensuring that we can go from an $O(\delta)$ approximate center
for $\kappa^{0}$ to an $O(\delta)$ approximate center for $\kappa^{1}$
with a Newton step. 
\begin{proposition}\label{prop:approximate}
	Suppose that $(R^{0},S^{0},D^{0},X^{0},Y^{0},Z^{0})$ satisfy 
	
	\begin{align*}
	R^{0} & =M-D^{0}\succeq0\\
	S^{0} & =\kappa^{0}S^{0}-M\succeq0\\
	D^{0} & \succeq0\\
	Z^{0}+\kappa^{0}Y^{0} & =X^{0}
	\end{align*}
	with $\delta(R^{0},X^{0})\leq\delta,\delta(D^{0},Z^{0})\leq\delta,\delta(S^{0},Y^{0})\leq\delta$
	for some $\delta\in(0,1)$. Further, let $\Delta\kappa=\kappa^{0}-\kappa^{1}$
	with 
	\begin{align*}
	\Delta\kappa & =\frac{\beta}{Tr(D^{0}\cdot(\kappa^{0}D^{0}-M)^{-1})}
	\end{align*}
	where $\beta\in(0,1)$ is a sufficiently small constant, then with
	\begin{align*}
	\overline{R}^{0} & =R^{0},\overline{S}^{0}=-\Delta\kappa D^{0}+S^{0},\overline{D}^{0}=D^{0}\\
	\overline{X}^{0} & =X^{0},\overline{Y}^{0}=Y^{0},\overline{Z}^{0}=\Delta\kappa Y^{0}+Z^{0}
	\end{align*}
	we have 
	$\overline{R}^{0} =M-\overline{D}^{0}\succeq0$, $\overline{S}^{0} =\kappa^{1}\overline{D}^{0}-M\succeq 0$, $\overline{D}^{0} \succeq0$, $\overline{Z}^{0}+\kappa^{1}\overline{Y}^{0} =\overline{X}^{0}$,
	and $\delta(\overline{R}^{0},\overline{X}^{0})  \leq\beta$, $\delta(\overline{S}^{0},\overline{Y}^{0})\leq\delta+\beta$, $\delta(\overline{D}^{0},\overline{Z}^{0})\leq\delta+\beta$.

\end{proposition}
\proof{Proof}
    See the appendix.
	\hfill \halmos
\endproof
\textbf{}
%
The above three results guarantee that if we start from an $O(\delta)$
approximate center for $\kappa^{0}$, by taking a small but constant
step $\Delta\kappa$, a Newton update step yields an $O(\delta)$
approximate center for $\kappa^{1}=\kappa^{0}-\Delta\kappa$, and
we may iteratively generate approximate centers in this fashion. In
the next result, we show that approximate centers, as the name suggests,
yields a potential that is close to that of the exact center, and
so we have an algorithm with approximate centers, such that the reduction
in potential at every step is constant, and the termination criterion
is when the potential evaluated at the approximate center drops below
some threshold. 
\begin{theorem}
	\label{thm:approximate center}Let $\overline{D}^{0}$ and $\overline{D}^{1}$
	be approximate centers for $\kappa^{0}$ and $\kappa^{1}=\kappa^{0}-\frac{\beta}{Tr(\overline{D}^{0}\cdot(\kappa^{0}\overline{D}^{0}-M)^{-1})}$
	respectively, obtained using the procedures in Proposition \ref{prop:initial}
	to generate feasible point and the Newton update with Nesterov-Todd
	direction for $\beta$ sufficiently small. If 
	\begin{align*}
	\delta(\overline{R}^{0},\overline{X}^{0}) & \leq\delta,\delta(\overline{D}^{0},\overline{Z}^{0})\leq\delta,\delta(\overline{S}^{0},\overline{Y}^{0})\leq\delta
	\end{align*}
	for $\delta$ a small universal constant, then 
	\begin{align*}
	\delta(\overline{R}^{1},\overline{X}^{1}) & \leq\delta,\delta(\overline{D}^{1},\overline{Z}^{1})\leq\delta,\delta(\overline{S}^{1},\overline{Y}^{1})\leq\delta
	\end{align*}
	and $P(\overline{D}^{1},\kappa^{1})\leq P(\overline{D}^{0},\kappa^{0})-c\beta$
	for $c\in(0,1)$ a universal constant. 
\end{theorem}
\proof{Proof}
	See the appendix.
	\hfill \halmos
\endproof

\begin{algorithm}
	\label{alg:approximate}
	
	Step 0. Let $\overline{D}^{0}$ be an $O(\beta)$ approximate analytic
	center of $\Gamma(\kappa^{0})$ with $\kappa^{0}>\kappa^{\ast}$.
	Set $k=0$. 
	
	Step 1. Let $\Delta\kappa^{k}=\frac{\beta}{Tr(\overline{D}^{0}\cdot(\kappa^{0}\overline{D}^{0}-M)^{-1})}$
	for some small constant $0<\beta<1$ and let $\kappa^{k+1}=\kappa^{k}-\Delta\kappa^{k}$.
	Update 
	\begin{align*}
	\overline{S}^{0}\leftarrow & -\Delta\kappa\overline{D}^{0}+\overline{S}^{0}\\
	\overline{Z}^{0}\leftarrow & \Delta\kappa Y^{0}+\overline{Z}^{0}
	\end{align*}
	to obtain feasible point for $\kappa^{k+1}$. 
	
	Step 2. Use Newton's update to generate approximate analytic center
	$\overline{D}^{k+1}$ of $\Gamma(\kappa^{k+1})$. 
	
	Step 3. If $P(\kappa^{k+1})>O(-pt)$, set $k\leftarrow k+1$ and return
	to Step 1. 
\end{algorithm}
%
The above result thus guarantees that if we start from an approximate
center that is accurate enough, we can always ensure that the updated
approximate center obtained from a Newton step with Nesterov-Todd
direction remain as accurate, given small but constant step size.
Our results in this section provided us with two algorithms that generate
optimal diagonal preconditioners that guarantee reduction in condition
number, given any fixed matrix. In practice, we observe that running
the bisection algorithm or Newton update for a few itereations already
generates a good preconditioner, and that is what we implement when
comparing with other preconditioning methods. 
